Sparse and Low-rank Tensor Estimation via Cubic Sketchings

In this paper, we propose a general framework for sparse and low-rank tensor estimation from cubic sketchings. A two-stage non-convex implementation is developed based on sparse tensor decomposition and thresholded gradient descent, which ensures exact recovery in the noiseless case and stable recovery in the noisy case with high probability. The non-asymptotic analysis sheds light on an interplay between optimization error and statistical error. The proposed procedure is shown to be rate-optimal under certain conditions. As a technical by-product, novel high-order concentration inequalities are derived for studying high-moment sub-Gaussian tensors. An interesting tensor formulation illustrates the potential application to high-order interaction pursuit in high-dimensional linear regression.

==> t-cubic-sketch1-intro.tex <==



%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}\label{sec:intro}
%%%%%%%%%%%%%%%%%%%%%%%%%%%

The rapid advance in modern scientific technology gives rise to a wide range of high-dimensional tensor data \citep{K08, kolda2009}. Accurate estimation and fast communication/processing of tensor-valued parameters are crucially important in practice. For example, a tensor-valued predictor, which characterizes the association between brain diseases and scientific measurements, such as magnetic resonance imaging, becomes the point of interest \citep{zhou2013,li2013tucker, SL17}. Another example is tensor-valued image acquisition algorithms that can considerably reduce the number of required samples by exploiting the compressibility property of signals \citep{CC13, friedland2014compressive}. 

In particular, the following tensor estimation model is widely considered in recent literatures,
\begin{equation}\label{eq:general-model}
y_i = \langle \mT^\ast, \mX_i\rangle + \epsilon_i, \quad i=1,\ldots, n.
\end{equation}
Here, $\mX_i$ and $\epsilon_i$ are the measurement tensor and the noise, respectively. The goal is to estimate the unknown tensor $\mT^\ast$ from measurements $\{y_i, \mX_i\}_{i=1}^n$. A number of specific settings with varying forms of $\mX_i$ have been studied, e.g., tensor completion \citep{liu2013,yuan2016tensor,yuan2017incoherent,zhang2016cross,montanari2016spectral}, tensor regression \citep{zhou2013, li2013tucker,raskutti2015convex,chen2016non,li2017parsimonious, SL17}, multi-task learning \citep{romera2013multilinear}, etc.


%In this work, we assume tensor $\mT^*$ possesses CANDECOMP/PARAFAC low-rank, which is originally from CP-decomposition \citep{KB09} and commonly assumed in the tensor literature. In addition, we impose sparsity assumptions on the decomposition components $(\bbeta_{1k}^*, \bbeta_{2k}^*, \bbeta_{3k}^*)$, as justified by interaction models. 
%{\red (shorten this part, and move it to later paragraph.)} 
%{\red (connect some spcific settings here with the above general estimation framework, and combine with the previous paragraph)}%For example, \citep{yuan2016tensor, yuan2017incoherent, zhang2016cross} considered the low-rank tensor recovery from a small fraction of observable entries; different methods, \citep{zhou2013, li2013tucker,raskutti2015convex,chen2016non,rauhut2017low,li2017parsimonious} considered the sparse and low-rank tensor regression... \cite{romera2013multilinear} considered multi-task learning that {\red (Can you add more explanations?)}, \cite{Sun2016} considered tensor decomposition ..., 

%More specifically, the measurement tensors $\mX_i = \bx_i \circ \bx_i \circ \bx_i$ (symmetric cubic sketching) or $\mX_i= \bu_i\circ \bv_i\circ \bw_i$ (non-symmetric cubic sketching), where $\bx_i, \bu_i, \bv_i$, and $\bw_i$ are vectors of dimension corresponding to $\mT^\ast$, i.e.,


In this paper, we focus on the case that the measurement tensor can be written in a cubic form. For example, $\mX_i = \bx_i\circ\bx_i\circ\bx_i$ or $\mX_i=\bu_i\circ \bv_i\circ \bw_i$, depending on $\mT^*$ is symmetric or not. The cubic sketching form of $\mX_i$ is motivated by a number of applications.
\begin{itemize}
	\item \emph{Interaction effect estimation:} High-dimensional high-order interaction models have been considered under a variety settings \citep{bien2013lasso, hao2014interaction,fan2016interaction, basu2018iterative}. By writing $\mX_i = \bx_i\circ\bx_i\circ\bx_i$, we find that the interaction model has an interesting tensor representation (see left panel of Figure \ref{fig:illurstration}) which allows us to estimate high-order interaction terms using tensor techniques. This is in contrast with the existing literature that mostly focused on pair-wise interactions due to the model complexity and computational difficulties. More detailed discussions will be provided in Section \ref{sec:interaction}.
	\item \emph{High-order imaging/video compression:} High-order imaging/video compression %{\red (needs to mention this corresponds to non-symmetric tensor...)} 
	is an important task in modern digital imaging with various applications (see right panel of Figure \ref{fig:illurstration}), such as hyper-spectral imaging analysis \citep{li2010tensor} and facial imaging recognition \citep{vasilescu2003multilinear}. 
	In contrast to Gaussian ensembles for compression that each entry of $\mX_i$ is i.i.d. randomly generated \citep{zhou2013, raskutti2015convex,chen2016non}, the non-symmetric cubic sketchings, i.e., $\mX_i=\bu_i\circ \bv_i\circ \bw_i$, reduces the memory storage from $O(np^3)$ to $O(np)$, where $n$ is sample size and $p$ is the maximal dimension of tensor modes, but still preserve the optimal statistical rate. More detailed discussions will be provided in Section \ref{sec:non-symmetrc}. %This problem has a close connection with  tensor estimation with non-symmetric cubic sketchings. 
	%\item \emph{High-order moment estimation:} The estimation of higher moment, or high-order statistics, plays an important role in modern data analysis...  \cite{bourin1998efficiency} ... 
\end{itemize}
In practice, the total number of measurements $n$ is considerably smaller than the number of parameters in unknown tensor $\mT^*$, due to all kinds of restrictions such as time and storage. Fortunately, a variety of high-dimensional tensor data possess intrinsic structures, such as low-rankness \citep{kolda2009} and sparsity \citep{Sun2016}, which highly reduce the effective dimension of the parameter and make the accurate estimation possible. Please refer to \eqref{eq:mT_low-rank} and \eqref{eq:low_rank_nonsym} for  low-rank and sparse assumptions.

\begin{figure}[h!]
	\centering
		\vspace{0.1cm}
		\includegraphics[scale=0.5]{figure/tensor_inter.png}\;\;\;\;\;\;\;\;\;
		\includegraphics[scale=0.3]{figure/tensor_image.png}
		\vspace{-0.1in}
	\caption{Illustration for interaction reformulation and tensor image/video compression.}
	\label{fig:illurstration}
\end{figure}

In this paper, we propose a computationally efficient non-convex optimization approach for sparse and low-rank tensor estimation via cubic-sketchings. Our procedure is two-stage: 
\begin{itemize}
	\item[(i)] obtain an initial estimate via the method of tensor moment (motivated by high-order Stein's identity), and then apply sparse tensor decomposition to the initial estimate to output a provably warm start;
	\item[(ii)] use a thresholded gradient descent to iteratively refine the warm start along each tensor mode until convergence.
\end{itemize}
%{\red (More details are needed to describe our implementation.)} %This is essentially different from some low-rank projection techniques \citep{chen2016non} since the low-rankness in our algorithm will be automatically preserved. 
%The algorithm is data-driven and adaptive to each individual entry without tuning. {\red (This is a strong claim. From the algorithm we can see we need tons of tons of tuning parameters.)}
In theory, we carefully characterize the optimization and statistical errors at each iteration step. The output estimate is shown to converge in a geometric rate to an estimation with minimax optimal rate in statistical error (in terms of tensor Frobenius norm). In particular, after a logarithm factor of iterations, whenever $n \gtrsim K^2(s\log(ep/s))^{\tfrac{3}{2}}$, the proposed estimator $\hat{\mT}$ achieves
\begin{equation}\label{eq:rintro-recovery-rate}
	\left\|\hat{\mT} - \mT^*\right\|_F^2 \leq C\sigma^2\frac{Ks\log (p/s)}{n},
\end{equation}
with high probability, where $s$, $K$, $p$, and $\sigma^2$ are the sparsity, rank, dimension, and noise level, respectively. 
We further establish the matching minimax lower bound to show that \eqref{eq:rintro-recovery-rate} is indeed optimal over a large class of sparse low-rank tensors. Our optimality result can be further extended to the non-sparse domain (such as tensor regression \citep{chen2016non,rauhut2017low}) -- to the best of our knowledge, this is the first optimality result in both sparse and non-sparse low-rank tensor regressions.

The above theoretical analyses are non-trivial due to the non-convexity of the empirical risk function, and the need to develop some new high-order sub-Gaussian concentration inequalities. Specifically, the empirical risk function in consideration satisfies neither restricted strong convexity (RSC) condition nor sparse eigenvalue (SE) condition in general. Thus, many previous results, such as the one based on local optima analysis \citep{WLZ14, LW15,chen2016non}, are not directly applicable. Moreover, the structure of cubic-sketching tensor leads to high-order products of sub-Gaussian random variables. Thus, the matrix analysis based on Hoeffding-type or Bernstein-type concentration inequality \citep{Cai2015,chen2015exact} will lead to sub-optimal statistical rate and sample complexity. This motivates us to develop new high-order concentration inequalities and sparse tensor-spectral-type bound, i.e., Lemmas \ref{cor:concentr_high_order} and \ref{lemma:tensor_spectral} in Section \ref{sec:high-order-concentration-inequality}. These new technical results are obtained based on the careful partial truncation of high-order products of sub-Gaussian random variables and the argument of bounded $\psi_{\alpha}$-norm \citep{ALPT2011}, and may be of independent interest.

A related line of research is low-rank matrix estimation in the literature, e.g., the spectral method and nuclear norm minimization \citep{candes2009exact,keshavan2009matrix,koltchinskii2011nuclear}.  
%as the convex implementation and relaxation of rank-constraint optimization. 
However, our cubic sketching model is by-no-means a simple extension from matrix estimation problems. %with rank-one projections \citep{Cai2015, chen2015exact}. 
In general, many related concepts or methods for matrix data, such as singular value decomposition, are problematic to apply in the tensor framework \citep{richard2014statistical,zhang2017tensor}. It is also found that simple unfolding or matricizing of tensors may lead to suboptimal results due to the loss of structural information \citep{Mu14}. Technically, the tensor nuclear norm is NP-hard to even approximate \citep{yuan2016tensor,yuan2017incoherent,friedland2017nuclear}, and thus the method to handle tensor low-rankness is particularly different from the matrix. 
%Additionally, \cite{raskutti2015convex} proposed a general theory for convex tensor regression but lack of efficient algorithm. \cite{chen2016non} proposed a non-convex projected gradient descent for tensor regression based on restricted strong convexity assumption. As we will discuss later, such a condition may not hold in our cubic sketchings framework. %Therefore, we are in need of new methods for tensor estimation based on cubic-sketchings. 



%In addition to symmetric cubic sketchings and estimation for symmetric tensors {\red (you need to mention in the beginning that our discussion first focus on symmetric case, rather than point this out by the end of introduction section.)}, the results can be further extended to non-symmetric cubic sketchings. Unlike symmetric tensor estimator, the minimization of non-symmetric empirical risk function is a triconvex optimization problem. This motivates us to implement the alternatively update in the thresholded gradient descent step. Moreover, our theoretical analysis guarantees the global convergence of this triconvex optimization problem as well as the optimal statistical rate. %{\red (any other novelty beyond the symmetric case?)}


%Although the current presentation is limited to the sparse third-order tensor estimation, the newly developed methodology and theoretical results can be further extended to non-sparse or higher order tensors by slight modifications (see Sections \ref{sec:main-theoretical} and \ref{sec:discussion} for more details). %{\red (Again, this should be mentioned in the beginning of introduction section.)} 
%Another notable feature of our framework lies on the potential extension to non-Gaussian sketchings with bounded $\psi_{\alpha}$-norm. Those two extensions take advantage of the higher-order Stein's identity and novel concentration results. %{\red (this part can be merged with the paragraph on technical tools. )} 

The rest of the paper is organized as follows. Section \ref{sec:prelim} provides preliminaries on notation and basic knowledge of tensor data. A two-stage method for symmetric tensor estimation is proposed in Section \ref{sec:symmetric}, with the corresponding theoretical analysis (in terms of upper and lower bounds) given in Section \ref{sec:theory-symmetric}. A concrete application to  high-order interaction effect models is described in Section \ref{sec:interaction}. The non-symmetric tensor estimation model is introduced and discussed in Section \ref{sec:non-symmetrc}. Numerical analysis is provided in Section \ref{sec:simu} to support the proposed procedure and theoretical results of this paper. Section \ref{sec:discussion} discusses extensions to higher-order tensors. The proofs of technical results are given in Section \ref{sec:proof} and supplementary materials.

\section{Preliminary}\label{sec:prelim}
Throughout the paper, vector, matrix, and tensor are denoted by boldface lower-case letters (e.g., $\bx, \by$), boldface upper-case letters (e.g., $\bX, \bY$), and script letters (e.g., $\cX, \cY$), respectively. %For a vector $\bx\in\mathbb R^p$ and a subset $A\subset \{1,\ldots, p\}$, we denote $\bx_{A}\in \mathbb R^p$ by keeping the coordinates of $\bx$ with indices in $A$ unchanged, while changing all other entries to zero.  
For any set $A$, let $|A|$ be the cardinality. The $\diag(\bx)$ is a diagonal matrix generated by $\bx$. For two vectors $\bx$ and $\by$, $\bx\circ\by$ is the outer product. Define $\|\bx\|_q:=(|x_1|^q+\cdots+|x_p|^q)^{1/q}$. We also define the $l_0$ quasi-norm by $\|\bx\|_0 = \#\{j:x_j\neq 0\}$ and $l_{\infty}$ norm by $\max_{1\leq j \leq p}|x_j|$. Denote the set $\{1,2,\ldots, n\}$ by $[n]$. Let $\be_j$ be the canonical vectors, whose $j$-th entry equals to 1 and all other entries equal to zero. %$\be_j:=(\underbrace{0,\ldots,0}_{j-1},1,\underbrace{0,\ldots,0}_{p-j})^\top$. 
For any two sequences $\{a_n\}_{n=1}^\infty, \{b_n\}_{n=1}^\infty$, we say $a_n = \cO(b_n)$ if there exists some positive constant $C_0$ and sufficiently large $n$ such that $a_n\leq C_0b_n$. We also write $a_n\asymp b_n$ if there exists $C, c>0$ such that $ca_n\leq b_n \leq Ca_n$ for all $n\geq 1$. Additionally, $C_1,C_2,\ldots,c_1,c_2,\ldots$ are generic constants, whose actual values may be different from line to line. 

We next introduce notations and operations on the matrix. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Matrix Notations}\label{sec:notation-matrix}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
For matrices $\bA = [\ba_1,\ldots, \ba_J]\in \mathbb R^{I\times J}$ and $\bB = [\bb_1,\ldots, \bb_L]\in \mathbb R^{K\times L}$, the \emph{Kronecker product} is defined as a $(IK)$-by-$(JL)$ matrix $\bA \otimes \bB = [\ba_1\otimes \bB ~ \cdots \ba_J \otimes \bB]$, where $\ba_j\otimes \bB=(a_{j1}\bB^{\top}, \ldots, a_{jI}\bB^{\top})^{\top}$.
%\begin{gather*}
%	\bA \circ \bB  = 
%	\begin{pmatrix} 
%		a_{11}\bB &\cdots&a_{1J}\bB \\ 
%		\vdots&\ddots&\vdots\\
%		a_{I1}\bB&\cdots&a_{IJ}\bB
%	\end{pmatrix}.
%\end{gather*}
%Note that when $\bA$ and $\bB$ are vectors, \emph{Kronecker product} is the same as the vector outer product. 
If $\bA$ and $\bB$ have the same number of columns $J=L$, the \emph{Khatri-Rao product} is defined as $\bA \odot \bB = [\ba_1\circ \bb_1, \ba_2\circ \bb_2, \cdots, \ba_J\circ \bb_J] \in \mathbb{R}^{IK \times J}.$ %Here, ``$\circ$" is the out-product between vectors/matrices. 
%{\red (do we need to explain the operator $\circ$? I think $\circ$ is not vector outer product here. In Kolda and Bader (2009), they use $\otimes$. $$\ba\otimes \bb = (a_1b_1, a_1b_2, \ldots a_1b_K, \ldots, a_Ib_1, \ldots, a_Ib_K)\in\mathbb R^{IK\times 1}.$$) }
%where $\{\ba_k\}_{k=1}^K$, $\{\bb_k\}_{k=1}^K$ are column vectors of $\bA$ and $\bB$. The \emph{Khatri–Rao product} is the ``matching columnwise" \emph{Kronecker product}.
If the matrices $\bA$ and $\bB$ are of the same dimension, the \emph{Hadamard product} is their element-wise matrix product, such that $(\bA * \bB)_{ij} = \bA_{ij}\cdot \bB_{ij}$.
%\begin{gather*}
%	\bA * \bB  = 
%	\begin{pmatrix} 
%		a_{11}b_{11} &\cdots&a_{1J}b_{1J} \\ 
%		\vdots&\ddots&\vdots\\
%		a_{I1}b_{I1}&\cdots&a_{IJ}b_{IJ}
%	\end{pmatrix} \in \mathbb{R}^{I\times J}.
%\end{gather*}
For matrix $\bX = [\bx_1 \cdots \bx_n]\in \mathbb R^{m\times n}$, we also denote the vectorization $\text{vec}(\bX) = (\bx_1^{\top}, \ldots, \bx_n^{\top})\in\mathbb R^{1\times mn}$ and column-wise $\ell_2$ norms as $\text{Norm}(\bX)=(\|\bx_1\|_2,\ldots, \|\bx_n\|_2)\in\mathbb R^{1 \times n}$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Tensor Notations}\label{sec:notation-tensor}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In the end, we focus on tensor notation and relevant operations. Interested readers are referred to \cite{kolda2009} for more details. Suppose  $\cX\in\mathbb R^{p_1\times p_2\times p_3}$ is an order-3 tensor, %A third-order tensor means a array along three directions. 
then the $(i, j, k)$-th element of $\cX$ is denoted by $[\cX]_{ijk}$. The successive tensor multiplication with vectors $\bu\in\mathbb R^{p_2}$, $\bv\in\mathbb R^{p_3}$ is denoted by $\cX\times_2 \bu \times_3\bv = \sum_{j\in[p_2], l\in[p_3]}u_j v_l \cX_{[:,j,l]}\in \mathbb R^{p_1}.$ We say $\cX \in \mathbb{R}^{p_1\times p_2\times p_3}$ is \emph{rank-one} if it can be written as the outer product of three vectors, i.e., $\cX = \bx_1 \circ \bx_2 \circ \bx_3$ or $[\cX]_{ijk} = x_{1i}x_{2j}x_{3k}$ for all $i, j, k$. Here ``$\circ$" represents the vector outer product. %This means that each element of the tensor is the product of the corresponding vector elements, i.e. $[\cX]_{ijk} = x_{1i}x_{2j}x_{3k}$. 
$\cX$ is symmetric if $[\cX]_{ijk} = [\cX]_{ikj} = [\cX]_{jik} = [\cX]_{jki} = [\cX]_{kij} = [\cX]_{kji}$ for all $i, j ,k$. Rank-one tensor is symmetric if and only if it can be decomposed as $\bx\circ \bx\circ \bx$ for some vector $\bx$. 

More generally, we may decompose a tensor as the sum of rank one tensors as follows,
\begin{equation}\label{eq:CP-decomposition}
\cX = \sum_{k=1}^K \eta_k\bx_{1k}\circ \bx_{2k} \circ \bx_{3k},
\end{equation} 
where $\eta_k\in \mathbb{R}, \bx_{1k}\in \mathbb{S}^{p_1-1}, \bx_{2k}\in \mathbb{S}^{p_2-1}, \bx_{3k}\in \mathbb{S}^{p_3-1}$.
This is the so-called CANDECOMP/PARAFAC, or CP decomposition \citep{kolda2009} with CP-rank being defined as the minimum number $K$ such that \eqref{eq:CP-decomposition} holds.   $\{\bx_{1k}\}_{k=1}^K, \{\bx_{2k}\}_{k=1}^K, \{\bx_{3k}\}_{k=1}^K$ are called \emph{factors} along first, second and third mode. Note that factors are normalized as unit vectors to guarantee the uniqueness of decomposition, and $\boldsymbol{\eta} = \{\eta_1, \ldots, \eta_K\}$ plays an analogous role of singular values in matrix value decomposition here. %{\red (I feel this paragraph should be moved to introduction section since it clearly defines what is low rank and sparsity in our mind.)}
%$$ \cX = \sum_{k=1}^K \eta_k\bx_{1k}\circ \bx_{2k} \circ \bx_{3k}.$$

Several tensor norms also need to be introduced. The tensor Frobenius norm and tensor spectral norm are defined respectively as
\begin{equation}\label{def:tensor_spectral_norm}
\|\cX\|_{F} = \sqrt{\sum_{i=1}^{p_1}\sum_{j=1}^{p_2}\sum_{k=1}^{p_3}\cX_{ijk}^2}, \ \|\cX\|_{op}:=\sup_{\bu\in\mathbb R^{p_1},\bv\in\mathbb R^{p_2},\bw\in\mathbb R^{p_3}}\frac{|\langle\cX, \bu\circ\bv\circ\bw\rangle|}{\|\bu\|_2\|\bv\|_2\|\bw\|_2},
\end{equation}
where $\langle\cX,\cY \rangle = \sum_{i,j,k} \cX_{ijk}\cY_{ijk}$. Clearly, $\|\cX\|_F^2 = \langle\cX,\cX\rangle$. We also consider the following sparse tensor spectral norm, 
\begin{equation}\label{def:sparse_spectral}
\|\cX\|_{s} := \sup_{\substack{\|\ba\|=\|\bb\|=\|\bc\|=1 \\ \max\{\|\ba\|_0,\|\bb\|_0, \|\bc\|_0\}\leq s}}\big|\langle\cX, \ba\circ\bb\circ\bc\rangle\big|.
\end{equation}
%This norm is used to quantify the perturbation error in a sparse scenario, and will be used during our perturbation error analysis. 
By definition, $\|\cX\|_s\leq \|\cX\|_{op}$. Suppose $\cX = \bx_1\circ \bx_2\circ \bx_3$ and $\cY = \by_1\circ \by_2 \circ \by_3$ are two rank-one tensors, then it is easy to check that
$\|\cX\|_{F} = \|\bx_1\|_2\|\bx_2\|_2\|\bx_3\|_2$ and $\langle\cX, \cY\rangle = (\bx_1^{\top}\by_1)(\bx_2^{\top}\by_2)(\bx_3^{\top}\by_3)$. %where $\|\cE\|_{op}$ is the tensor spectral norm defined in \eqref{def:tensor_spectral_norm}. 

%\Botao{Need proof?} {\blue It doesn't hurt to have a proof in the Appendix. If you don't want to do it, it is also fine.}
%\begin{proposition}
%	If both $\cA$ and $\cB$ is PARAFAC rank-one, we can have a simplified form
%	\begin{eqnarray*}
%		\langle\ba_1\circ\ba_2\circ\ba_3, \bb_1\circ\bb_2\circ\bb_3\rangle=(\ba_1^{\top}\bb_1)(\ba_2^{\top}\bb_2)(\ba_3^{\top}\bb_3).
%	\end{eqnarray*}
%\end{proposition}

==> t-cubic-sketch2-symmetry.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Symmetric Tensor Estimation via Cubic Sketchings}\label{sec:symmetric}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this section, we focus on the estimation of sparse and low-rank symmetric tensors,
\begin{equation}\label{eq:model}
y_i = \big\langle\mT^*, \mX_i \big\rangle+\epsilon_i, \quad \mX_i = \bx_i\circ \bx_i\circ \bx_i\in \mathbb R^{p\times p\times p}, \quad i=1,\ldots,n,
\end{equation}
 where $\bx_i$ are random vectors with i.i.d. standard normal entries. As previously discussed, the tensor parameter $\mT^*$ often satisfies certain low-dimensional structures in practice, among which the factor-wise sparsity and low-rankness \citep{raskutti2015convex} commonly appear. We thus assume $\mT^*$ is CP rank-$K$ for $K \ll p$ and the corresponding factors are sparse,
\begin{equation}\label{eq:mT_low-rank}
	\begin{split}
	\mT^* = \sum_{k=1}^K \eta_k^*\bbeta_{k}^*\circ\bbeta_{k}^*\circ\bbeta_{k}^*, \quad\text{with} \quad \|\bbeta_k^*\|_2 = 1, \|\bbeta_k^*\|_0\leq s, \forall k\in [K].
	\end{split}
\end{equation}
The CP low-rankness has been widely assumed in literature for its nice scalability and simple formulation \citep{li2010tensor, li2017parsimonious, SL17}. Different from the matrix factor analysis, we do not assume the tensor factors $\bbeta_k^*$ here are orthogonal. On the other hand, since the low-rank tensor estimation is NP-hard in general \citep{hillar2013most}, we will introduce an incoherence condition in the forthcoming Condition \ref{con:incoherence_sym} to ensure that the correlation among different factors $\bbeta_k^*$ is not too strong. Such a condition has been used in recent literature on tensor data analysis \citep{anandkumar2014tensor}, compressed sensing \citep{donoho2006compressed}, matrix decomposition \citep{chandrasekaran2011rank}, and dictionary learning \citep{arora2014new}. %The formal statement is provided in the forthcoming Condition \ref{con:incoherence_sym}.


%{\red where $\cZ$ is a small remainder term in terms of tensor spectral norm. CP-low-rankness assumption is widely considered in tensor literatures. Most of Past works on tensor regression have focused on the case of exact CP low-rankness. Here, we consider a more general setting of approximately CP low-rank tensor, including the exact setting as a particular case. }
%Here the CP-rank $K$ is typically much smaller than the dimension $p$. 
%We also assume that the factor vectors $\{\bbeta_k^*\}_{k=1}^K$ are sparse, in the sense that the number of nonzero coefficients is relatively small. Specifically, we assume 
%In this section, we focus on the estimation of low-rank symmetric tensor model \eqref{eq:model} and \eqref{eq:mT_low-rank}. 

Based on observations $\{y_i, \mX_i\}_{i=1}^n$, we propose to estimate $\mT^*$ via minimizing the empirical squared loss since the close-form gradient provides computational convenience,
\begin{equation}\label{eq:empirical risk minimization}
\hat{\mT} = \argmin_{\mT}\mathcal{L}(\mT)\quad \text{subject to $\mT$ is sparse and low-rank},
\end{equation} 
where
\begin{equation}\label{eq:L_s-T}
\begin{split}
\cL(\mT) & = \mathcal{L}\left(\eta_k, \bbeta_1, \ldots, \bbeta_K\right) = \frac{1}{n}\sum_{i=1}^n \left(y_i - \langle\mT, \mX_i\rangle\right)^2\\
&=  \frac{1}{n}\sum_{i=1}^n\left(y_i - \sum_{k=1}^K\eta_k\left(\bx_i^\top \bbeta_k\right)^3\right)^2. %\ \text{subject to} \ \mT \ \text{is sparse and low-rank}.
\end{split}
\end{equation}
%The subscript ``$s$" here corresponds symmetric tensor. %As being an non-convex optimization problem, it is difficult to find the exact solution to \eqref{eq:L_s-T}. %Rather than finding a convex relaxation, which is typically NP-hard \citep{hillar2013most}, we focus on the non-convex alternative. 
%Directly plugging in the CP-decomposition form \ref{eq:mT_low-rank}, the empirical risk function takes the form of 
%Surprisingly, the CP-decomposition form matches the cubic-sketching perfectly as both of them contain the rank-one structure. 
%By the property of tensor inner product, cubic-sketching can sketch the tensor by factor-wise
%\begin{equation*}
%\sum_{k=1}^K \eta_k\big\langle\bbeta_{k}\circ\bbeta_{k}\circ\bbeta_{k},  \bx_i\circ \bx_i\circ \bx_i\big\rangle = \sum_{k=1}^K\eta_k(\bx_i^{\top}\bbeta_k)^3.
%\end{equation*}
%It could output us a reduced and nice form of empirical risk function. 
Equivalently, \eqref{eq:empirical risk minimization} can be written as,
\begin{equation}\label{eqn:risk_function_sym}
\begin{split}
&\min_{\eta_k, \bbeta_k} \frac{1}{n}\sum_{i=1}^n\Big(y_i-\sum_{k=1}^K\eta_k(\bx_i^{\top}\bbeta_k)^3\Big)^2, \\
&\text{s.t.} \  \|\bbeta_k\|_2 = 1, \|\bbeta_k\|_0\leq s, \ \text{for} \ k\in[K].
\end{split}
\end{equation} 
Clearly, \eqref{eqn:risk_function_sym} is a non-convex optimization problem. To solve it, we propose a two-stage method as described in the next two subsections.
%Next, we introduce the thresholded gradient descent recovery procedure and provide the corresponding theoretical analysis for the symmetric tensor recovery with cubic sketchings in Sections \ref{sec:procedure-symmetric} and \ref{sec:theory-symmetric}, respectively.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Initialization}\label{sec:procedure-symmetric}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Due to the non-convex optimization  \eqref{eqn:risk_function_sym}, a straightforward implementation of many local search algorithms, such as gradient descent and alternating minimization, may easily get trapped into local optimums and obtain sub-optimal statistical performances. Inspired by recent advances of spectral method (e.g., EM algorithm \citep{zhang2016spectral}, phase retrieval \citep{CLM16}, and tensor SVD \citep{zhang2017tensor}), we propose to evaluate an initial estimate $\{\eta_k^{(0)}, \bbeta_k^{(0)}\}$ via the method of moment and sparse tensor decomposition (a variant of high-order spectral method) in the following Steps 1 and 2, respectively. The pseudo-code is given in Algorithm \ref{alg:overall_symmetric}.

\textbf{Step 1: Unbiased Empirical Moment Estimator.} Construct the empirical moment based estimator $\cT_s$,
	\begin{equation}
	\label{eqn:moment_tensor_sym}
	\begin{split}
	& \cT_s:= \frac{1}{6}\Big[\frac{1}{n}\sum_{i=1}^n y_i \bx_i\circ \bx_i\circ \bx_i \\
	&- \sum_{j=1}^p\Big(\bdm_1\circ \be_j\circ \be_j+ \be_j\circ \bdm_1 \circ \be_j+\be_j\circ \be_j\circ \bdm_1\Big)\Big],\\
	& \text{where}\ \bdm_1 := \frac{1}{n}\sum_{i=1}^n y_i\bx_i,\ \be_j \ \text{is the canonical vector}.
	\end{split}
	\end{equation}
	~\\
	\noindent  As will be shown in Lemma \ref{lemma:moment_symmetric}, $\cT_s$ is an unbiased estimator of $\mT^\ast$. The construction of \eqref{eqn:moment_tensor_sym} is motivated by high-order Stein's identity (\cite{janzamin2014score}; also see Theorem \ref{thm:steins_higher} for a complete statement). Intuitively speaking, based on the third-order score function for a Gaussian random vector $\bx$: $\cS_3(\bx) = \bx\circ \bx\circ \bx - \sum_{j=1}^p(\bx\circ \be_j\circ \be_j+ \be_j\circ \bx \circ \be_j+\be_j\circ \be_j\circ \bx)$, we can construct the unbiased estimator of $\mT^*$ by properly choosing a continuously differentiable function in high-order Stein's identity. See the proof of Lemma \ref{lemma:moment_symmetric} for more details.
 %The initialization for matrix estimation has been justified similarly through second-order Stein's identity in \cite{yang2017stein}. 
	%Due to the unbiaseness of $\mT^*$, the original problem can be reformatted to a version of tensor denoising:
	%\begin{eqnarray}
	%\label{eqn:denoising_model}
	%\cT_s = \mT^*+\cE, \quad\text{where} \quad \cE = \cT_s - \mathbb E(\cT_s).
	%\end{eqnarray}
	%\begin{Remark}
	%The construction of \eqref{eqn:moment_tensor_sym} is motivated by high-order Stein's identity (\cite{janzamin2014score}; also see Theorem \ref{thm:steins_higher} for a complete statement). Intuitively speaking, based on the third-order score function for a Gaussian random vector $\bx$: $\cS_3(\bx) = \bx\circ \bx\circ \bx - \sum_{j=1}^p(\bx\circ \be_j\circ \be_j+ \be_j\circ \bx \circ \be_j+\be_j\circ \be_j\circ \bx)$, we can construct an unbiased estimator for $\mT^*$ by properly choosing a continuously differentiable function in high-order Stein's identity. See the proof of Lemma \ref{lemma:moment_symmetric} more detailed explanations.
	%\end{Remark}
	
\textbf{Step 2: Sparse Tensor Decomposition.}  The method of moment estimator obtained in Step 1 provides an initial estimate for tensor $\mT^*$. Then we further obtain good initialization for the factors $\{\eta_k^{(0)}, \bbeta_k^{(0)}\}$ via truncation and alternating rank-1 power iterations \citep{AGJ14,Sun2016},
	$$\cT_s \approx \sum_{k=1}^K \eta_k^{(0)}\bbeta_{k}^{(0)}\circ \bbeta_{k}^{(0)}\circ \bbeta_{k}^{(0)}.$$ 
	%Following the idea of \cite{AGJ14,Sun2016}, 
	%We apply truncation and alternating rank-1 power iterations to construct the sparse initial estimate. 
	 Note that the tensor power iterations recover one rank-1 component per time. To identify all rank-1 components, we generate a large number of different initialization vectors at first, implement a clustering step, and choose the centroids as the estimates in the initialization stage. This scheme originally appears in tensor decomposition literature \citep{anandkumar2014tensor, AGJ14}, although our problem setting and proof techniques are very different. This procedure is also very different from the matrix setting since the rank-1 component in singular value decomposition is mutually orthogonal, but we do not enforce the exact orthogonality here for $\mT^*$.
	
	More specifically, we firstly choose a large integer $M \gg K$ and generate $M$ starting vectors $\{\bb_m^{(0)}\}_{m=1}^M \in\mathbb{R}^p$ through sparse SVD as described in Algorithm \ref{alg:sparse_svd_sym}. Then for each $\bb_m^{(0)}$, we apply the following truncated power update:
	$$
	\tilde{\bb}_{m}^{(l+1)} = \frac{\cT_s\times_2\bb_{m}^{(l)}\times_3 \bb_{m}^{(l)}}{\|\cT_s\times_2\bb_{m}^{(l)}\times_3 \bb_{m}^{(l)}\|_2}, \quad
\bb_{m}^{(l+1)} =\frac{T_d(\tilde{\bb}_m^{(l+1)})}{\|T_d(\tilde{\bb}_m^{(l+1)})\|_2},\quad l=0,\ldots, 
$$
	 where $\times_2, \times_3$ are tensor multiplication operators defined in Section \ref{sec:prelim} and $T_d(\bx)\in \mathbb{R}^p$ is a truncation operator that sets all but the largest $d$ entries in absolute values to zero for any vector $\bx \in \mathbb{R}^p$. It is noteworthy that the symmetry of $\cT_s$ implies
\begin{equation*}
    \cT_s\times_2\bb_{m}^{(l)}\times_3 \bb_{m}^{(l)} = \cT_s\times_1\bb_{m}^{(l)}\times_3 \bb_{m}^{(l)}= \cT_s\times_1\bb_{m}^{(l)}\times_2 \bb_{m}^{(l)}.
\end{equation*}
This means the multiplications along different modes are the same. We run power iterations till its convergence, and denote $\bb_m$ as the outcome. Finally, we apply $K$-means to partition $\{\bb_{m}\}_{m=1}^M$ into $K$ clusters, then let the centroids of the output clusters be $\{\bbeta_k^{(0)}\}_{k=1}^K$ and calculate $\eta_k^{(0)} = \cT_s\times_1\bbeta_{k}^{(0)}\times_2 \bbeta_{k}^{(0)}\times_3 \bbeta_{k}^{(0)}$ for $k\in [K]$. 

	
	\begin{algorithm}
	\small
	\caption{Initialization in cubic sketchings}
	\begin{algorithmic}[1]
		\REQUIRE response $\{y_i\}_{i=1}^n$, sketching vector $\{\bx_i\}_{i=1}^n$, truncation level $d$, rank $K$, stopping error $\epsilon = 10^{-4}$.
		\STATE  \textbf{Step 1:} Calculate the moment-based tensor $\cT_s$ as \eqref{eqn:moment_tensor_sym}.\\
		\STATE \textbf{Step 2:} 
		\STATE \quad\textbf{For} $m = 1$ \textbf{to} $L$ \\
		%\item option 1:  randomly initialize $\bbeta_{m}^{(0)}\in \cN(0, I_p)$.
		\quad\quad Generate $\bb_m^{(0)}$ through Algorithm \ref{alg:sparse_svd_sym}.
		
		\STATE \quad\quad \textbf{Repeat}  power update:
		\begin{eqnarray*}
			&&\tilde{\bb}_{m}^{(l+1)} = \frac{\cT_s\times_2\bb_{m}^{(l)}\times_3 \bb_{m}^{(l)}}{\|\cT_s\times_2\bb_{m}^{(l)}\times_3 \bb_{m}^{(l)}\|_2}, \quad \bb_{m}^{(l+1)} =\frac{T_d(\tilde{\bb}_m^{(l+1)})}{\|T_d(\tilde{\bb}_m^{(l+1)})\|_2}, \quad l = l+1.
		\end{eqnarray*}
		\STATE \quad\quad  \textbf{Until} $\|\bb_m^{(l+1)} - \bb_m^{(l)}\|_2\leq \epsilon$.
		\STATE \quad\textbf{End for.}
		\STATE \quad Perform $K$-means for $\{ \bb_{m}^{(l)}\}_{m=1}^M$. Denote the centroids of $K$ clusters by $\{\bbeta_{k}^{(0)}\}_{k=1}^K$.\\ \STATE \quad Calculate $\eta_k^{(0)} = \cT_s\times_1\bbeta_{k}^{(0)}\times_2 \bbeta_{k}^{(0)}\times_3 \bbeta_{k}^{(0)}, k\in[K].$\\
		\RETURN symmetric tensor estimator $\{\eta_k^{(0)}, \bbeta_k^{(0)}\}_{k=1}^K$.
	\end{algorithmic}
	\label{alg:overall_symmetric}
\end{algorithm}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%	
\subsection{Thresholded Gradient Descent}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

After obtaining a warm start in the first stage, we propose to apply the thresholding gradient descent to iteratively refine the solution to the non-convex optimization problem \eqref{eqn:risk_function_sym}. Specifically, denote $\bX = (\bx_1,\ldots, \bx_n) \in  \mathbb{R}^{p\times n}$, $\by = (y_1,\ldots, y_n)^{\top}\in \mathbb R^{n}$, $\boldsymbol{\eta} = (\eta_1, \ldots, \eta_K)^{\top}\in \mathbb R^{K}$ and $\bB = (\bbeta_1, \ldots, \bbeta_K)\in \mathbb{R}^{p\times K}$. Recall that $\cL(\bB, \boldsymbol{\eta}) = \cL(\mT)$, and hence let 
$$
\nabla_{\bB} \cL(\bB, \boldsymbol{\eta}) = (\nabla_{\bbeta_1} \cL(\bB, \boldsymbol{\eta})^{\top}, \ldots, \nabla_{\bbeta_K} \cL(\bB, \boldsymbol{\eta})^{\top}) \in \mathbb R^{1\times pK},
$$ 
be the gradient function with respect to $\bB$. Based on the detailed calculation in Lemma \ref{lemma:gradient_equivalence_sym}, $\nabla_{\bB} \cL(\bB, \boldsymbol{\eta})$ can be written as
\begin{equation}
\label{eqn:symmetric_gradient}
\nabla_{\bB} \cL(\bB, \boldsymbol{\eta}) = \frac{6}{n}[\{(\bB^{\top}\bX)^{\top}\}^3\boldsymbol{\eta} - \by]^{\top}[(\{(\bB^{\top}\bX)^{\top}\}^2\odot\boldsymbol{\eta}^{\top})^{\top} \odot \bX]^{\top},
\end{equation}
where $\{(\bB^\top \bX)^\top\}^3$ and $\{(\bB^\top \bX)^\top\}^2$ are entry-wise cubic and squared matrices of $(\bB^\top \bX)^\top$. Define $\varphi_h(x)$ as the thresholding function with a level $h$ that satisfies the following minimal assumptions:
\begin{equation}
\label{eqn:thresholding}
\left|\varphi_h(x)-x\right|\leq h, \forall x\in\mR, \ \text{and} \ \varphi_{h}(x) = 0 , \text{ when }|x|\leq h.
\end{equation}
Many widely used thresholding schemes, such as hard thresholding $H_h(x)=xI_{(|x|>h)}$, soft-thresholding $S_h(x)=\sign(x)\max(|x|-h, x)$, satisfy \eqref{eqn:thresholding}. With slightly abuse of notations, we further define the vector thresholding function as $\varphi_h(\bx) =(\varphi_h(x_1), \ldots, \varphi_h(x_p))$, for $\bx \in \mathbb{R}^p$. 

The initial estimates $\boldsymbol{\eta}^{(0)}$ and $\bB^{(0)}$ will be updated by thresholded gradient descent in two steps summarized in Algorithm	\ref{alg:overall_symmetric-gradient}. It is noteworthy that only $\bB$ is updated in the Step 3, while $\boldsymbol{\eta}$ will be updated in Step 4 after the update of $\bB$ is finished. 

\textbf{Step 3: Updating $\bB$ via Thresholded Gradient descent.} We update $\bB^{(t)}$ in each iteration step via thresholded gradient descent, 
\begin{equation}
\label{eqn:thresholed_update_sym}
\tv(\bB^{(t+1)}) = \varphi_{\frac{\mu\bh(\bB^{(t)})}{\phi}}(\tv(\bB^{(t)}) - \frac{\mu}{\phi}\nabla_{\bB} \cL(\bB^{(t)}, \boldsymbol{\eta}^{(0)})).
\end{equation}
 Here, 
\begin{itemize}
	\item $\mu$ is the step size and $\phi=\sum_{i=1}^ny_i^2/n$ serves as an approximation for $(\sum_{k=1}^K\eta_k^*)^2$ (see Lemma \ref{lemma:marginal_effect});
	\item $\bh(\bB)\in \mR^{1\times K}$ is the thresholding level defined as
	\begin{equation*}
	\label{eqn:threshold_level_symmetric}
	\bh(\bB) = \sqrt{\frac{4\log np}{n^2}}[\{\{(\bB^{\top}\bX)^{\top}\}^3\boldsymbol{\eta}^{(0)} - \by\}^2]^{\top}\{\{(\bB^{\top}\bX)^{\top}\}^2\odot\boldsymbol{\eta}^{(0)\top}\}^2.
	\end{equation*}
\end{itemize}

\textbf{Step 4: Updating $\boldsymbol{\eta}$ via Normalization.} We normalize each column of $\bB^{(T)}$ and estimate the weight parameter as
	\begin{equation}\label{eq:weight-update}
	\begin{split}
	&\hat{\bB} =(\hat{\bbeta}_1, \ldots, \hat{\bbeta}_K)^{\top} = \Big(\frac{\bbeta_1^{(T)}}{\|\bbeta_1^{(T)}\|_2}, \ldots, \frac{\bbeta_K^{(T)}}{\|\bbeta_K^{(T)}\|_2}\Big),\\
	&\hat{\boldsymbol{\eta}}=  (\hat{\eta}_1, \ldots, \hat{\eta}_K)^{\top} = \Big(\eta_1^{(0)}\|\bbeta_1^{(T)}\|_2^{3}, \ldots, \eta_K^{(0)}\|\bbeta_K^{(T)}\|_2^{3}\Big)^{\top}.
	\end{split}
	\end{equation}
   The final estimator for $\mT^\ast$ is
	$$
	\hat{\mT} = \sum_{k=1}^{K}\hat{\eta}_k\hat{\bbeta}_{k}\circ \hat{\bbeta}_{k}\circ \hat{\bbeta}_{k}.
	$$
	\begin{algorithm}
	\small
	\caption{Thresholded gradient descent in cubic sketchings}
	\begin{algorithmic}[1]
		\REQUIRE response $\{y_i\}_{i=1}^n$, sketching vector $\{\bx_i\}_{i=1}^n$, step size $\mu$, rank $K$, stopping error $\epsilon = 10^{-4}$, warm-start $\{\eta_k^{(0)}, \bbeta_k^{(0)}\}_{k=1}^K$.
		\STATE \textbf{Step 3:} Let $t=0$. \\
		\STATE \quad \textbf{Repeat} thresholded gradient descent
		\STATE \begin{itemize}
			\item Compute thresholding level $\bh(\bB)$.
			\item Calculate the thresholded gradient descent update 
			$$\tv(\bB^{(t+1)}) = \varphi_{\frac{\mu\bh(\bB)}{\phi}}\Big(\tv(\bB^{(t)}) -\frac{\mu}{\phi}\nabla_{\bB}\cL(\bB^{(t)}, \boldsymbol{\eta}^{(0)})\Big),$$ 
			where $\phi=\frac{1}{n}\sum_{i=1}^ny_i^2$. The detailed form of $\nabla_{\bB}\cL(\bB, \boldsymbol{\eta}^{(0)})$ refers to  \eqref{eqn:symmetric_gradient}.
		\end{itemize}
		\STATE \quad \textbf{Until} $\|\bB^{(T+1)} - \bB^{(T)}\|_F\leq \epsilon$. \\
		
		\STATE \textbf{Step 4:} Perform column-wise normalization and update the weight as \eqref{eq:weight-update}. Construct the final estimator $\hat{\mT} = \sum_{k=1}^{K}\hat{\eta}_k\hat{\bbeta}_{k}\circ \hat{\bbeta}_{k}\circ \hat{\bbeta}_{k}$.\\
		\RETURN symmetric tensor estimator $\hat{\mT}$.
	\end{algorithmic}
	\label{alg:overall_symmetric-gradient}
\end{algorithm}

\begin{algorithm}
	\caption{Sparse SVD}
	\begin{algorithmic}[1]
		\REQUIRE tensor $\cT_s$, cardinality parameter $d$.
		\STATE Compute $\tilde{\btheta}  =T_d(\btheta)$, where $\btheta\sim \cN(0,I_d)$.
		\STATE Calculate $\bu$ as the leading singular vector of $\cT_s\times_1\tilde{\btheta}$.
		\RETURN the sparse vector $T_d(\bu)/\|\bu\|_2$.
	\end{algorithmic}
	\label{alg:sparse_svd_sym}
\end{algorithm} 

\begin{comment}
\begin{remark}
Note that when we evaluate the gradient \eqref{eqn:symmetric_gradient}, there is no tensor inner product involved, which is typically the computational heaviest step in tensor problem. Due to the cubic sketching and low-rank assumption, the computational complexity of \eqref{eqn:symmetric_gradient} reduces from  $\cO(np^3)$  to $\cO(npK^2)$ with $K\ll p$. Moreover, the matrix form reformulation \eqref{eqn:symmetric_gradient} will also decrease the computational cost in most of software. {\red (Seems like a valid argument, but I don't quite get your point. Do you mean, the proposed algorithm is better in computation cost? If so, what algorithm are you comparing with? )}

{\blue Consider the gradient function in tensor regression model: 
	\begin{equation*}
	\nabla_{\bB}\cL(\bB) = \frac{2}{n}\sum_{i=1}^n\Big(\langle\bB, \cX_i \rangle-y_i\Big)\cX_i.
	\end{equation*}
	Evaluating it one time needs $\cO(np^3)$ operations. Our gradient function needs $\cO(npK^2)$ operations since we have less parameters to estimate. And here I also want to point out the matrix form gradient is not only for notation simplicity, but only facilitate the computation to some degrees. We avoid for loop in $n$ and $K$ in each iteration. For example, in R or python, running a for loop is slower than running a matrix multiplicationn. 
}


\end{remark}
\end{comment}


\begin{comment}
\begin{remark}[Adaptive Choice of Step Size]
	\label{remark:step_size}
	The selection of the step size $\mu$ plays crucial role in the proposed procedure. Following the suggestion in \cite{CLS15}, the larger the uncertainty or the noisier the estimate. This suggests that in the early iterations we should go forward a small step as the noise is large since we are not yet close to the solution. However, as the iterations count increases and we make progress, the size of the noise will also decrease and we can pick larger values for the step size. Empirically we use 
	\begin{eqnarray}
		\mu_t = \min(1-e^{-t/t_0}, \mu_{\max}),
	\end{eqnarray}
	where $t$ denotes the number of iteration and $t_0$ is a baseline value. Both $\mu_{\max}$ and $t_0$ will be specified in the simulation study.
%	As suggestion in \cite{CLS15}, the further away, the larger the uncertainty or the noisier the estimate. This suggests that in the early iterations we should go forward a small step as the noise is large since we are not yet close to the
%	solution. However, as the iterations count increases and we make progress, the size of the noise will also decrease and we can pick larger values for the step size. Empirically we use 
%	\begin{eqnarray}
%	\mu_t = \min(1-e^{-t/t_0}, \mu_{\max}),
%	\end{eqnarray}
%	where $t$ denotes the number of iteration and $t_0$ is a baseline value. Both $\mu_{\max}$ and $t_0$ will be specified in the simulation study.
\end{remark}
\end{comment}


\begin{Remark}[(Stochastic Thresholded Gradient descent)]
%In many cases, the summand risk functions have a simple form that enables inexpensive evaluations of the sum-function and the sum gradient. For example, in statistics, one-parameter exponential families allow economical function-evaluations and gradient-evaluations. However, in our cases, when the sample size and the dimension of tensor are enormous, evaluating the sum-gradient may still require expensive calculates of the gradients from all summand functions. This is due to the tensor product who needs $\cO(p^3)$ operators. To economize on the computational cost at every iteration, stochastic version of the block gradient descent algorithm samples a subset of summand functions at every step. This is very effective in the case of large-scale sparse tensor recovery problems.
Evaluating the gradient \eqref{eqn:symmetric_gradient} at each iteration requires $\cO(npK^2)$ operations, which is an issue when $n$ or $p$ is large. To economize the computational cost, a stochastic version of thresholded gradient descent algorithm can be easily carried out by sampling a subset of summand functions \eqref{eqn:symmetric_gradient} at each iteration. This will accelerate the procedure especially in the case of large-scale settings. Details could refer to Section \ref{subsec:stochas} in the supplementary materials. 
\end{Remark}


\section{Theoretical Analysis}\label{sec:theory-symmetric}


In this section, we establish the geometric convergence rate in optimization error and minimax optimal rate in statistical error of the proposed symmetric tensor estimator. %Given a provably initialization, we explicitly characterize the optimization and statistical error of each iterative update and show the optimal convergence rate. 
\subsection{Assumptions}
Conditions \ref{con:ident}-\ref{con:incoherence_sym} are on the true tensor parameter $\mT^*$ while Conditions \ref{con:noise}-\ref{con:sample} are on the measurement scheme. The first condition guarantees the model identifiability for CP-decomposition. 
\begin{Condition}[(Uniqueness of CP-decomposition)]\label{con:ident}
	The CP-decomposition form \eqref{eq:mT_low-rank} is unique in the sense that if there exists another CP-decomposition $\mT^* = \sum_{k=1}^{K'} \eta_k^{*'}\bbeta_{k}^{*'}\circ\bbeta_{k}^{*'}\circ\bbeta_{k}^{*'}$, it must have $K=K'$ and be invariant up to a permutation of $\{1,\ldots, K\}$.
\end{Condition}
For technical purpose, we introduce the following conditions to ensure that the CP-decomposition of $\mT^\ast$ has a regular form in the sense that the operator norm of $\mT^\ast$ can be bounded by the largest factor and all factors are in the same order. Similar assumptions were previously used in literature (e.g., \cite{zhou2013, Sun2016}).
\begin{Condition}[(Parameter space)]\label{con:parameter}
	The CP-decomposition $\mT^* = \sum_{k=1}^K \eta_k^*\bbeta_{k}^*\circ\bbeta_{k}^*\circ\bbeta_{k}^*$ satisfies
	\begin{equation}\label{eq:condition-parameter-space}
	\|\mT^*\|_{op}\leq C\eta_{\max}^*, \quad K=\cO(s), \quad \text{and}\quad R =\eta_{\max}^*/\eta_{\min}^*\leq C'
	\end{equation}
	for some absolute constants $C,C'$, where $\eta_{\min}^* = \min_{k}\eta_k^*$ and $\eta_{\max}^* = \max_{k}\eta_k^*$. Recall that $s$ is the sparsity for $\bbeta_k^*$.
\end{Condition}


 The performance of Step 2, i.e. the tensor decomposition for initialization, is crucial to the final estimation. However, as shown in the seminal work of \cite{hillar2013most}, the estimation of the low-rank tensor is NP-hard in general. Hence, we impose the following incoherence condition that is widely used in tensor decomposition literature \citep{AGJ14,Sun2016}. 
\begin{Condition}[(Parameter incoherence)]
	\label{con:incoherence_sym}
	The true tensor components are incoherent such that 
	\begin{eqnarray*}
		\Gamma:=\max_{1\leq k_1\neq k_2\leq K}|\langle\bbeta_{k_1}^*, \bbeta_{k_2}^*\rangle|\leq \min\{C^{''}K^{-\tfrac{3}{4}}R^{-1}, s^{-\tfrac{1}{2}}\},
	\end{eqnarray*}
where $R$ is the singular value ratio defined in \eqref{eq:condition-parameter-space} and $C^{''}$ is some small constant. 
\end{Condition}

\begin{remark}
The preceding incoherence condition has been widely used in different scenarios in recent high-dimensional research, such as compressed sensing \citep{donoho2006compressed}, matrix decomposition \citep{chandrasekaran2011rank}, and dictionary learning \citep{arora2014new}. It can also be viewed as a relaxation of orthogonality: if $\{\bbeta_1^*, \ldots, \bbeta_K^*\}$ are mutually orthogonal, $\Gamma$ equals zero. In addition, we can show from both theory (Lemma \ref{lemma:proof_incoherence} in the supplementary materials) and simulation (Section \ref{sec:simu}) that the low-rank tensor $\mT^*$ induced by \eqref{eq:mT_low-rank} satisfies the incoherence condition with high probability, if the component vectors $\bbeta_k^*$ are randomly generated, say from Gaussian distribution.
\end{remark}

We also introduce the following conditions on noise and sample complexity. 
\begin{Condition}[(Sub-exponential noise)]\label{con:noise}
	The noise $\{\epsilon_i\}_{i=1}^n$ are i.i.d. randomly generated with mean 0 and variance $\sigma^2$ satisfying $0<\sigma<C\sum_{k=1}^K\eta_k^*$. $(\epsilon_i/\sigma)$ is sub-exponential distributed, i.e., there exists constant $C_{\epsilon}>0$ such that $\|(\epsilon_i/\sigma)\|_{\psi_1} := \sup_{p\geq 1} p^{-1}(\mathbb{E}|\epsilon_i/\sigma|^p)^{1/p}\leq C_{\epsilon}$, and independent of $\{\mX_i\}_{i=1}^n$.
	%We assume the random noise $\{\epsilon_i\}_{i=1}^n$ follows a sub-exponential tail with parameter $\sigma$ satisfying $0<\sigma<\sum_{k=1}^K\eta_k^*/\log n$.  {\red (Could you state the specific form that $\epsilon_i$ satisfies? What is exactly ``sub-exponential tail"?)}
\end{Condition}

The sample complexity condition	is crucial for our algorithm, especially in the initialization stage. Ignoring any polylog factors, Condition \ref{con:sample} is even weaker than the sparse matrix estimation case $(n\gtrsim s^2)$ in \cite{CLM16}.
\begin{Condition}[(Sample complexity)] \label{con:sample}
	We assume a sufficient number of observations is observed, %The sample size requirement for sparse and low-rank tensor estimation is 
	\begin{equation*}
	n \geq C^{'''}K^2(s\log(ep/s))^{\tfrac{3}{2}}\log^4n.
	\end{equation*}
	%It is easy to check that this condition is further implied by $n\geq CK^2s^{3/2}\log^{6}p$ {\red (why to mention this sufficient condition? )}. 
\end{Condition}
%Ignoring any polylog factor, the minimum sample complexity of our algorithm to achieve an optimal statistical rate is $n\gtrsim s^{3/2$. This condition is crucial for the effectiveness of initialization stage. This sample complexity seems to be optimal in a board class of tensor problem. For a sparse and rank-one matrix estimation, \cite{CLM16} proposed a sub-optimal sample complexity $n\gtrsim s^{2}$ to obtain an optimal statistical rate. \cite{chen2015solving} claimed that solving random quadratic systems of equations is nearly as easy as solving linear systems. This may not be the case for tensor estimation since solving random cubic systems of equations is harder than solving linear systems from sample complexity perspective.

%As we will show in later theoretical analysis, if the sample size satisfies this condition, the proposed procedure yields a consistent estimation. %This outperforms many previous literatures on tensor regression. %\cite{raskutti2015convex,rauhut2017low}

\subsection{Main Theoretical Results}\label{sec:main-theoretical}

Our main Theorem \ref{thm:symmetric_main} shows that based on a good initializer, the output from the proposed thresholded gradient descent can achieve optimal statistical rate after sufficient iterations. Here, we define a contraction parameter 
$$0<\kappa = 1-32\mu K^{-2}R^{-\tfrac{8}{3}}<1,$$ and also denote $\cE_1 = 4K\eta_{\max}^{*\tfrac{2}{3}}\varepsilon_0^2$ and $\cE_2= C_0\eta_{\min}^{*-\tfrac{4}{3}}/16$ for some $C_0>0.$ 
\begin{Theorem}[(Statistical Error and Optimization Error)]
	\label{thm:symmetric_main}
    Suppose Conditions \ref{con:incoherence_sym}-\ref{con:sample} hold and the initial estimator $\{\bbeta_k^{(0)}, \eta_k^{(0)}\}_{k=1}^K$ satisfies 
    \begin{equation}\label{ineq:initial}
    \max_{1\leq k\leq K}\Big\{\big\|\bbeta_k^{(0)} - \bbeta_k^*\big\|_2, |\eta_k^{(0)} - \eta_k^*|\Big\}\lesssim K^{-1}, 
\end{equation}    	
with probability at least $1-\cO(1/n)$ and $|\supp(\bbeta_k^{(0)})|\lesssim s$. %with a truncation level $s \leq d \leq Cs$ 
Assume the step size $\mu\leq \mu_0$, where $\mu_0$ is defined in \eqref{eqn:mu_0}. Then, the output from the thresholded gradient descent update in \eqref{eqn:thresholed_update_sym} satisfies:
	\begin{itemize}
		\item For any $t=0,1,2,\ldots$, the factor-wise estimator satisfies
		\begin{eqnarray}\label{ineqn:error_bound}
			\sum_{k=1}^{K}\Big\|\sqrt[3]{\eta_k^{\scriptscriptstyle{(0)}}}\bbeta_k^{(t+1)} -\sqrt[3]{\eta_k^*}\bbeta_k^{*} \Big\|_2^2
			\leq \cE_1\kappa^t+\cE_2\frac{\sigma^2s\log p}{n},
		\end{eqnarray}
		with probability at least $1- \cO(tKs/n)$.
		\item When the total number of iterations is no smaller than
		\begin{eqnarray}\label{eqn:T^*}
			T^*=\Big(\log (\frac{n}{\sigma^2s \log p} \vee 1) + \log \frac{\cE_1}{\cE_2}\Big)/\log \kappa^{-1},
\end{eqnarray}
there exists a constant $C_1$ (independent of $K, s, p, n, \sigma^2$) s.t. the final estimator $\hat{\mT} = \sum_{k=1}^K\eta_k^{(0)}\bbeta_k^{(T^*)}\circ\bbeta_k^{(T^*)}\circ\bbeta_k^{(T^*)}$ is upper bounded by  
\begin{eqnarray}\label{ineqn:final_rate}
\Big\|\hat{\mT}-\mT^*\Big\|_F^2\leq \frac{C_1\sigma^2Ks\log p}{n},
\end{eqnarray}
with probability at least $1-\cO(T^*Ks/n)$.
	\end{itemize}
\end{Theorem}

\begin{Remark}
From \eqref{ineqn:error_bound},  the error bound can be decomposed into an optimization error $\cE_1\kappa^t$ (which decays with a geometric rate as iterations) and a statistical error $\cE_2\frac{\sigma^2s\log p}{n}$ (which does not decay as iterations). %Similar decomposition has been investigated in other non-convex problems such as Gaussian mixture model \citep{BWY15, wang2014}. Their technique is different from us since we make use of noiseless gradient as a bridge rather than the population-sample analysis in \cite{BWY15, wang2014}.
In particular, the convergence rate of the optimization error relies on the rank $K$ and the singular value ratio $R$ in the sense that the smaller $K$ or $R$, the faster convergence. Also from (\ref{ineqn:final_rate}), we note that in the special case that $\sigma =0$, $\hat{\mT}$ exactly recover $\mT^\ast$ with high probability.
%the error bound in \eqref{ineqn:error_bound} measures optimization error $\kappa^t$ for $0<\kappa<1$ and statistical error $\frac{\sigma^2s\log p}{n}$ jointly in each iteration. While the optimization error decays with a geometric rate, the statistical error remains the same when $t$ grows. Therefore, this enables us to provide a meaningful choice of the maximal number of iterations $T$ beyond which the optimization error is dominated by the statistical error such that the whole error bound is in the same order of the statistical error. %The probability term $1-4TK^2s/n$ will tend to one asymptotically since $T$ is of order logarithm in $n,s$.
\end{Remark}

%\begin{remark}
%	%There have been a number of existing results on the performance of  non-convex methods for non-convex learning problems. 
%	Recently, \cite{WLZ14} and \cite{LW15} considered the statistical and computational performance of proximal gradient method for a class of non-convex regularized M-estimator based on assumptions, such as restricted strong convexity (RSC), restricted isometry property (RIP) or sparse eigen value (SE). However, similarly as the arguments by \cite{Cai2015,CLS15,CLM16, Tu2016}, one can check that the empirical risk function \eqref{eqn:risk_function_sym} in cubic-sketching tensor recovery problem does not satisfy RSC, RIP or SE conditions in general. Thus these previous results cannot be directly applied here. 
%%As pointed out by \cite{CLS15,CLM16, Tu2016} in matrix recovery literature, the nonlinear-type empirical risk function \eqref{eqn:risk_function_sym} satisfies neither  restricted strong convexity (RSC) condition nor sparse eigenvalue (SE) condition in general. Previous approachs \citep{WLZ14, LW15} which measure the statistical performance of good local optima are not applicable since they heavily rely on RSC and SE conditions.
%\end{remark}

\begin{comment}
\begin{remark}
	In theory, we consider $\hat{\mT} = \sum_{k=1}^K\eta_k^{(0)}\bbeta_k^{(T)}\circ\bbeta_k^{(T)}\circ\bbeta_k^{(T)}$ with unnormalized updated factor, which is a slightly different than we did in Step three of Algorithm \ref{alg:overall_symmetric}. Note that this will not affect the final construction of $\hat{\mT}$. We assumed $\mT^*$ is exactly low-rank in the analysis for Theorem \ref{thm:main_symmetric}. Moreover, when $\mT^\ast$ is approximately low-rank, in the sense that $\mT^* = \sum_{k=1}^K \eta_k^*\bbeta_{k}^*\circ\bbeta_{k}^*\circ\bbeta_{k}^*+\Phi$ with some perturbation $\Phi$ with small amplitude, we can further derive similar upper bound guarantees for $\hat{\mT}$.
\end{remark}
\end{comment}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The next theorem shows that Steps 1 and 2 of Algorithm \ref{alg:overall_symmetric} provides a good initializer required in Theorem \ref{thm:symmetric_main}. %This intermediate result provides a key step in our theoretical analysis in Theorem \ref{thm:symmetric_main}. 
\begin{Theorem}[(Initialization Error)]
	\label{thm:initial_symmetric}
    Suppose the number of initializations $L \geq K^{C_3\gamma^{-4}}$, where $\gamma$ is a constant defined in \eqref{def:gamma}. Given that Conditions \ref{con:ident}-\ref{con:noise} hold, the initial estimator obtained from Steps 1-2 with a truncation level $s \leq d\leq Cs$ satisfies
	\begin{equation}\label{eqn:initial_rate}
	\max_{1\leq k \leq K}\Big\{\|\bbeta_{k}^{(0)}-\bbeta_{k}^*\|_2, |\eta_k^{(0)}-\eta_k^*|\Big\} \leq C_2KR\delta_{n,p,s} + \sqrt{K}\Gamma^2,
	\end{equation}
	and $|\supp(\bbeta_k^{(0)})|\lesssim s$ with probability at least $1-5/n$, where 
	\begin{equation}\label{eqn:initial_stat_rate}
	\delta_{n,p,s} = (\log n)^3\Big(\sqrt{\frac{s^3\log ^3(ep/s)}{n^2}} + \sqrt{\frac{s\log (ep/s)}{n}}\Big).
	\end{equation}
	Moreover, if the sample complexity condition \ref{con:sample} is satisfied, then the above bound satisfies \eqref{ineq:initial}.
\end{Theorem}
\begin{Remark}[(Interpretation of initialization error)]\label{rm:initialization error}
The upper bound of \eqref{eqn:initial_rate} consists of two terms, which corresponds to the approximation error of $\cT_s$ to $\mT^\ast$ and the incoherence condition of $\bbeta_{k}^\ast$'s, respectively. Especially, the former converges to zero as $n$ grows while the latter does not. %We can see no matter how large the sample size $n$ is, the sparse tensor decomposition cannot guarantee exact recovery since the model error does not disappear when $K>2$. Second, 
This indicates that the convergence rate of the initial estimate is significantly slower than that of the final estimate after iterative updates, unless 
$$n\gtrsim (s\log (ep/s))^2\quad \text{and}\quad \Gamma^2 \lesssim \sqrt{\frac{s\log(ep/s)}{nK}}.$$
More detailed numerical comparisons will be provided later in Section \ref{sec:simu}.
%there is an interesting trade-off between optimal statistical rate and minimum sample complexity in rate \eqref{eqn:initial_stat_rate}. Note that the second term of \eqref{eqn:initial_stat_rate} is essentially optimal statistical rate. However, only if the sample size $n\gtrsim (s\log (p/s))^2$, the second term will dominate \eqref{eqn:initial_stat_rate}. When $(s\log (p/s))^{3/2}\lesssim n\lesssim (s\log (p/s))^2$, the rate \eqref{eqn:initial_rate} will lead a suboptimal rate. Succeeded by thresholded gradient descent, we can obtain optimal rate with minimum sample complexity.
	
%The upper bound of \eqref{eqn:initial_rate} consists of two parts: one is sample error, which captures the empirical mean approximation performance, another is model error, which measures the complexity in decomposing the true tensor. First, no matter how large the sample size is, the sparse tensor decomposition cannot guarantee exact recovery since the model error does not disappear when $K>2$. Second, there is an interesting trade-off between optimal statistical rate and minimum sample complexity in rate \eqref{eqn:initial_stat_rate}. Note that the second term of \eqref{eqn:initial_stat_rate} is essentially optimal statistical rate. However, only if the sample size $n\gtrsim (s\log (p/s))^2$, the second term will dominate \eqref{eqn:initial_stat_rate}. When $(s\log (p/s))^{3/2}\lesssim n\lesssim (s\log (p/s))^2$, the rate \eqref{eqn:initial_rate} will lead a suboptimal rate. Succeeded by thresholded gradient descent, we can obtain optimal rate with minimum sample complexity.
\end{Remark}
The proof of Theorems \ref{thm:symmetric_main} and \ref{thm:initial_symmetric} are involved and postponed to Section \ref{subsec:proof_ini}-\ref{subsec:gradient-update-proof} in the supplementary materials. The combination of Theorems \ref{thm:symmetric_main} and \ref{thm:initial_symmetric} immediately yields the following upper bound for the final estimate as one main result in this paper.
\begin{Theorem}[(Upper Bound)]
	\label{thm:symmetric_upper_bound}
Suppose Conditions \ref{con:ident} -- \ref{con:sample} hold, $s\leq d\leq Cs$. After $T^*$ iterations, there exists a constant $C_1$ not depending on $K, s, p, n, \sigma^2$, such that the proposed procedure yields
\begin{eqnarray}\label{ineqn:final_rate_main}
\Big\|\hat{\mT}-\mT^*\Big\|_F^2\leq \frac{C_1\sigma^2Ks\log p}{n},
\end{eqnarray}
with probability at least $1-\cO(T^*Ks/n)$, where $T^*$ is defined in \eqref{eqn:T^*}.
%{\red (Could you derive the result in expectation? It is ok to further impose some reasonable conditions. The target is to prove)
%$$\mathbb{E}\Big\|\hat{\mT}-\mT^*\Big\|_F^2\leq \frac{C_1R\sigma^2Ks\log p}{n}.
%$$}
\end{Theorem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The above upper bound turns out to match with the minimax lower bound for a large class of sparse and low rank tensors.%Combining Theorems \ref{thm:symmetric_upper_bound} and \ref{th:lower_bound}, we can see that the proposed Algorithm \ref{alg:overall_symmetric} achieves minimax-optimal rate of convergence in terms of recovery as long as $\log p \asymp \log(p/s)$.
\begin{Theorem}[(Lower Bound)]
	\label{th:lower_bound}
	Consider the following class of sparse and low-rank tensors,
	\begin{equation}\label{eq:mathcal_F_symmetric}
	\mathcal{F}_{p, K, s} = \left\{\mT: \begin{array}{l}
	\mT = \sum_{k=1}^K\eta_k \bbeta_k\circ \bbeta_k\circ \bbeta_k, \|\bbeta_k\|_0 \leq s, \text{ for } k \in[K],\\ 
	\mT \ \text{satisfies Conditions \ref{con:ident},  \ref{con:parameter}, and \ref{con:incoherence_sym}}.
	\end{array}\right\}.
	\end{equation}
	Suppose that $\{\mX_i\}_{i=1}^n$ are i.i.d standard normal cubic sketchings with i.i.d. $N(0, \sigma^2)$ noise in  \eqref{eq:model}. We have the following lower bound result,
	\begin{equation*}
		\inf_{\tilde{\mT}}\sup_{\mT \in \mathcal{F}_{p, K, s}} \mathbb{E} \left\|\tilde{\mT} - \mT\right\|_F^2\geq c\sigma^2\frac{Ks \log(ep/s)}{n}.
	\end{equation*}
\end{Theorem}
The proof of Theorem \ref{th:lower_bound} is deferred to Section \ref{proof:thm_minimax} in the supplementary materials. Combining Theorem \ref{thm:symmetric_upper_bound} and Theorem \ref{th:lower_bound} together, we immediately obtain the following minimax-optimal rate for sparse and low-rank tensor estimation with cubic sketchings when $\log p \asymp \log (p /s)$:
	%Suppose we observe $n$ samples $\{y_i, \mX_i\}_{i=1}^n$ from symmetric tensor cubic skeching model \eqref{eq:model} \eqref{eq:mT_low-rank}, where $n= \cO((s\log p/s)^{\tfrac{3}{2}})$. %{\red Under regularity conditions presented in ... }, 
	%The estimator $\hat{\mT}$ achieves
	\begin{equation}\label{eqn:optimal_rate}
	\inf_{\tilde{\mT}}\sup_{\mT^* \in \mathcal{F}_{p, K, s}}\mathbb{E}\left\|\tilde{\mT} - \mT^*\right\|_F^2 \asymp \sigma^2\frac{Ks\log (p/s)}{n}.
	\end{equation}
The rate in \eqref{eqn:optimal_rate} sheds light upon the effect of dimension $p$, noise level $\sigma^2$, sparsity $s$, sample size $n$ and rank $K$ to the estimation performance.


\begin{Remark}[(Non-sparse low-rank tensor estimation via cubic-sketchings)]
	When the low-rank tensor $\mT^\ast$ is not necessarily sparse, i.e.,
	\begin{equation*}
	\mT^* \in \mathcal{F}_{p, K} = \left\{\mT: \begin{array}{l}
	\mT = \sum_{k=1}^K\eta_k \bbeta_k\circ \bbeta_k\circ \bbeta_k, \text{ for } k \in[K],\\ 
	\mT \ \text{satisfies Conditions \ref{con:ident}, \ref{con:parameter}, and \ref{con:incoherence_sym}}
	\end{array}\right\},
	\end{equation*}
	we can apply the proposed procedure with all the truncation/thresholding steps removed. If $n \geq \cO (p^{3/2})$, one can apply similar arguments of Theorems \ref{thm:symmetric_main}-\ref{thm:symmetric_upper_bound} to show that the output estimation $\hat{\mT}'$ satisfies
	\begin{equation}\label{eq:non-sparse-rate}
		\left\|\hat{\mT}' - \mT^*\right\|_F^2\lesssim \frac{\sigma^2 Kp}{n}.
	\end{equation}
	for any $\mT^* \in \mathcal{F}_{p, K}$ with high probability. Furthermore, similar arguments of Theorem \ref{th:lower_bound} imply that the rate in \eqref{eq:non-sparse-rate} is minimax optimal. %{\red (can we claim that (4.10) is also new?)}
\end{Remark}
	
\begin{Remark}[(Comparison with existing matrix results)]\label{rm:comparison-matrix-setting}
Our cubic sketching tensor results are not a direct extension of the existing matrix results. For example, \cite{chen2015exact,Cai2015} studied the low-rank matrix recovery based on rank-1 projections: $y_i = \bx_i^\top \bT \bx_i + \epsilon_i$ based on the convex nuclear norm minimization. The theoretical properties of their estimate are analyzed under a $\ell_1/\ell_2$-RIP or Restricted Uniform Boundedness (RUB) condition. %\cite{WLZ14} and \cite{LW15} considered the statistical and computational performance of proximal gradient method for a class of non-convex regularized M-estimator based on assumptions, such as restricted strong convexity (RSC), restricted isometry property (RIP) or sparse eigenvalue (SE). 
    However, tensor nuclear norm is computationally infeasible and following the arguments in \cite{CLS15,CLM16}, 
	one can check that our cubic sketching framework does not satisfy RIP or RUB conditions in general. Thus, these previous results cannot be directly applied.
	
 In addition, the analysis of gradient updates for the tensor case is significantly more complicated than the matrix case. First, we require high-order concentration inequalities for the tensor case since the cubic-sketching tensor leads to high-order products of sub-Gaussian random variables (see Section \ref{sec:high-order-concentration-inequality} for details). The necessity of high-order expansions in the analysis of gradient updates for the tensor case also significantly increases the hardness of the problem. To ensure the geometric convergence, we need much more subtle controls on the regularity conditions comparing to the ones in the matrix case \citep{CLS15}.

	
	%\cite{candes2013phaselift,CLS15,eldar2015sparse,CLM16} considered the phase retrieval, that one observes $y_i = |\langle \bu, \bbeta_i \rangle|^2 + \epsilon_i$ and aim to recover $\bu_i$ from $\{y_i, \bbeta_i\}_{i=1}^n$. To this end, \cite{CLS15,CLM16} proposed the gradient-descent-based Wirtinger flow minimization/ truncated Wirtinger flow minimization. In our cubic sketching tensor recovery framework, the cube structure within the empirical loss function \eqref{eqn:risk_function_sym} causes high-order form of Gaussian random variables. In this case, typical Hoeffding's or Berstein's concentration inequality used in \cite{Cai2015} and \cite{CLM16} lead to suboptimal statistical rate and sample complexity. 
\end{Remark}

%{\red ( To me, this remark may be merged into introduction section to show the previous techniques used in matrix case donot extend to tensor case easily. If that is the case, please remove this remark.)}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Key Lemmas: High-order Concentration Inequalities}\label{sec:high-order-concentration-inequality}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

As mentioned earlier, one major challenge for theoretical analysis of cubic sketching is to handle heavy tails of high-order Gaussian moments. One can only handle up-to second moments of sub-Gaussian random variables by directly applying the existing Hoeffding's or Bernstein's concentration inequalities. Rather, we need to develop the following two high-order concentration inequalities as technical tools: Lemma \ref{cor:concentr_high_order} characterizes the tail bounds for the sum of sub-Gaussian products, and Lemma \ref{lemma:tensor_spectral} provides the concentration inequalities for Gaussian cubic sketchings. The proofs of Lemma \ref{cor:concentr_high_order} and \ref{lemma:tensor_spectral} are given in Section \ref{subsec:concentration}.
% and may be of independent interest.  %which together characterize the concentration of high moments of sub-Gaussian random variables. 

%In particular, we first truncate the Gaussian high-order moments at a careful chosen level, then bound the $\psi_{\alpha}$ norm of these truncated random variables, and derive and the corresponding concentration result. %By the combination of truncation argument and the usage of $\psi_{\alpha}$-norm, we are able to provide optimal statistical rate and sample complexity. 

%In order to analyze the proposed procedure in Section \ref{sec:symmetric}, our first step is to carefully treat the unbiased estimator $\cT_s$, which is essentially a sixth moment tensor structure of Gaussian random variables. To this end, we develop the following two lemmas, which together characterize the concentration of high moments of sub-Gaussian random variables. These results serve as the key technical tools for the theoretical analysis, and may be of independent interests in other problems. 

%Lemma \ref{cor:concentr_high_order} provides a concentration inequality for the sum of products of sub-Gaussian random variables. 
\begin{Lemma}[(Concentration inequality for sum of  sub-Gaussian products)]\label{cor:concentr_high_order}	
	Suppose $\bX_i= (\bx_{1i}^{\top}, \ldots, \bx_{mi}^{\top})^{\top}\in \mathbb R^{m\times p}$, $i\in[n]$ are $n$ i.i.d  random matrices. Here, $\bx_{ij}$ is the $j$-th row of $\bX_i$ and suppose it is an isotropic sub-Gaussian vector. Then for any vectors $\ba = (a_1\ldots,a_n)\in\mathbb R^n$, $\{\bbeta_j\}_{j=1}^m\subseteq \mathbb R^{p}$, and $0<\delta<1$, we have
	\begin{equation*}
	\begin{split}
		&\Big|\sum_{i=1}^na_i\prod_{j=1}^m(\bx_{ij}^{\top}\bbeta_j)-\mathbb E\Big(\sum_{i=1}^na_i\prod_{j=1}^m(\bx_{ij}^{\top}\bbeta_j)\Big)\Big|\\
		&\leq C\prod_{j=1}^m\|\bbeta_j\|_2\Big(\|\ba\|_{\infty}(\log \delta^{-1})^{m/2}+\|\ba\|_2(\log \delta^{-1})^{1/2}\Big),
		\end{split}
	\end{equation*}
	with probability at least $1-\delta$ for some constant $C$. 
\end{Lemma}
	Note that in Lemma \ref{cor:concentr_high_order}, entries in each matrix $\bX_i$ are not necessarily independent even $\{\bX_i\}_{i=1}^n$ are independent matrices. Building on Lemma \ref{cor:concentr_high_order}, Lemma \ref{lemma:tensor_spectral} provides a generic spectral-type concentration inequality that can be used to quantify the approximation error for $\cT_s$ introduced in Step 1 of the proposed procedure. 
\begin{Lemma}[(Concentration inequality for Gaussian cubic sketchings)]
	\label{lemma:tensor_spectral}
	Suppose $\{\bx_{1i}\}_{i=1}^n \overset{iid}{\sim} \cN(0, \bI_{p_1})$, $\{\bx_{2i}\}_{i=1}^n\overset{iid}{\sim} \cN(0, \bI_{p_2})$, $\{\bx_{3i}\}_{i=1}^n \overset{iid}{\sim} \cN(0, \bI_{p_3})$, $\bbeta_1\in \mathbb R^{p_1}$, $\bbeta_2\in \mathbb R^{p_2}$, $\bbeta_3\in \mathbb R^{p_3}$ are fixed vectors. 
	\begin{itemize}
		\item Define $M_{\text{nsy}} = \frac{1}{n}\sum_{i=1}^n\langle \bx_{1i}\circ \bx_{2i}\circ \bx_{3i}, \bbeta_1\circ \bbeta_2\circ \bbeta_3\big\rangle\bx_{1i}\circ\bx_{2i}\circ\bx_{3i}$. Then $\mathbb{E}(M_{\text{nsy}}) = \bbeta_1\circ\bbeta_2 \circ\bbeta_3$, and
		\begin{equation*}
		\begin{split}
			&\Big\|M_{\text{nsy}} - \mathbb E(M_{\text{nsy}})\Big\|_s\\
			&\leq C(\log n)^3\Big(\sqrt{\frac{s^3\log^3 (ep/s)}{n^2}} + \sqrt{\frac{s\log (ep/s)}{n}}\Big)\|\bbeta_1\|_2\|\bbeta_2\|_2\|\bbeta_3\|_2,
			\end{split}
		\end{equation*}
		with probability at least $1-10/n^3$.
		\item Define $M_{\text{sym}} = \frac{1}{n}\sum_{i=1}^n\langle \bx_{1i}\circ \bx_{1i}\circ \bx_{1i}, \bbeta_1\circ \bbeta_1\circ \bbeta_1\big\rangle\bx_{1i}\circ\bx_{1i}\circ\bx_{1i}$. Then $\mathbb E(M_{\text{sym}})=6\bbeta_1\circ \bbeta_1 \circ \bbeta_1+3\sum_{m=1}^p(\bbeta_1\circ \be_m\circ \be_m + \be_m\circ \bbeta_1\circ\be_m + \be_m\circ \be_m\circ \bbeta_1)$, and
		\begin{equation*}
		\begin{split}
		&	\Big\|M_{\text{sym}} - \mathbb E(M_{\text{sym}})\Big\|_s\\
		&\leq  C(\log n)^3\Big(\sqrt{\frac{s^3\log^3 (ep/s)}{n^2}} + \sqrt{\frac{s\log (ep/s)}{n}}\Big)\|\bbeta_1\|_2^3,
			\end{split}
		\end{equation*}
		with probability at least $1-10/n^3$.
	\end{itemize}	
	Here, $C$ is an absolute constant and $\|\cdot\|_{s}$ is the sparse tensor spectral norm defined in \eqref{def:sparse_spectral}.
\end{Lemma}
Note that $M_{\text{sym}}$ is the major term in the unbiased empirical moment estimator $\cT_s$ in \eqref{eqn:moment_tensor_sym}, while $M_{\text{nsy}}$ corresponds to the non-symmetric unbiased empirical moment estimator $\cT$ that will be introduced later in \eqref{eq:moment_asy}. %{\red (It is helpful to discuss how to apply it. For example, link $M_{sym}$ to $\cT_s$. Also, point out that $M_{nsy}$ is for the non-symmetric case.)}

%The proof of Lemma \ref{lemma:tensor_spectral} is a combination of truncation argument, $\psi_{2/3}$-norm and $\varepsilon$-net on the discretized sparse set. %The extra $(\log n)^3$ is contributed by the truncation step. 
%To ensure that Lemma \ref{lemma:tensor_spectral} provides a non-trivial upper bound, it requires $n\geq C (s\log(p/s))^{\tfrac{3}{2}}$ for some large constant $C$. Only if $n\geq C(s\log (p/s))^2$, this spectral norm bound can achieve optimal statistical rate. 



==> t-cubic-sketch3-interaction.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Application to High-Order Interaction Effect Models}\label{sec:interaction}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this section, we estimate high-order interaction effect models in the cubic sketching framework. Specifically, we consider the following three-way interaction model
\begin{equation}\label{eq:interaction_model}
y_l  = \xi_0 +  \sum_{i=1}^p \xi_i z_{li}  + \sum_{i, j = 1}^{p} \gamma_{ij} z_{li}z_{lj} + \sum_{i,j,k = 1}^p \eta_{ijk} z_{li}z_{lj}z_{lk}+\epsilon_l, \quad l=1,\ldots, n.
\end{equation}
Here $\bxi$, $\bgamma$, and $\boldsymbol{\eta}$ are coefficients for main effect, pairwise interaction, and triple-wise interaction, respectively. Importantly, \eqref{eq:interaction_model} can be reformulated as the following tensor form (also see the left panel in Figure \ref{fig:illurstration})
\begin{equation}\label{eq:skeching}
y_l = \langle \cB, \bx_l \circ \bx_l \circ \bx_l\rangle + \epsilon_l,\quad l=1,\ldots, n,
\end{equation}
where $\bx_l = (1, \bz_l^\top)^\top \in \mathbb{R}^{p+1}$ and $\cB\in \mathbb{R}^{(p+1)\times (p+1)\times (p+1)}$ is a tensor parameter corresponding to coefficients in the following way:
\begin{equation}
\left\{\begin{array}{l}
\cB_{[0, 0, 0]} = \xi_0,\\ 
\cB_{[1:p, 1:p, 1:p]} = (\eta_{ijk})_{1\leq i,j,k\leq p}, \\
\cB_{[0, 1:p, 1:p]} = \cB_{[1:p, 0, 1:p]} = \cB_{[1:p, 1:p, 0]} = (\gamma_{ij}/3)_{1\leq i,j\leq p}, \\
\cB_{[0, 0, 1:p]} = \cB_{[0, 1:p, 0]} = \cB_{[1:p, 0, 0]} = (\xi_i/3)_{1\leq i \leq p}.
\end{array}\right.
\end{equation}



%\begin{eqnarray*}
%	Y_l &=& \beta_0+\underbrace{\beta_1X_1+\ldots+\beta_pX_p}_{\text{Main Effect}}+\underbrace{\beta_{1,1}X_1^2+\beta_{1,2}X_1X_2+\ldots+\beta_{p,p}X_p^2}_{\text{Two-way Interaction}}\\
%	&&+\underbrace{\beta_{1,1,1}X_1^3+\beta_{1,1,2}X_1^2X_2+\cdots+\beta_{p,p,p}X_p^3}_{\text{Three-way Interaction}} + \underbrace{\varepsilon}_{\text{noise}}, \quad l=1,\ldots, n.
%\end{eqnarray*}
%To improve the joint screening of all main and interaction effects, we utilize the tensor nature of the interactions terms and consider a reduced model.

%Let's define $\bX=(1, X_1, X_2,\ldots, X_p)$. Then we consider the symmetric tensor $\cX=\bX\circ\bX\circ\bX$. The model is
%\begin{eqnarray*}
%\mathbb E(Y|X)=\langle \cB,\bX\circ\bX\circ\bX\big \rangle.
%\end{eqnarray*}
%If $\cB$ is of rank-$K$, then
%\begin{eqnarray*}
%\mathbb E(Y|X)&=&\Big\langle \sum_{k=1}^K\eta_k\bbeta_k\circ\bbeta_k\circ\bbeta_k,\bX\circ\bX\circ\bX\Big \rangle\\
%&=& \sum_{k=1}^{K}\eta_k\big(\bX^{\top}\bbeta_k\big)^3 = \sum_{k=1}^{K}\eta_k\big(\beta_{k1}+\beta_{k2}X_1\ldots+\beta_{kp}X_p\big)^3.
%\end{eqnarray*}
%According to Multinomial Theorem,
%\begin{eqnarray*}
%\Big(x_1+x_2+\ldots+x_m\Big)^n=\sum_{k_1+k_2+\cdots+k_m=n}\binom{n}{k_1,k_2,\ldots,k_m}\prod_{t=1}^m x_t^{k_t}.
%\end{eqnarray*}

%Suppose $\bX = (1,X_1,X_2,\ldots, X_p)^{\top}$ and the tensor based interaction effect model can be rewritten as
%\begin{equation}
%Y = \langle\bB, \bX\circ \bX \circ\bX \rangle  + \varepsilon,
%\end{equation}
%where $\bB\in \mathbb{R}^{(p+1)\times(p+1)\times(p+1)}$ incorporate all intercept, main, two-way, and three-way effects:
%\begin{equation*}
%\begin{split}
%\left\{\begin{array}{ll}
%B_{[1,1,1]} = \beta_{0},\\
%B_{[2:(p+1),2:(p+1),2:(p+1)]} = (\beta_{i, j, k}/6)1≤i,j,k≤p,
% B[1,2:(p+1),2:(p+1)] = B[2:(p+1),1,2:(p+1)] = B[2:(p+1),2:(p+1),1] = (γij/3)1≤i,j≤p,  B[1,1,2:(p+1)] = B[1,2:(p+1),1] = B[2:(p+1),1,1] = (βi/3)1≤i≤p.
%\end{array}
%\right.
%\end{split}
%\end{equation*}

%As mentioned in \cite{Hung2016}, in modern biomedical research, it's reasonable to assume $\cB$ is highly sparse since only a small portion of the covariates contribute to $\by$. If only pairwise interactions are considered, the tensor $\cB$ is also likely to be low-rank while $\cB$ is sparse. Moreover, a rank-one tensor is sparse if and only if one or more of the underlying loadings are sparse. For small enough rank, sparse loadings imply a sparse tensor. The converse is not necessarily true: sparse tensor doesn't mean sparse loadings in general. On the other hand, the elements of a tensor are multivariate polynomials in the loadings, thus if the loadings are randomly drawn from a jointly continuous distribution, the tensor will not be sparse, almost surely. Accordingly to these considerations, \cite{SK12} suggests that for low-enough rank it is reasonable to model sparse tensors as arising from sparse loadings, saying CP-decomposition. 

We next argue that it is reasonable to assume $\cB$ is low rank and sparse in the tensor formulation of high-order interaction models. First, in modern biomedical research such as \cite{Hung2016}, only a small portion of coefficients contribute to the response, leading to a highly sparse $\cB$. Further, \cite{SK12} suggested that for the low-enough rank it is suitable to model sparse tensors as arising from sparse loadings, saying CP-decomposition. Moreover, this low-rank-and-sparse assumption (or approximation) seems necessary when the sample size is limited. Specifically, we assume $\cB$ is of CP rank-$K$ with $s$-sparse factors, where $K, s\ll p$. It is easy to see that the number of parameters in \eqref{eqn:tensor_interaction} is $K(p+1)$, which is significantly smaller than $(p+1)^3$, the total number of parameters in the original three-way interaction effect model \eqref{eq:interaction_model}. In this case, \eqref{eq:skeching} can be written as 
\begin{equation}\label{eqn:tensor_interaction}
\begin{split}
	& y_l=\Big\langle \sum_{k=1}^K\eta_k\bbeta_k\circ\bbeta_k\circ\bbeta_k,\bx_l\circ\bx_l\circ\bx_l\Big \rangle + \epsilon_l,\quad l=1,\ldots, n,\\
	& \text{where}\quad \|\bbeta_k\|_2 =1, \quad \|\bbeta_k\|_0 \leq s, \quad k\in [K].
\end{split}
\end{equation} 
%Therefore, the three-way interaction effect model can be reduced to the symmetric tensor recovery model with rank-1 sketchings.  %Intrinsically, the symmetric tensor recovery model can be treated as a high-order interaction effect model. 


%\begin{eqnarray*}
%	\mathbb E(Y|X)&=&\Big\langle \sum_{k=1}^K\eta_k\bbeta_k\circ\bbeta_k\circ\bbeta_k,\bX\circ\bX\circ\bX\Big \rangle\\
%	&=& K + \underbrace{3\sum_{j=1}^p\sum_{k=1}^K \beta_{kj}X_j}_{\text{main effect}}\\
%	&&+\underbrace{3\sum_{j=1}^p\sum_{k=1}^K\beta_{kj}^2X_j^2+6\sum_{i,j}\sum_{k=1}^K\beta_{ki}\beta_{kj}X_iX_j}_{\text{two-way interaction effect}}\\
%	&& + \underbrace{3\sum_{j=1}^{p}\sum_{k=1}^K\beta_{kj}^3X_j^3+6\sum_{i,j,m}\sum_{k=1}^K\beta_{ki}\beta_{kj}\beta_{km}X_i X_j X_m+3\sum_{i,j}\sum_{k=1}^K\beta_{ki}^2\beta_{kj}X_i^2X_j}_{\text{three-way interaction effect}}. 
%\end{eqnarray*}

\begin{comment}
\begin{remark}
The tensor reformulation for interaction effect has the following appealing features:
\begin{enumerate}
	\item If the main effect $X_j$ is not significant, all high-order interactions involving $X_j$ are not significant.
	
	\emph{Proof.} $\sum_{k=1}^K \beta_{kj} = 0 \Rightarrow \beta_{1j}=\ldots=\beta_{kj}=0$. This is due to the sign consistent constraint. {\red (I don't get this.)} Therefore, it's easy to verify $\sum_{k=1}^K\beta_{kj}^2, \sum_{k=1}^K\beta_{ki}\beta_{kj},\sum_{k=1}^K\beta_{kj}^3, \sum_{k=1}^K\beta_{ki}\beta_{kj}\beta_{km},\sum_{k=1}^K\beta_{ki}^2\beta_{kj}$, the coefficients of high-order interaction containing $X_j$ are equal to 0.
	
	\item If high-order interaction term $X_iX_j$ is significant, all the corresponding main effects are significant. 
	
	\emph{Proof.} Since $\sum_{k=1}^K\beta_{ki}\beta_{kj}\neq 0$, we obtain $\sum_{k=1}^K \beta_{ki}\neq 0$ and $\sum_{k=1}^K \beta_{kj}\neq 0$. If not, at least one of them are 0. Without loss of generality, let's $\sum_{k=1}^K \beta_{ki}= 0\Rightarrow \beta_{1i}=\ldots\beta_{ki}=0$. This will lead to $\sum_{k=1}^K\beta_{ki}\beta_{kj}= 0$, which is a contradiction.
	
	\item If one high-order interaction term is not significant, the main effect is no need to be insignificant.
\end{enumerate}
\end{remark}
\end{comment}
By assuming $\bz_l \overset{iid}{\sim}N_{p}(0, \bI_{p})$, the high-order interaction effect model \eqref{eq:skeching} reduces to the symmetric tensor estimation model \eqref{eq:model} with the only difference that the first coordinate of $\bx_l$, i.e., the intercept, is always 1. %Although only the first coordinate of sketching vector $X_l$ is different from the symmetric tensor recovery model, 
%However, this small difference makes the procedure phase will dramatically change compared with ordinary symmetric tensor recovery, since the first intercept covariate is non-random and non-centralized. We first construct an empirical moment based initial tensor for interaction model. Define three quantities
To accommodate this slight difference, we only need to adjust the initial unbiased estimate in the above two-step procedure. We first obtain $\cT_s$ in \eqref{eqn:moment_tensor_sym} by replacing $\bx_i$ therein by $\bx_{l}$, where $\bx_{l}$ corresponds the $l$-th observation 
\begin{equation}\label{eqn:moment_inter}
\begin{split}
\cT_s = & \frac{1}{6n}\sum_{l=1}^n y_l \bx_l \circ \bx_l \circ \bx_l- \frac{1}{6}\sum_{j=1}^p(\ba\circ \be_j\circ \be_j+ \be_j\circ \ba \circ \be_j+\be_j\circ \be_j\circ \ba), \\
& \text{where } \quad \ba = \frac{1}{n}\sum_{l=1}^n y_l \bx_l,
%& \ba = \frac{1}{n}\sum_{l=1}^n y_l X_l, \quad \tilde{\cA} = \frac{1}{n}\sum_{i=l}^n y_l X_l \circ X_l \circ X_l\\
%&\cT_s = \frac{1}{6}(\tilde{A}- \sum_{j=1}^p(\ba\circ \be_j\circ \be_j+ \be_j\circ \ba \circ \be_j+\be_j\circ \be_j\circ \ba)).
\end{split}
\end{equation}
then construct empirical-moment-based initial tensor $\cT_{s'}$ as
\begin{itemize}
	\item For $i,j,k\neq 0$, $\cT_{s'[i,j,k]} = \cT_{s[i,j,k]}$. And $\cT_{s'[i,j,0]} = \cT_{s[i,j,0]}, \cT_{s'[0,j,k]} = \cT_{s[0,j,k]}, \cT_{s'[i,0,k]} = \cT_{s[i,0,k]}$.
	\item For $i\neq 0$, $\cT_{s'[0,0,i]} = \cT_{s'[ 0, i, 0]} = \cT_{s'[i,0,0]} = \frac{1}{3}\cT_{s[0,0,i]} - \frac{1}{6}(\sum_{k=1}^p\cT_{s[k,k,i]}-(p+2)a_i)$.
	\item $\cT_{s'[0,0,0]} = \frac{1}{2p-2}(\sum_{k=1}^p\cT_{s[0,k,k]} - (p+2)\cT_{s[0,0,0]})$. 
\end{itemize}
Lemma \ref{lemma:moment_interaction} verifies that $\cT_{s'}$ is an unbiased estimator for $\mathcal{B}$.

Theoretical results in Section \ref{sec:theory-symmetric} imply the following upper and lower bound results in this particular example. 
\begin{Corollary}
	Suppose that $\bz_1,\ldots, \bz_n$ are i.i.d. standard Gaussian random vectors and $\mathcal{B}$ satisfies Conditions \ref{con:ident}, \ref{con:parameter} and \ref{con:incoherence_sym}. The output, denoted as $\hat \cB$, from the proposed Algorithms \ref{alg:overall_symmetric} and \ref{alg:overall_symmetric-gradient} based on $\cT_{s'}$ satisfies
	\begin{equation}
	\left\|\hat{\cB} - \cB\right\|_F^2 \leq C\frac{\sigma^2Ks\log p}{n}
	\end{equation}
	with high probability. On the other hand, considering the following class of $\mathcal{B}$,
	\begin{equation*}
	\mathcal{F}_{p+1, K, s} = \left\{\mathcal{B}: \begin{array}{l}
	\mathcal{B} = \sum_{k=1}^K\eta_k \bbeta_k\circ \bbeta_k\circ \bbeta_k, \|\bbeta_k\|_0 \leq s, \text{ for } k \in[K],\\ 
	\mathcal{B} \ \text{satisfies Conditions \ref{con:ident},  \ref{con:parameter}, and \ref{con:incoherence_sym}},
	\end{array}\right\}.
	\end{equation*}
	then the following lower bound holds,
	\begin{equation*}
	\inf_{\hat{\mathcal{B}}}\sup_{\mathcal{B}\in \mathcal{F}_{p+1, K, s}}\mathbb{E}\left\|\hat{\cB} - \cB\right\|_F^2 \geq C\frac{\sigma^2Ks\log p}{n}.
	\end{equation*}
\end{Corollary}



\begin{comment}
{\red (Can you describe the procedure, and the corresponding Corollary here?)

I realized the following fact, which might be useful for your calculation :-), for each $1\leq i <j<k\leq p$,
\begin{equation*}
\begin{split}
& \left(\frac{1}{n}\mathbb{E} \sum_{l=1}^n y_l \bX_l\circ \bX_l \circ \bX_l\right)_{0,0,0} = \bB_{0,0,0} + 3 \sum_{i=1}^p B_{[0, i,i]}\\
& \left(\frac{1}{n}\mathbb{E} \sum_{l=1}^n y_l \bX_l\circ \bX_l \circ \bX_l\right)_{0,0,i} = 3 \sum_{j=0}^p \bB_{[i, j,j]}\\
& \left(\frac{1}{n}\mathbb{E} \sum_{l=1}^n y_l \bX_l\circ \bX_l \circ \bX_l\right)_{0,i,i} = 6\bB_{i,i, 0} + 3 \sum_{k=0}^p B_{[k,k, 0]}\\
& \left(\frac{1}{n}\mathbb{E} \sum_{l=1}^n y_l \bX_l\circ \bX_l \circ \bX_l\right)_{0,i,j} = 6\bB_{[0, i,j]}\\
& \left(\frac{1}{n}\mathbb{E} \sum_{l=1}^n y_l \bX_l\circ \bX_l \circ \bX_l\right)_{i,i,i} = 6\bB_{i,i,i} + 9 \sum_{k=0}^p B_{k,k,i}\\
& \left(\frac{1}{n}\mathbb{E} \sum_{l=1}^n y_l \bX_l\circ \bX_l \circ \bX_l\right)_{i,i,j} = 6\bB_{i,i,j} + 3 \sum_{k=0}^p B_{k,k,j}\\
& \left(\frac{1}{n}\mathbb{E} \sum_{l=1}^n y_l \bX_l\circ \bX_l \circ \bX_l\right)_{i,j,k} = 6\bB_{i,j,k}
\end{split}
\end{equation*}
Denote $\tilde{T} = \frac{1}{n}\sum_{l=1}^n y_l \bX_l\circ \bX_l\circ \bX_l$. Thus, we have the following unbiased estimator for $\bB$: $\bT \in \mathbb{R}^{(p+1)\times(p+1)\times(p+1)}$, 
\begin{equation*}
\begin{split}
& T_{i,j,k} = \frac{1}{6} \tilde{T}_{i,j,k} \\
& T_{i,i,j} = \frac{1}{6}\tilde{T}_{i,i,j} - \frac{1}{2(3p+15)}\sum_{k=0}^p \tilde{T}_{k,k,j}\\
& T_{i,i,i} = \frac{1}{6}\tilde{T}_{i,i,i} - \frac{3}{2(3p+15)}\tilde{T}_{k,k,j}\\
& T_{0,i,j} = \frac{1}{6} \tilde{T}_{1,i,j} \\
& T_{0,i,i} = \frac{1}{6} \tilde{T}_{1,i,i} - \frac{1}{2(3p+18)}\left\{\sum_{k=1}^p \tilde{T}_{k,k,0} + 6\tilde{T}_{0,0,0}\right\}\\
&  T_{0,0,i} = \frac{1}{3}\tilde{T}_{0,0,i} - \sum_{j=1}^p T_{j,j,i} \\
&  T_{0,0,0} = \tilde{T}_{0,0,0} - 3\sum_{i=1}^p T_{[0,i,i]} \\
\end{split}
\end{equation*}
%On the other hand,
%\begin{equation*}
%\begin{split}
%& \mathbb{E}\left(\frac{1}{n}\mathbb{E} \sum_{l=1}^n y_l \bX_l\circ \bX_l\right)_{0,0} = \sum_{i=0}^p B_{[0,i,i]}\\
%& \mathbb{E}\left(\frac{1}{n}\mathbb{E} \sum_{l=1}^n y_l \bX_l\circ \bX_l\right)_{0,i} = B_{[0,0,i]}\\
%& \mathbb{E}\left(\frac{1}{n}\mathbb{E} \sum_{l=1}^n y_l \bX_l\circ \bX_l\right)_{i,i} = B_{[0,i,i]}+2\sum_{j=0}^p B_{[0,j,j]}\\
%& \mathbb{E}\left(\frac{1}{n}\mathbb{E} \sum_{l=1}^n y_l \bX_l\circ \bX_l\right)_{i,j} = \sum_{i=0}^p B_{[0,i,i]}\\
%\end{split}
%\end{equation*}

}
\end{comment}


\begin{comment}\cite{Hung2016} utilize the matrix nature of two-way interaction terms and consider a reduced model with matrix low-rank structure. A commonly used joint-screening method for gene-gene detection is to apply Lasso on the model
\begin{eqnarray}
\mathbb E(\bY|\bg) = \gamma + \sum_{j=1}^{p}\xi_j g_j + \sum_{j<k}a_{jk}(g_j g_k).
\end{eqnarray}
In this model, $(g_jg_k)$ is the $(j,k)$th element of the symmetric matrix $\bJ = \bg\bg^{\top}$. Thus, an equivalent expression of above model is
\begin{eqnarray}
\mathbb E(\bY|\bg) = \gamma + \bxi^{\top}\bg + \text{vecp}(\bA)^{\top} \text{vecp}(\bJ),
\end{eqnarray}
where $\bxi$ is the coefficient vector of main effects, and $\text{vecp}(\cdot)$ denotes the operator that stacks the lower half of a symmetric matrix columnwisely into a long vector. Then they posit the condition
\begin{eqnarray*}
\bA:\text{being sparse and low rank}.
\end{eqnarray*}
This will largely reduce the parameter space.
\end{comment}

==> t-cubic-sketch4-nonsym.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Non-symmetric Tensor Estimation Model}\label{sec:non-symmetrc}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this section, we extend the previous results to the non-symmetric tensor case. Specifically, we have $\mT^*\in \mathbb R^{p_1\times p_2\times p_3}$, and 
\begin{equation}\label{eq:model_asymmetric}
\begin{split}
y_i = \langle\mT^*, \mX_i \rangle+\epsilon_i, \ \mX_i = \bu_i\circ \bv_i\circ \bw_i, \ i\in[n],
\end{split}
\end{equation}
where $\bu_i\in \mathbb{R}^{p_1}, \bv_i\in \mathbb{R}^{p_2}, \bw_i\in \mathbb{R}^{p_3}$ are random vectors with i.i.d. standard normal entries. Again, we assume $\mT^*$ is sparse and low-rank in a similar sense that
\begin{equation}\label{eq:low_rank_nonsym}
\begin{split}
& \mT^* = \sum_{k=1}^K \eta_k^*\bbeta_{1k}^*\circ\bbeta_{2k}^*\circ\bbeta_{3k}^*,\\  
& \|\bbeta_{1k}^*\|_2 = \|\bbeta_{2k}^*\|_2 = \|\bbeta_{3k}^*\|_2 = 1,\quad \max\{\|\bbeta_{1k}^*\|_0, \|\bbeta_{2k}^*\|_0, \|\bbeta_{3k}^*\|_0\}\leq s.
\end{split}
\end{equation}
Denote the following:
\begin{itemize}
	\item $\bB_1 = (\bbeta_{11}, \cdots,\bbeta_{1K})$, $\bB_2 = (\bbeta_{21}, \cdots,\bbeta_{2K})$, $\bB_3 = (\bbeta_{31}, \cdots,\bbeta_{3K})$,
	\item $\bU=(\bu_1, \ldots,\bu_n),  \ \bV=(\bv_1, \ldots,\bv_n), \ \bW=(\bw_1, \ldots,\bw_n)$, \\
	 $\boldsymbol{\eta} = (\eta_1, \ldots, \eta_k)^{\top}, \by = (y_1, \ldots, y_n)^{\top}.$
\end{itemize} 
Then, the empirical risk function can be written compactly as
\begin{equation}\label{def:risk_function_nym}
\cL(\bB_1, \bB_2, \bB_3, \boldsymbol{\eta} ) 
= \frac{1}{n}\Big\|(\bU^{\top}\bB_1) * (\bV^{\top}\bB_2) * (\bW^{\top}\bB_3)\cdot\boldsymbol{\eta} - \by\Big\|_2^2.
\end{equation}
We note that \eqref{def:risk_function_nym} is non-convex, but fortunately tri-convex in terms of $\bB_1$, $\bB_2$ and $\bB_3$. This allows us to develop a block-wise thresholded gradient descent algorithm as detailed below. 

The major steps of the estimation procedure for non-symmetric tensors are sketched below. The complete algorithm is deferred to Section \ref{alg:overall_nonsymmetric} in the supplementary materials.
\begin{description}
	\item[Step 1: (Method of Tensor Moments)] Construct an empirical-moment-based estimator,
	\begin{eqnarray}\label{eq:moment_asy}
	\cT:=\frac{1}{n}\sum_{i=1}^n y_i \bu_i\circ \bv_i\circ \bw_i\in \mathbb R^{p_1\times p_2\times p_3}.
	\end{eqnarray}	 
	to which sparse tensor decomposition is applied for initialization. 
	\item[Step 2: (Block-wise Gradient descent)] Lemma \ref{lemma:gradient_equivalence_aym} in the supplementary materials shows that the gradient function for \eqref{def:risk_function_nym} with respect to $\bB_1$ can be written as
	\begin{equation}
	\label{eqn:gradient_nonsym}
		\nabla_{\bB_1}\cL(\bB_1, \bB_2, \bB_3, \boldsymbol{\eta}) = \bD^{\top}(\bC_1^{\top}\odot\bU)^{\top}\in \mathbb R^{1\times (p_1K)},
	\end{equation}
	where $\bD = (\bB_1^{\top}\bU)^{\top}*(\bB_2^{\top}\bV)^{\top}*(\bB_3^{\top}\bW)^{\top}\boldsymbol{\eta} - \by$ and $\bC_1 = (\bB_2^{\top}\bV)^{\top}*(\bB_3^{\top}\bW)^{\top}\odot \boldsymbol{\eta}^{\top}$.
  	For $t=1,\ldots, T$ we fix $\bB_2^{(t)}$ and $\bB_3^{(t)}$ and update $\bB_1^{(t+1)}$ via block-wise thresholded gradient descent,
	\begin{eqnarray*}
		\tv(\bB_1^{(t+1)}) = \varphi_{\tfrac{\mu h(\bB_1^{(t)})}{\phi}}\Big(\tv(\bB_1^{(t)}) - \frac{\mu}{\phi}\nabla_{\bB_1}\cL(\bB_1^{(t)}, \bB_2^{(t)}, \bB_3^{(t)}, \boldsymbol{\eta})\Big), 
	\end{eqnarray*}
	where $\phi= \sum_{i=1}^{n}y_i^2/n$, $\mu$ is the step size and $\bh(\bB) = \sqrt{\frac{4\log np}{n^2}\{\bD^{2}\}^{\top}\{\bC^2\}}$. The updates of $\bB_2, \bB_3$ are similar.
\end{description}


The main theoretical analysis is different from the symmetric one in two folds. First, the non-symmetric cubic sketching tensor is formed by three independent Gaussian vectors. This leads to differences in many high-order moment calculations. Second, the corresponding CP-decomposition, i.e., \eqref{eq:low_rank_nonsym}, essentially forms a bi-convex optimization. In this case, standard convex analysis for vanilla gradient descent \citep{Bubeck15} could be applied given a good enough initialization. 

We impose similar regularity conditions whose detailed forms and explanations are postponed to Section \ref{alg:overall_nonsymmetric} and the proof to Section \ref{sec:proof_asym}.  The main theorems for non-symmetric tensor estimation are presented as follows.
\begin{Theorem}[(Upper Bound)]
	\label{thm:main_nym}
	Suppose Conditions \ref{con:ident_nym} -- \ref{con:noise_non} in the supplementary materials hold and $n\gtrsim (s\log (p_0/s))^{3/2}$, where $p_0 = \max\{p_1, p_2, p_3\}$. For any $t=0,1,2,\ldots$, the estimation output by Algorithm \ref{alg:overall_nonsymmetric} satisfies
		\begin{eqnarray*}
			\sum_{k=1}^{K}\sum_{j=1}^3\Big\|\sqrt[3]{\eta_{k}}\bbeta_{jk}^{(t+1)} -\sqrt[3]{\eta_k^*}\bbeta_{jk}^{*} \Big\|_2^2 \leq \cO_p\Big(\kappa^t+\frac{\sigma^2s\log p_0}{n}\Big)
		\end{eqnarray*}
	for some $0<\kappa<1$. When the total number of iterations is no smaller than $\log (\frac{n}{\sigma^2s \log p_0} \vee 1) /\log \kappa^{-1}$, the final estimator $\hat{\mT}$ satisfies
		\begin{eqnarray*}
			\Big\|\hat{\mT}-\mT^*\Big\|_F^2\leq \cO_p\Big(\frac{\sigma^2Ks\log p_0}{n}\Big).
		\end{eqnarray*}
\end{Theorem}
%The proof of Theorem \ref{thm:main_nym} are deferred to Section \ref{sec:non-symmetrc} in the supplemental material. 
%The minimax lower bound for non-symmetric tensor estimation can be developed correspondingly.
\begin{Theorem}[(Lower Bound)]
	\label{th:lower_bound_asymmetric}
	Consider the class of incoherent sparse and low-rank tensors $\mathcal{F} = \{\mT: \mT = \sum_{k=1}^K \bbeta_{1k}\circ \bbeta_{2k}\circ \bbeta_{3k}, \|\bbeta_{i,k}\|_0 \leq s \text{ for } i = 1, 2, 3, k=1,\ldots, K\}$. If $\{\mX_i\}_{i=1}^n$ are i.i.d standard normal cubic sketchings with i.i.d. $N(0,\sigma^2)$ noises in \eqref{eq:model_asymmetric}, the following lower bound holds,
	\begin{equation}
	\inf_{\hat{\mT}}\sup_{\mT \in \mathcal{F}} \mathbb{E} \left\|\hat{\mT} - \mT\right\|_F^2\geq \frac{C\sigma^2sK\log(e\cdot p_0/s)}{n}.
	\end{equation}
\end{Theorem}
It can be seen from Theorems \ref{thm:main_nym} and \ref{th:lower_bound_asymmetric} that our proposed algorithm achieves minimax-optimal estimation error rate in the class of $\mathcal{F}$ as long as $\log(p_0) \asymp \log(p_0/s)$.



%\begin{remark}
%	Note that quantity $\cT$ and $\cT_s$ don't include any unknown quantity. The second term in $\cT_s$ is for de-bias purpose since the correlation from symmetric structure causes bias, which is different from the non-symmetric case.
%\end{remark}


%Intuitively, once we are given sufficiently large number of samples, the well-constructed tensor $\cT$ and $\cT_s$ should be a roughly good estimate for the truth $\mT$. Based on Lemma \ref{lemma:moment}, it will formulate an tensor denoising model $\cT = \mT^*+\cE$, where $\cE = \cT - \mathbb E(\cT)$. Therefore, by applying sparse tensor decomposition method on $\cT$ and $\cT_s$, we can get an initial estimate for $\{\bB_1, \bB_2, \bB_3\}$  in the first phase, see Table \ref{algorithm1}.

%\begin{remark}
%	The difference of our method and \cite{Sun2016} lies on two parts. Firstly, we do not use sparse SVD as warm start for tensor decomposition procedure. This is due to the fact that the computation cost for SVD is even heavier than alternating update step. And random initialization is lack of theoretical guarantee although it performs well in practice. On the other hand, instead of using hard thresholding, we use soft-threshold $S(\cdot, \rho) = \sign(\cdot)\max(|\cdot|-\rho, \cdot)$, which could provide us support recovery guarantee.
%\end{remark}

%Note that the sparse tensor decomposition could also be applied to symmetric tensor by slightly changing the algorithm.


==> t-cubic-sketch5-numeri-disc.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Numerical Results}\label{sec:simu}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this section, we empirically examine the effect of noise level, CP-rank, sample size, dimension, and sparsity on the estimation performance. We also examine the robustness of the proposed algorithm under the setting when the incoherence assumption used in theory fails to hold.

In each setting, we generated $\mT^* = \sum_{k=1}^K \bbeta_k^*\circ \bbeta_k^* \circ \bbeta_k^*$, where $|\supp(\bbeta_k^*)|=s$ was uniformly selected from $\{1,\ldots, p\}$, the nonzero entries of $\bbeta_k^*$ were drawn from standard Gaussian distribution. Next we normalized each vector $\bbeta_k^*$ and aggregated the coefficient as $\eta_k^*$.   The cubic sketchings $\{\mX_i\}_{i=1}^n$ were generated as $\mX_i = \bx_i\circ \bx_i\circ \bx_i$, where $\{\bx_i\}_{i=1}^n$ were from standard Gaussian distribution. The noise $\{\epsilon_i\}_{i=1}^n \overset{iid}{\sim} N(0, \sigma^2)$ or $\text{Laplace}(0, \sigma/\sqrt{2})$. Additionally, we adopt the following stopping rules: (1) the initialization iteration (Step 2 in Algorithm \ref{alg:overall_symmetric}) is stopped if $\|\bb_m^{(l+1)} - \bb_m^{(l)}\|_2\leq 10^{-6}$; (2) the gradient update iteration (Step 3 in Algorithm \ref{alg:overall_symmetric-gradient}) is stopped if $\|\bB^{(T+1)} - \bB^{(T)}\|_F\leq 10^{-6}$. All presented results were based on 200 repetitions. The code was written in R and implemented on an Intel Xeon-E5 processor with
64 GB of RAM. %times with independently generated $\{\mX_i,\epsilon_i\}_{i=1}^n$. In this section, the sparsity parameter $s_0$ is defined as the proportion of non-zero elements.

%In the simulation, there is no need to specify the number of iterations $N, T$ in both sparse tensor decomposition step and thresholded gradient descent. Instead, 

%To measure the estimation performance, we report two types of  average errors: one in absolute Frobenius norm $\|\hat{\mT}-\mT^*\|_F$, another one in relative Frobenius norm $\|\hat{\mT}-\mT^*\|_F/\|\mT^*\|_F$.



First, we consider the percent of successful recovery in the noiseless case. Let $K=3$, $s/p=0.3$, $p = 30$ or $50$, so that the total number of unknown parameters in $\mT^\ast$ is $2.7\times 10^4$ or $1.25\times 10^5$. The sample size $n$ ranges from 500 to 6000. The recovery is called successful if the relative error $\|\hat{\mT}-\mT^*\|_F/\|\mT^*\|_F < 10^{-4}$. We report the percent of successful recovery in Figure \ref{fig_exact}.
	\begin{figure}
		\centering
			\includegraphics[width =0.48\linewidth,height=2.0in]{figure/exact_recovery.png}
			\caption{Percent of successful recovery with varying sample size.}
			\label{fig_exact}
	\end{figure}
It is clear from Figure \ref{fig_exact} that the empirical relation with dimensionality and sample size is consistent with our theory. 

We then move to the noisy case where the empirical estimation error is examined. We select $K=3$, $s/p=0.3$, $p=30$ or $50$, $\{\epsilon_i\}_{i=1}^n \overset{iid}{\sim} N(0, \sigma^2)$ and consider two specific scenarios: (1) sample size $n$ = 6000, 8000, or 10000, $s/p=0.3$, the noise level $\sigma$ varies from 0 to 200; (2) noise level $\sigma = 200$, sample size $n$ varies from 4000 to 10000, $p=30$, $s/p=0.1, 0.3, 0.5$. The estimation errors in terms of $\|\hat{\mT} - \mT^*\|_F$ under these two scenarios are plotted in Figures \ref{fig_noise_level} and \ref{fig_sample_size}, respectively. From these results, we can see that the proposed algorithm achieves reasonable estimation performance: Algorithms \ref{alg:overall_symmetric} and \ref{alg:overall_symmetric-gradient} yield more accurate estimation with smaller variance $\sigma^2$ and/or large value of sample size $n$. 
	\begin{figure}
	\centering
	\includegraphics[width =0.48\linewidth,height=2.0in]{figure/noise_effect_p30.png}
	\includegraphics[width =0.48\linewidth,height=2.0in]{figure/noise_effect_p50.png}
	\caption{Estimation error for different noise levels. The left panel is $p=30$ and the right panel is $p=50$.}
	\label{fig_noise_level}
	%	\end{figure}	
	%	\begin{figure}
	%	\centering
	\includegraphics[width =0.48\linewidth,height=2.0in]{figure/sample_size_effect_ini.png}
	\includegraphics[width =0.48\linewidth,height=2.0in]{figure/sample_size_effect_final.png}
	\caption{Estimation error for different sample sizes. The left panel is for initial estimation error and the right panel is for final estimation error. }
	\label{fig_sample_size}
\end{figure}


Next, we demonstrate that the low-rank tensor parameter $\mT^*$ with randomly generated factors $\bbeta_k^*$ satisfies the
incoherence Condition \ref{con:incoherence_sym} with high probability. Set the CP-rank $K=3$ and the sparsity level $s/p = 0.3$ with the dimension $p$ ranging from 10 to 2000. We compute the incoherence parameter $\Gamma$ defined in Condition \ref{con:incoherence_sym}. The left panel of Figure \ref{fig_incoherence} shows that the incoherence parameter $\Gamma$ decays in a polynomial rate as $s$ grows, which matches the bound in Condition \ref{con:incoherence_sym}. Recall we also provide theoretical justification on this point in Lemma \ref{lemma:proof_incoherence}. 

\begin{figure}
\centering
    \includegraphics[width =0.48\linewidth,height=2.0in]{figure/incoherence_check.png}			\includegraphics[width =0.48\linewidth,height=2.0in]{figure/incoherence_compare.png}
			\caption{Left panel: incoherence parameter $\Gamma$ with varying sparsity. Here, the red line corresponds to the rate $\sqrt{s}$ required in the theoretical analysis. Right panel: average relative estimation error for tensors with varying incoherence.
			}
	\label{fig_incoherence}
	\end{figure}

We further examine the performance of the proposed algorithm when the incoherence condition required in the theoretical analysis fails to hold. Specifically, we set the CP-rank $K=3$, $p=30$, and the sparsity level $s/p = 0.3$. We construct enormous copies of tensor parameter $\mT^*_j$ with i.i.d. standard normal factor vectors $\bbeta_k^*$. For each $\mT^*_j$, we calculate the incoherence $\Gamma_j$ defined in Condition \ref{con:incoherence_sym}, and then manually pick 40 parameter tensors $\mT^*_{j'}$ such that 
$$0.01\cdot (j'-1)\leq \Gamma_{j'}\leq 0.01 \cdot j' \quad \text{for}\quad j' = \{1, 2, \ldots, 40\}.$$
By this construction, we obtain a set of tensor parameter $\{\mT^*_{j'}\}$ with incoherence uniformly varying from 0 to 0.4. The right panel of Figure \ref{fig_incoherence} plots the relative error for estimating $\mT^*$ based on observations from cubic sketchings of $\mT^*_{j'}$ based on 1000 repetitions. We can see that the proposed algorithm  achieves small relative errors even when the true factors are highly coherent.
%{\blue It seems that you didn't repeat in this experiment. So the curves are not very smooth. Do you think it is more valid to repeat?}



Moreover, we consider another setting with Laplace distributed noise which is a sub-exponential random variable. Suppose $\{\epsilon_i\}_{i=1}^n \overset{iid}{\sim}Lap(\sigma)$ with density $f(x) = \frac{1}{\sigma}\exp(-2|x|/\sigma)$. With $n=3000$, $p=30$, and varying values of $\sigma$, the average estimation error and its comparison with Gaussian noise setting are provided in Figure \ref{fig_laplace_error}. We note that the estimation errors under Laplace noise are slightly higher than those under Gaussian noise. 


%Next, for a fixed noise level $\sigma = 200$, we examine the how the sample size affects the initialization and final estimation under different sparsity settings. The CP-rank $K=3$ and the factor dimension is $p=30$. The sample size varies from 4000 to 10000. The detailed results are stated in Figure \ref{fig_sample_size}
	\begin{figure}
		\centering
		\includegraphics[width =0.48\linewidth,height=2.0in]{figure/laplace_error.png}
		\caption{Comparison of estimation errors between Laplace error and Gaussian error. }
		\label{fig_laplace_error}
	\end{figure}



	Next, we compare the estimation errors of initial and final estimators for different ranks and sample sizes. First we set $K=3, p =30, s/p = 0.3$ and consider the noiseless setting. It is clear from Figure \ref{fig_initial_effect} that the initialization error decays sufficiently, but does not converge to zero as sample size $n$ grows. This result matches our theoretical findings in Theorem \ref{thm:initial_symmetric}. As discussed in Remark \ref{rm:initialization error}, the initial stage may yield an inconsistent estimator due to the incoherence among $\bbeta_k$'s. After sufficient steps of thresholded gradient descent (Steps 3 and 4 in Algorithm \ref{alg:overall_symmetric-gradient}), the initial estimator is refined to lead to the final estimate that is proven to be minimax-optimal. Thus, we evaluate and compare estimation errors for both initial and final estimators for $K=3$ or 5 and growing sample sizes $n$. We can see from the right panel of Figure \ref{fig_initial_effect}, the final estimator is more stable and accurate compared with the initial one, which illustrates the merit of thresholded gradient descent step of the proposed procedure.
	\begin{figure}
		\centering
		\includegraphics[width =0.48\linewidth,height=2.0in]{figure/initial_effect.png}
		\includegraphics[width =0.48\linewidth,height=2.0in]{figure/rank_effect.png}
		\caption{Log absolute estimation error of initial estimation error (left panel) and initialization/final estimation error comparisons (right panel).}
		%\caption{Initial estimation error with varying sample size.}
		\label{fig_initial_effect}
	\end{figure}

%We compare the rank-effect in the next scenarios. The CP-rank $K=3$ and the factor dimension is $p=30$ and the noise level $\sigma = 200$. CP-rank $K=3$ and $K=5$ are considered. We report both initial estimation error and final estimation error. The detailed results are stated in Figure \ref{fig_rank_effect}
%	\begin{figure}
%		\centering
%			\includegraphics[width =0.48\linewidth,height=2.0in]{figure/rank_effect.png}
%			\caption{Log absolute estimation error of initial estimation error and final estimation error for different ranks.}
%	\label{fig_rank_effect}
%	\end{figure}
	
%Finally, we specifically compare the initial stage and show that no matter how large the sample size is, the initial stage can not output a consistent estimate. And hence it verifies our theoretical findings. We select $K=3, p =30, s/p = 0.3$ and consider a noiseless setting. The detailed results are stated in Figure \ref{fig_initial_effect}. 
%	\begin{figure}
%		\centering
%			\includegraphics[width =0.48\linewidth,height=2.0in]{figure/initial_effect.png}
%			\caption{Initial estimation error with varying sample size.}
%		\label{fig_initial_effect}
%	\end{figure}

Last but not the least, we compare the performance of our method with the alternating least square (ALS)-based tensor regression method \citep{zhou2013}. We specifically consider two schemes for the initialization of ALS: (a) $\{\bbeta_k^{(0)}\}$ were generated as i.i.d. standard Gaussian (cold start), and (b) $\{\bbeta_k^{(0)}\}$ were generated from the proposed Algorithm \ref{alg:overall_symmetric} (warm start). Setting $K=2$, $s/p=0.2$, $p=30$, $\{\epsilon_i\}_{i=1}^n \overset{iid}{\sim} N(0, 200^2)$, we applied both our proposed procedure and the ALS-based algorithm, and recorded average estimation errors with standard deviations for both initial and final estimators in Table \ref{tab:sim_result_tensorreg}. From the result, one can see our proposed algorithm significantly outperforms the ALS proposed by \cite{zhou2013} under both cold and warm start schemes. The main reason was pointed out in Remark \ref{rm:comparison-matrix-setting}: the cubic sketchings setting possesses distinct aspects compared with the i.i.d. random Gaussian sketching setting, so that the method proposed by \cite{zhou2013} does not exactly fit. %and does not satisfy the assumption most of existing tensor regression literatures made which have a $i.i.d$ Gaussian sketching tensor. %Second, the alternating least square fails to capture the exact symmetric structure.
\begin{table}[htb]
	\centering
	\label{tab:sim_result_tensorreg}
	\vskip 1 em
	\begin{tabular}{c|c|c|c|c}
		\hline
		Sample size &ours & warm start & cold start & initial \\
		\hline
	   $n=4000$ &$4.023_{0.135}$   & $32.828_{1.798}$ & $37.785_{1.233}$& $38.032_{1.748}$  \\
		\hline
		$n=5000$&$1.945_{0.097}$  &$32.346_{2.343}$ & $36.962_{2.106}$ &$33.716_{1.786}$  \\
		\hline   
		$n=6000$ &$1.773_{0.092}$ &$22.220_{1.215}$  &$59.972_{3.407}$ & $25.579_{1.483}$ \\
		\hline
	\end{tabular}
	\caption{The estimation error and the standard deviation (in subscript) of the proposed method and ALS-based method.}
\end{table}




 

	\begin{comment}	
	
	\item We examine the tuning parameter effect. In the algorithm \eqref{alg:overall_symmetric}, we have two tuning parameter. One is used in the initialization and one is used in the gradient update. Note that since they are in the different stages, they will not interact with each other. For this consideration, we fixed the truncation level parameter $\rho=5$ first and varied the cardinality parameter from 0 to 20. Then we fixed the cardinality parameter to the truth $d=9$ in $p=30$ case and varied the truncation level parameter from 0 to 20. We report the recover relative error in Figure
	\begin{figure}[h!]\label{fig_noise}
	\centering
	\begin{small}
	\caption{The left figure reports the relative estimation error for different cardinality parameters. The right figure reports the relative estimation error for different truncation levels. }
	\label{fig:sim_clustering}
	\includegraphics[scale=0.3]{ini_truncation_p30.png}
	\includegraphics[scale=0.3]{truncation_effect_p30.png}
	\end{small}
	\end{figure}
	\end{comment}

\begin{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Interaction Effect Model}\label{sub:sim_interact}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this subsection, we examine the effect of our algorithm applying to interaction effect model. 
\begin{itemize}
	\item Exact low-rank case. Consider $p=30, N = 300$. And each $\bx_i = (1, x_{1i},\ldots, x_{30i})^{\top}$ is drawn from $\cN(0, \bI_p)$. We will fit an interaction effect model with main effects, pair-wise interaction effects and triple-wise interaction effects. The total number of parameter should be $30^3 = 27000$. Correspondingly, suppose tensor parameter $\cB$ in \eqref{eq:skeching} is of exact CP rank-two. The first factor $\bbeta_1$ is designed by setting the first five coordinate be $(1, 0, 0, 1, 1)$ and the rest be zero.  The second factor is designed by setting the first five coordinate be $(1, 1, 0, 1, 1)$ and the rest be zero. Accordingly to \eqref{eqn:tensor_interaction}, the fully expanded interaction effect model can be written as
	\begin{eqnarray*}
		y_i &=& \big\langle\bbeta_1\circ\bbeta_1\circ\bbeta_1+ \bbeta_2\circ\bbeta_2\circ\bbeta_2, \bx_i\circ\bx_i\circ\bx_i \big\rangle+\epsilon_i\\
		&=& 2+3x_{1i}+6x_{3i}+6x_{4i}\\
		&&+6x_{1i}x_{3i}+6x_{1i}x_{4i}+12x_{3i}x_{4i}+3x_{1i}^2+6x_{3i}^2+6x_{4i}^2\\
		&&+3x_{1i}^2x_{3i}+3x_{1i}^2x_{4i}+3x_{3i}^2x_{1i}+3x_{4i}^2x_{1i}++6x_{3i}^2x_{4i}+6x_{4i}^2x_{3i}\\
		&&+x_{1i}^3+2x_{3i}^3+2x_{4i}^3+6x_{1i}x_{3i}x_{4i}+\epsilon_i.
	\end{eqnarray*}
	This model is more flexible than the traditional linear regression and pair-wise interaction model. It includes main effects, pair-wise interaction effects, triple-wise interaction effects and even quadratic and cubic effects. 
\end{itemize}
\end{comment}
\begin{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Real Data Illustration in High-order Interaction Pursuits}\label{sub:real_data}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this section, we investigate our tensor recovery method on the inbred mouse microarray
gene expression dataset \citep{lan2006combined}. The inbred mouse microarray dataset contains 60 mouse arrays, with 31 from female mice and 29 from
male mice, respectively. Each array measures the expression values of 22,690 genes. The response is a continuous phenotypic variable measured by real-time RT-PCR, stearoyl-CoA desaturase 1 (SCD1). Tensor recovery method is applied to this dataset to find the significant genes, pairwise interaction effect and triple-wise interaction effect. We first select top $100$ significant genes by correlation screening, and label them by Gene 1 to Gene 100. Then the third-order symmetric tensor recovery is applied to identify main effect, pair-wise interaction effect and triple-wise interaction effect. The truncation parameter $d$ is given by the proportion of significant main effects selected by Lasso. 
Since symmetric tensor recovery procedure tends to select a bigger model in terms of high-order interaction terms, we add an additional truncation step to truncate the small coefficients. The result shows that the tensor recovery procedure can select 13 genes as main effect, which are Gene 2, 6, 13, 18, 20, 38, 47, 49, 59, 60, 70, 80, 94, as well as 36 pair-wise interaction effects including quadratic effects and 47 triple-wise interaction effects including cube effects. Previous study failed to identify the third-order interaction effects.

{\red (Can you say something more, maybe draw a picture or list a table for this part?)}
\end{comment}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Discussions}\label{sec:discussion}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The current paper focuses on the third order tensor estimation. But, all the results can be extended to higher-order case via high-order sketchings as follows.  To be specific, suppose
$$y_i = \langle \mT^\ast, \bx_i^{\otimes d} \rangle + \epsilon_i, \quad i=1,\ldots, n,$$
where $\mT^\ast \in (\mathbb{R}^{p})^{\otimes d}$ is an order-$d$, sparse, and low-rank tensor. In order to estimate $\mT^\ast$ from $\{y_i, \bx_i\}_{i=1}^n$, one can first generalize Theorem \ref{thm:steins_higher} to construct the order-$d$ tensor moment estimate for the initial stage, by noting that the score function $\cS_d(\bx)$ and the density function $p(\bx)$ satisfy a nice recursive equation: $$\cS_d(\bx):=-\cS_{d-1}(\bx)\circ \nabla\log p(\bx)-\nabla \cS_{d-1}(\bx).$$ Then, one can similarly perform high-order sparse tensor decomposition and thresholded gradient descent to estimate $\mT^*$. On the theoretical side, by a careful generalization of the truncation argument and $\psi_{(2/d)}$-norm concentration inequality, we can similarly show under mild conditions, when $n\geq C(\log n)^d(s\log p)^{d/2}$, the proposed procedure achieves the following rate of convergence with high probability,
\begin{equation*}
\left\|\tilde{\mT} - \mT^*\right\|_F^2\lesssim \sigma^2\frac{Kds\log (p/s)}{n},
\end{equation*}
where $C>0$ is some constant which does not depend on $n, p, K$, and $\sigma^2$. The minimax optimality can be shown similarly. %In terms of sample complexity, both $\log n$ from truncation and $(s\log p)^{1/2}$ from tensor parameter complexity grow with the order of underlying tensor.

\begin{comment}
In addition, we only provide a possible way to express interaction effect model into a tensor recovery formulation in this work. We believe it may have wider applications if we consider more complicated structure. Varying-coefficient model \citep{hastie1993varying, fan2008statistical} is a good potential model to incorporate tensor reformation. The varying-coefficient models assume the form of multivariate regression function as 
\begin{equation*}
m(\bU, \bX) = \bX^{\top}\ba(\bU),
\end{equation*}
for some unknown functional coefficient $\ba(\bU)$. This model permits nonlinear interactions between $\bU$ and $\bX$. By some basis function expansions of non-parameter function $\ba$, we can express the varying-coefficient model as a series of different order interaction terms. Therefore, the tensor reformulation and estimation technique are applicable. {\red (This discussion paragraph is quite confusing at this moment. Are you able to make it clearer? If it takes much efforts, we can just remove and save it for the future use.)}
\end{comment}

==> t-cubic-sketch6-proof.tex <==

%%%%%%%%%%%%%%%%
\section{Proofs}\label{sec:proof}
%%%%%%%%%%%%%%%%
In this section, we provide detailed proofs for empirical moment estimator and concentration results in Sections \ref{sec:moment_calculation} and \ref{subsec:concentration}. %(ii) Theorems \ref{thm:symmetric_main} and \ref{thm:initial_symmetric} in Sections \ref{subsec:proof_ini} and \ref{subsec:gradient-update-proof}. 	
	
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Moment Calculation} \label{sec:moment_calculation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	
	
We first introduce three lemmas to show that the empirical moment based tensors \eqref{eqn:moment_tensor_sym}, \eqref{eqn:moment_inter}, and \eqref{eq:moment_asy} are all unbiased estimators for the target low-rank tensor in the corresponding scenarios. Detail proofs of three lemmas are postponed to Sections \ref{proof_moment_asy}, \ref{proof_moment_sym} and \ref{proof_moment_inter} in the supplementary materials.
	\begin{Lemma}[(Unbiasedness of moment estimator under non-symmetric sketchings)]
		\label{lemma:moment_asy}
		For non-symmetric tensor estimation model \eqref{eq:model_asymmetric} \& \eqref{eq:low_rank_nonsym}, define the empirical-moment-based tensor $\cT$ by
		$$\cT:=\frac{1}{n}\sum_{i=1}^n y_i \bu_i\circ \bv_i\circ \bw_i.$$ Then $\cT$ is an unbiased estimator for $\mT^*$, i.e.,
		\begin{eqnarray*}
			\mathbb E(\cT) = \sum_{k=1}^K\eta_k^*\bbeta_{1k}^*\circ\bbeta_{2k}^*\circ\bbeta_{3k}^*.
		\end{eqnarray*}
	\end{Lemma}
	%The construction of empirical moment based tensor for symmetric case needs an additional first-order moment based term. It could remove the bias caused by the symmetric structure.
	The extension to the symmetric case is non-trivial due to the dependency among three identical sketching vectors. We borrow the idea of high-order Stein's identity, which was originally proposed in \cite{janzamin2014score}. To fix the idea, we present only third order result for simplicity. The extension to higher-order is straightforward.
	\begin{Theorem}[(Third-order Stein's Identity, \citep{janzamin2014score})] \label{thm:steins_higher}
		Let $\bx \in \mathbb{R}^{p}$ be a random vector with joint density function $p(\bx)$. Define the third order score function $\cS_3(\bx):\mathbb R^p\rightarrow \mathbb R^{p\times p \times p}$ as $\cS_3(\bx) = -\nabla^{3}p(\bx)/p(\bx)$. Then for continuously differentiable function $G(\bx):\mathbb{R}^{p} \rightarrow \mathbb{R}$, %satisfying some regularity conditions, 
		we have
		\begin{equation}\label{eqn:stein_identity}
		\mathbb E \left[ G(\bx) \cdot \cS_3(\bx) \right] = \mathbb E \left[ \nabla^{3} G(\bx) \right].
		\end{equation}
	\end{Theorem}
	In general, the order-$m$ high-order score function is defined as
	\begin{equation*} 
	\cS_m(\bx)=(-1)^m \frac{\nabla^{m} p(\bx)}{p(\bx)}.
	\end{equation*}
	Interestingly, the high-order score function has a recursive differential representation   
	\begin{equation}\label{eqn:recursive_form}
	\cS_m(\bx):=-\cS_{m-1}(\bx)\circ \nabla\log p(\bx)-\nabla \cS_{m-1}(\bx),
	\end{equation}
	with $\cS_0(\bx) = 1$. This recursive form is helpful for constructing unbiased tensor estimator under symmetric cubic sketchings. Note that the first order score function $\cS_1(\bx)=-\nabla \log p(\bx)$ is the same as score function in Lemma \ref{lemma:stein_lemma} (Stein's lemma \citep{stein2004use}).  The proof of Theorem \ref{thm:steins_higher} relies on iteratively applying the recursion representation of score function \eqref{eqn:recursive_form} and the first-order Stein's lemma (Lemma  \ref{lemma:stein_lemma}). We provide the detailed proof in Section \ref{proof:stein_higher} for the sake of completeness.
	
	In particular, if $\bx$ follows a standard Gaussian vector, each order score function can be calculated based on \eqref{eqn:recursive_form} as follows,
	\begin{equation}\label{eqn:S_x}
	\begin{split}
	&\cS_1(\bx) = \bx, \cS_2(\bx) = \bx\circ \bx -I_{d\times d},\\
	&\cS_3(\bx) = \bx\circ \bx\circ \bx - \sum_{j=1}^p\Big(\bx\circ \be_j\circ \be_j+ \be_j\circ \bx \circ \be_j+\be_j\circ \be_j\circ \bx\Big).
	\end{split}
	\end{equation}
	Interestingly, if we let $G(\bx) = \sum_{k=1}^K\eta_k^*(\bx^{\top}\bbeta_k^*)^3$, then 
	\begin{equation}\label{eqn:G_x}
	\frac{1}{6}\nabla^{3} G(\bx) = \sum_{k=1}^K\eta_k^*\bbeta_k^*\circ \bbeta_k^* \circ \bbeta_k^*,
	\end{equation}
	 which is exactly $\mT^*$. Connecting this fact with \eqref{eqn:stein_identity}, we are able to construct the unbiased estimator in the following lemma through high-order Stein's identity.	
	
	
	
	
	
	
	\begin{Lemma}[(Unbiasedness of moment estimator under symmetric sketchings)]
		\label{lemma:moment_symmetric}
		Consider the symmetric tensor estimation model \eqref{eq:model} \& \eqref{eq:mathcal_F_symmetric}. Define the empirical first-order moment $\boldsymbol{m}_1 :=\frac{1}{n}\sum_{i=1}^n y_i\bx_i$.
		If we further define an empirical third-order-moment-based tensor $\cT_s$ by
		$$\cT_s:= \frac{1}{6}\Big[\frac{1}{n}\sum_{i=1}^n y_i \bx_i\circ \bx_i\circ \bx_i - \sum_{j=1}^p\Big(\boldsymbol{m}_1\circ \be_j\circ \be_j+ \be_j\circ \boldsymbol{m}_1 \circ \be_j+\be_j\circ \be_j\circ \boldsymbol{m}_1\Big)\Big],
		$$
		then
		\begin{eqnarray*}
			\mathbb E(\cT_s) = \sum_{k=1}^K\eta_k^*\bbeta_{k}^*\circ\bbeta_{k}^*\circ\bbeta_{k}^*.
		\end{eqnarray*}
	\end{Lemma}
	\emph{Proof.} Note that $y_i=G(\bx_i) +\epsilon_i$. Then we have
	\begin{equation*}
	\mathbb E\Big(\frac{1}{n}\sum_{i=1}^{n}y_i\cS_3(\bx)\Big) = \mathbb E\Big(\frac{1}{n}\sum_{i=1}^{n}(G(\bx_i)+\epsilon_i)\cS_3(\bx_i)\Big),
	\end{equation*}
	where $\cS_3(\bx)$ is defined in \eqref{eqn:S_x}. By using the conclusion in Theorem \ref{thm:steins_higher} and the fact \eqref{eqn:G_x}, we obtain
	\begin{equation*}
	\mathbb E(\cT_s) = \mathbb E\Big(\frac{1}{6n}\sum_{i=1}^{n}y_i\cS_3(\bx)\Big) = \sum_{k=1}^K\eta_k^*\bbeta_{k}^*\circ\bbeta_{k}^*\circ\bbeta_{k}^*,
	\end{equation*}
	since $\epsilon_i$ is independent of $\bx_i$. This ends the proof. \hfill $\blacksquare$\\

	
	Although the interaction effect model \eqref{eq:interaction_model} is still based on symmetric sketchings, we need much more careful construction for the moment-based estimator, since the first coordinate of the sketching vector is always constant 1. We give such an estimator in the following lemma.%Comparing to the Gaussian random vector, it's non-random and non-centered. We need much more careful actions to construct the unbiased estimator in  the interaction effect model. 
	\begin{Lemma}[(Unbiasedness of moment estimator in interaction model)]
		\label{lemma:moment_interaction}
		For interaction effect model \eqref{eq:interaction_model}, construct the empirical moment based tensor $\cT_{s'}$ as following 
	\begin{itemize}
		\item For $i,j,k\neq 0$, $\cT_{s'[i,j,k]} = \cT_{s[i,j,k]}$. And $\cT_{s'[i,j,0]} = \cT_{s[i,j,0]}, \cT_{s'[0,j,k]} = \cT_{s[0,j,k]}, \cT_{s'[i,0,k]} = \cT_{s[i,0,k]}$.
		\item For $i\neq 0$, $\cT_{s'[0,0,i]} = \cT_{s'[ 0, i, 0]} = \cT_{s'[i,0,0]} = \frac{1}{3}\cT_{s[0,0,i]} - \frac{1}{6}(\sum_{k=1}^p\cT_{s[k,k,i]}-(p+2)a_i)$.
		\item $\cT_{s'[0,0,0]} = \frac{1}{2p-2}(\sum_{k=1}^p\cT_{s[0,k,k]} - (p+2)\cT_{s[0,0,0]})$. 
	\end{itemize}
		The $\cT_{s'}$ is an unbiased estimator for $\mathcal{B}$, i.e.,
		\begin{eqnarray*}
			\mathbb E(\cT_{s'}) = \sum_{k=1}^K\eta_k\bbeta_{k}\circ\bbeta_{k}\circ\bbeta_{k}.
		\end{eqnarray*}
	\end{Lemma}
	%Now we have constructed three empirical moment based initial tensor $\cT,\cT_s,\cA$ for three different scenarios.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proofs of Lemmas \ref{cor:concentr_high_order} and \ref{lemma:tensor_spectral}: Concentration Inequalities}\label{subsec:concentration}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We aim to prove Lemmas \ref{cor:concentr_high_order} and \ref{lemma:tensor_spectral} in this subsection. These two lemmas provide key concentration inequalities of the theoretical analysis for the main result. Before going into technical details, we introduce a quasi-norm called $\psi_{\alpha}$-norm.
%The first Lemma \ref{lemma:sum_psi_norm} characterizes the concentration behavior of high-order sub-Gaussian random variables by $\psi_{\alpha}$-norm. The second Lemma \ref{lemma:tensor_spectral} discusses a concentration inequality in tensor spectral norm in a sparse scenario. Those results are the core technique tools to establish the convergence rate for our final estimators. 

%In this subsection, we present two types of novel concentration inequalities.  The first Lemma \ref{lemma:sum_psi_norm} characterizes the concentration behavior of high-order sub-Gaussian random variables by $\psi_{\alpha}$-norm. The second Lemma \ref{lemma:tensor_spectral} discusses a concentration inequality in tensor spectral norm in a sparse scenario. Those results are the core technique tools to establish the convergence rate for our final estimators. 

%Before presenting the result for bounding high-order sub-Gaussian random variables, we introduce a quasi-norm called $\psi_{\alpha}$-norm for random variables (also see Section 2 in \cite{ALPT2011}).
\begin{Definition}[($\psi_{\alpha}$-norm \citep{ALPT2011})]
	The $\psi_{\alpha}$-norm of any random variable $X$ and $\alpha>0$ is defined as
	\begin{eqnarray*}
		\|X\|_{\psi_{\alpha}}:=\inf\Big\{C\in(0, \infty): ~ \mathbb E[\exp(|X|/C)^{\alpha}]\leq 2\Big\}.
	\end{eqnarray*}
\end{Definition}
Particularly, a random variable who has a bounded $\psi_2$-norm or bounded $\psi_1$-norm is called sub-Gaussian or sub-exponential random variable, respectively. %Additionally, the $\psi_{\alpha}$-norm of any random variable can be bounded by its moments: if $X$ satisfies $\mathbb E^{1/p}|X|^p\leq p^{1/\alpha}K$ for any $p\geq 1$ and some $K>0$, then $\|X\|_{\psi_{\alpha}}\leq c_{\alpha}K$, where $c_{\alpha}$ is a positive constant depending on only $\alpha$. The inverse argument is also true. 
Next lemma provides an upper bound for the $p$-th moment of sum of random variables with bounded $\psi_{\alpha}$-norm.
\begin{Lemma}\label{lemma:psi_moment_bound}
	Suppose $X_1,\ldots, X_n$ are $n$ independent random variables satisfying $\|X_i\|_{\psi_{\alpha}}\leq b$ with $\alpha> 0$, then for all $\ba=(a_1,\ldots, a_n)\in\mathbb R^n$ and $p\geq 2$,
	\begin{eqnarray}\label{eqn:psi_moment_bound}
	&&\Big(\mathbb E\Big|\sum_{i=1}^na_i X_i-\mathbb E(\sum_{i=1}^na_iX_i)\Big|^p\Big)^{\tfrac{1}{p}}\nonumber\\
	&\leq&
	\left\{\begin{array}{ll}
	C_1(\alpha)b\big(\sqrt{p}\|\ba\|_2+p^{1/\alpha}\|\ba\|_{\infty}\big), & \text{ if } 0<\alpha<1;\\
	C_2(\alpha)b\big(\sqrt{p}\|\ba\|_2+p^{1/\alpha}\|\ba\|_{\alpha^*}\big), & \text{ if } \alpha\geq 1.\\	
	\end{array}\right.
	\end{eqnarray}
	where $1/\alpha^*+1/\alpha = 1$, $C_1(\alpha),C_2(\alpha)$ are some absolute constants only depending on $\alpha$.
\end{Lemma}
%The proof of Lemma \ref{lemma:psi_moment_bound} starts from a symmetric random variable with bounded $\psi_{\alpha}$-norm. 






If $0<\alpha<1$, \eqref{eqn:psi_moment_bound} is a combination of Theorem 6.2 in \cite{HMO1997} and the fact that the $p$-th moment of a Weibull variable with parameter $\alpha$ is of order $p^{1/\alpha}$. If $\alpha\geq 1$, \eqref{eqn:psi_moment_bound} follows from a combination of Corollaries 2.9 and 2.10 in \cite{talagrand1994supremum}. Continuing with standard symmetrization arguments, we reach the conclusion for general random variables. When $\alpha=1$ or 2, \eqref{eqn:psi_moment_bound} coincides with standard moment bounds for a sum of sub-Gaussian and sub-exponential random variables in \cite{RV12}. The detailed proof of Lemma \ref{lemma:psi_moment_bound} is postponed to Section \ref{proof_psi_moment_bound}.


When $0<\alpha<1$, by Chebyshev's inequality, one can obtain the following exponential tail bound for the sum of random variables with bounded $\psi_{\alpha}$-norm. This lemma generalizes the Hoeffding-type concentration inequality for sub-Gaussian random variables (see, e.g. Proposition 5.10 in \cite{RV12}), and Bernstein-type concentration inequality for sub-exponential random variables (see, e.g. Proposition 5.16 in \cite{RV12}).
\begin{Lemma}\label{lemma:orlicz_concentra}
	Suppose $0<\alpha<1$, $X_1,\ldots, X_n$ are independent random variables satisfying $\|X_i\|_{\psi_{\alpha}}\leq b$. Then there exists absolute constant $C(\alpha)$ only depending on $\alpha$ such that for any $\ba=(a_1,\ldots,a_n)\in \mathbb R^n$ and $0<\delta<1/e^2$,
	\begin{eqnarray*}
		\Big|\sum_{i=1}^na_iX_i-\mathbb E(\sum_{i=1}^na_iX_i)\Big|\leq C(\alpha)b\|\ba\|_2(\log\delta^{-1})^{1/2}+C(\alpha)b\|\ba\|_{\infty}(\log \delta^{-1})^{1/\alpha}
	\end{eqnarray*}
	with probability at least $1-\delta$.
\end{Lemma}
% Lemma \ref{lemma:orlicz_concentra} provides concentration results for bounded $\psi_{\alpha}$-norm random variables with $0<\alpha<1$. 

\emph{Proof.} For any $t>0$, by Markov's inequality,
\begin{equation*}
\begin{split}
&\mathbb P\Big(\Big|\sum_{i=1}^n a_iX_i-\mathbb E\Big(\sum_{i=1}^na_iX_i\Big)\Big|\geq t \Big)=\mathbb P\Big(\Big|\sum_{i=1}^n a_iX_i-\mathbb E\Big(\sum_{i=1}^na_iX_i\Big)\Big|^p\geq t^p \Big)\\
\leq& \frac{\mathbb E\Big|\sum_{i=1}^n a_iX_i-\mathbb E\Big(\sum_{i=1}^na_iX_i\Big)\Big|^p}{t^p}\leq \frac{C(\alpha)^pb^p\Big(\sqrt{p}\|\ba\|_2+p^{1/\alpha}\|\ba\|_{\infty}\Big)^p}{t^p},
\end{split}
\end{equation*}
where the last inequality is from Lemma \ref{lemma:psi_moment_bound}. We set $t$ such that $\exp(-p) =C(\alpha)^pb^p(\sqrt{p}\|\ba\|_2+p^{1/\alpha}\|\ba\|_{\infty})^p/t^p$. Then for $p\geq 2$,
\begin{equation*}
    \Big|\sum_{i=1}^n a_iX_i-\mathbb E\Big(\sum_{i=1}^na_iX_i\Big)\Big|\leq eC(\alpha)b\Big(\sqrt{p}\|\ba\|_2+p^{1/\alpha}\|\ba\|_{\infty}\Big)
\end{equation*}
holds with probability at least $1-\exp(-p)$. Letting $\delta= \exp(-p)$, we have that for any $0<\delta<1/e^2$,
\begin{equation*}
    \Big|\sum_{i=1}^n a_iX_i-\mathbb E\Big(\sum_{i=1}^na_iX_i\Big)\Big|\leq C(\alpha)b\Big(\|\ba\|_2(\log\delta^{-1})^{1/2}+\|\ba\|_{\infty}(\log \delta^{-1})^{1/\alpha}\Big),
\end{equation*}
holds with probability at least $1-\delta$. This ends the proof. \hfill $\blacksquare$


The next lemma provides an upper bound for the product of random variables in $\psi_{\alpha}$-norm.
\begin{Lemma}[($\psi_{\alpha}$ for product of random variables)]\label{lemma:sum_psi_norm}
	Suppose $X_1,\ldots, X_m$ are $m$ random variables (not necessarily independent) with $\psi_{\alpha}$-norm bounded by $\|X_j\|_{\psi_{\alpha}}\leq K_j$. Then the $\psi_{\alpha/m}$-norm of $\prod_{j=1}^mX_j$ is bounded as $$\left\|\prod_{j=1}^m X_j\right\|_{\psi_{\alpha/m}}\leq\prod_{j=1}^m K_j.$$ 
\end{Lemma}
\emph{Proof.} For any $\{x_j\}_{j=1}^m$ and  $\alpha>0$, by using the inequality of arithmetic and geometric means we have
\begin{equation*}
\Big(|\prod_{j=1}^m\frac{x_j}{K_j}|\Big)^{\alpha/m} = \Big(\prod_{j=1}^m|\frac{x_j}{K_j}|^{\alpha}\Big)^{1/m}\leq \frac{1}{m}\sum_{j=1}^m|\frac{x_j}{K_j}|^{\alpha}.
\end{equation*} 
Since exponential function is a monotone increasing function, it shows that
\begin{equation}\label{eqn:psi_1}
\begin{split}
&\exp\Big(|\prod_{j=1}^m\frac{x_j}{K_j}|\Big)^{\alpha/m}\leq  \exp\Big(\frac{1}{m}\sum_{j=1}^m|\frac{x_j}{K_j}|^{\alpha}\Big)\\
& = \Big(\prod_{j=1}^m \exp (|\frac{x_j}{K_j}|^{\alpha})\Big)^{1/m}\leq \frac{1}{m}\sum_{j=1}^m\exp\Big(|\frac{x_j}{K_j}|^{\alpha}\Big).
\end{split}
\end{equation}
From the definition of $\psi_{\alpha}$-norm, for $j=1,2,\ldots,m$, each individual $X_j$ has 
\begin{equation}\label{eqn:psi_2}
\mathbb E\Big(\exp(\frac{|X_j|}{K_j})^{\alpha}\Big)\leq 2.
\end{equation}
Putting \eqref{eqn:psi_1} and \eqref{eqn:psi_2} together, we obtain
\begin{equation*}
\begin{split}
	&\mathbb E\Big[\exp\Big(|\frac{\prod_{j=1}^mX_j}{\prod_{j=1}^mK_j}|\Big)^{\alpha/m}\Big] = \mathbb E\Big[\exp\Big(|\prod_{j=1}^m\frac{X_j}{K_j}|\Big)^{\alpha/m}\Big]\\
	&\leq \frac{1}{m}\sum_{j=1}^m\mathbb E\Big[\exp\Big(|\frac{X_j}{K_j}|\Big)^{\alpha}\Big]\leq 2.
	\end{split}
\end{equation*}
Therefore, we conclude that the $\psi_{\alpha/m}$-norm of $\prod_{j=1}^mX_j$ is bounded by $\prod_{j=1}^mK_j$.  \hfill $\blacksquare$\\

\emph{Proof of Lemma \ref{cor:concentr_high_order}.} 
%the combination of Lemmas \ref{lemma:orlicz_concentra} and \ref{lemma:sum_psi_norm} implies Lemma \ref{cor:concentr_high_order}. 
Note that for any $j=1,2,\ldots, m$, the $\psi_2$-norm of $\bX_j^{\top}\bbeta_j$ is bounded by $\|\bbeta_j\|_2$ \citep{RV12}. According to Lemma \ref{lemma:sum_psi_norm}, the $\psi_{2/m}$-norm of $\prod_{j=1}^m(\bX_j^{\top}\bbeta_j)$ is bounded by $\prod_{j=1}^m\|\bbeta_j\|_2$. Directly applying Lemma \ref{lemma:orlicz_concentra}, we reach the conclusion.
\hfill $\blacksquare$\\


\emph{Proof of Lemma \ref{lemma:tensor_spectral}.}  We first focus on the non-symmetric version and the proof follows three steps:
\begin{enumerate}
	\item Truncate the first coordinate of $\bx_{1i}, \bx_{2i}, \bx_{3i}$ by a carefully chosen truncation level;
	\item Utilize the high-order concentration inequality in Lemma \ref{lemma:tensor_concentration} at order three;
	\item Show that the bias caused by truncation is negligible. 
\end{enumerate}

With slightly abuse of notations, we denote $a,x,y$ etc. as their \emph{first coordinate} of $\ba,\bx,\by$ etc.  Without loss of generality, we assume $p:=\max\{p_1,p_2,p_3\}$. By unitary invariance, we assume $\bbeta_1=\bbeta_2=\bbeta_3=\be_1$, where $\be_1 = (1,0,\ldots,0)^{\top}$. Then, it is equivalent to prove
\begin{eqnarray*}
	&&\Big\|M_{\text{nsy}} - \mathbb E(M_{\text{nsy}})\Big\|_s =\Big\|\frac{1}{n}\sum_{i=1}^nx_{1i}x_{2i}x_{3i}\bx_{1i}\circ\bx_{2i}\circ\bx_{3i}-\be_1\circ\be_1\circ\be_1\Big\|_{s}\\
	&\leq&  C(\log n)^3\Big(\sqrt{\frac{s^3\log^3 (p/s)}{n^2}} + \sqrt{\frac{s\log (p/s)}{n}}\Big) .
\end{eqnarray*}

Suppose $\bx_1\sim \cN(0, \bI_{p_1}), \bx_2\sim \cN(0, \bI_{p_2}), \bx_3\sim \cN(0, \bI_{p_3})$ and $\{\bx_{1i}, \bx_{2i}, \bx_{3i}\}_{i=1}^n$ are $n$ independent samples of $\{\bx_1, \bx_2, \bx_3\}$. And define a bounded event $\cG_n$ for the first coordinate and its corresponding population version,
\begin{eqnarray*}
	\cG_n=\{\max_{i}\{|x_{1i}|,|x_{2i}|, |x_{3i}|\}\leq M \},
	\cG=\{\max\{|x_1|,|x_2|, |x_3|\}\leq M\},
\end{eqnarray*}
where $M$ is a large constant to be specified later. Decomposing $\|M_{\text{nsy}} - \mathbb E(M_{\text{nsy}})\|_s$ as 
\begin{equation*}
\begin{split}
	&\Big\|M_{\text{nsy}} - \mathbb E(M_{\text{nsy}})\Big\|_s\\
	&\leq\underbrace{\Big\|\frac{1}{n}\sum_{i=1}^nx_{1i}x_{2i}x_{3i}\bx_{1i}\circ\bx_{2i}\circ\bx_{3i}-\mathbb E\Big(x_1x_2x_3\bx_1\circ\bx_2\circ\bx_3\big|\cG\Big)\Big\|_{s}}_{M_1:\text{main term}}\\
	&+\underbrace{\Big\|\mathbb E\Big(x_1x_2x_3\bx_1\circ\bx_2\circ\bx_3\big|\cG\Big)-\be_1\circ\be_1\circ\be_1\Big\|_{s}}_{M_2:\text{bias term}},\nonumber
\end{split}
\end{equation*}
 we will prove that $M_2$ is negligible in terms of convergence rate of $M_1$. 

\textbf{Bounding $M_1$.} For simplicity, we define
$\bx_{1}' = \bx_{1}| \cG, \ \bx_{2}' = \bx_{2}|\cG , \ \bx_{3}' = \bx_{3}| \cG
$, and $\{\bx_{1i}',\bx_{2i}', \bx_{3i}'\}_{i=1}^n$ are $n$ independent samples of $\{\bx_1', \bx_2', \bx_3'\}$. According to the law of total probability, we have
\begin{equation*}
\begin{split}
	&\mathbb P\Big(M_1\geq t\Big)\leq \mathbb P\Big(\cG_n^c\Big)\\
	&+ \mathbb P\Big(\underbrace{\Big\|\frac{1}{n}\sum_{i=1}^nx_{1i}'\bx_{1i}'\circ x_{3i}'\bx_{2i}'\circ x_{i1}'\bx_{3i}'-\mathbb E\Big(x_1'\bx_1'\circ x_2'\bx_2'\circ x_3'\bx_3'\Big)\Big\|_{s}}_{M_{11}}\geq t\Big).
	\end{split}
\end{equation*}
According to Lemma \ref{lemma:bounded_gaussian}, the entry of $x_{1i}'\bx_{1i}', x_{2i}'\bx_{2i}', x_{3i}'\bx_{3i}'$ are sub-Gaussian random variable with $\psi_2$-norm $M^2$. Applying Lemma \ref{lemma:tensor_concentration}, we obtain
\begin{eqnarray*}
	\mathbb P\Big(M_{11}\geq C_1M^{6}\delta_{n,s}\Big)\leq \frac{1}{p},
\end{eqnarray*}
where $\delta_{n,s} = ((s\log(p/s))^{3}/n^2)^{1/2}+(s\log(p/s)/n)^{1/2}$.

On the other hand, 
\begin{eqnarray*}
	\mathbb P(\cG_n^c)\leq 3\sum_{i=1}^n \mathbb P(|x_{1i}|\geq M)\leq 3ne^{1-C_2M^2}
\end{eqnarray*}
Putting the above bounds together, we obtain
\begin{eqnarray*}
	\mathbb P\Big(M_1\geq C_1 M^6 \delta_{n,s}\Big)\leq 1/s+3n e^{1-C_2M^2}.
\end{eqnarray*}
%The choice of $M$ should be possible but meanwhile keep the right side probability diverging. Thus, the best possible choice of $M$ is of order $\sqrt{\log n}$. 
By setting $M=2\sqrt{\log n/C_2}$, the bound of $M_1$ reduces to
\begin{eqnarray}
\label{bound_M1}
\mathbb P\Big(M_1\geq \frac{64C_1}{C_2^3}\delta_{n,s}(\log n)^3\Big)\leq \frac{1}{p}+\frac{3e}{n^3}.
\end{eqnarray}

\textbf{Bounding $M_2$.} There exists $ \varrho \in \mathbb S^{p-1}$ such that
\begin{eqnarray*}
	M_2 = \Big|\mathbb E\Big(x_1x_2x_3(\bx_1^{\top}\varrho)(\bx_2^{\top}\varrho)(\bx_3^{\top}\varrho)\Big|\cG\Big)-\big(\be_1^{\top}\varrho\big)^3\Big|.
\end{eqnarray*}
Since $x_{1j}$ is independent of $x_{1k}$ for any $j\neq k$, $\mathbb E(x_1(\bx_1^{\top}\varrho)|\cG) = \mathbb E(x_1^2\varrho_1|\cG)$. Then
\begin{eqnarray*}
	M_2&=&\Big|\mathbb E\Big(x_1^2x_2^2x_3^2\varrho_1^3\Big|\cG\Big)-\varrho_1^3\Big|\\
	&=&\Big|\varrho_1^3\mathbb E\Big(x_1^2\Big||x_1|\leq M\Big) \mathbb E\Big(x_2^2\Big||x_2|\leq M\Big) \mathbb E\Big(x_3^2\Big||x_3|\leq M\Big)-\varrho_1^3\Big|,
\end{eqnarray*}
where the second equation comes from the independence among each coordinate of $\{\bx_{1i}, \bx_{2i}, \bx_{3i}\}$. 

By the basic property of Gaussian random variable, we can show
\begin{eqnarray*}
	1\geq \mathbb E\Big(x_i^2\big||x_i|\leq M\Big)\geq 1-2Me^{-M^2/2} ,\quad  i=1,2,3.
\end{eqnarray*}
Plugging them into $M_2$, we have
\begin{eqnarray*}
	M_2 &\leq& \big|\varrho_1^3\big|\Big|\Big(1-2Me^{-M^2/2}\Big)^3-1\Big|\\
	&\leq& \Big|12M^2e^{-M^2}-6Me^{-M^2/2}-8M^3e^{-3M^2/2}\Big|\\
	&\leq& \Big|26M^3e^{-M^2/2}\Big|,
\end{eqnarray*}
where the second inequality is due to $\|\varrho\|_2^2=1$ and the last inequality holds for a large $M>0$.
By the choice of $M=2\sqrt{\log n/C_2}$, we have $M_2\leq 208/C_2^{3/2}(\log n)^{\frac{3}{2}}/n^2$ for some constant $C_2$. When $n$ is large, this rate is negligible comparing with \eqref{bound_M1}

\textbf{Bounding $M$:} We put the upper bounds of $M_1$ and $M_2$ together. After some adjustments for absolute constant, it suffices to obtain
\begin{eqnarray*}
	\mathbb P\Big(M_1+M_2\leq C(\log n)^3\Big(\sqrt{\frac{s^3\log^3 (p/s)}{n^2}} + \sqrt{\frac{s\log (p/s)}{n}}\Big)\Big)\geq 1- \frac{10}{n^3}.
\end{eqnarray*}
This concludes the proof of non-symmetric part. The proof of symmetric part remains similar and thus is omitted here.
\hfill $\blacksquare$\\

%The proof of Lemma \ref{lemma:tensor_spectral} is a combination of truncation argument, $\psi_{2/3}$-norm and $\varepsilon$-net on the discretized sparse set. The extra $(\log n)^3$ is contributed by the truncation step. The detailed proof of Lemma \ref{lemma:tensor_spectral} is postponed to Section \ref{subsec:proof_concentration} in the supplemental material. (To ensure the upper bound non-trivial, we require $n\geq C (s\log(p/s))^{\tfrac{3}{2}}$ for some large constant $C$. Only if $n\geq C(s\log (p/s))^2$, this spectral norm bound can achieve optimal statistical rate.)






==> t-cubic-sketch7-appen.tex <==




\newpage
\clearpage


%\setcounter{page}{1}
\setcounter{subsection}{0}
\renewcommand{\thesubsection}{S.\Roman{subsection}}
\setcounter{equation}{0}
\renewcommand{\theequation}{S.\arabic{equation}}
\setcounter{theorem}{0}
\renewcommand{\thetheorem}{S.\arabic{theorem}}
\renewcommand{\thelemma}{S.\arabic{lemma}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{center}
	\title{\Large Supplement to ``Sparse and Low-Rank Tensor Estimation via Cubic Sketchings"}
\end{center}

\medskip
\begin{center}
	Botao Hao\footnote{Ph.D student, Department of Statistics, Purdue University, West Lafayette, IN 47906. E-mail: hao22@purdue.edu.},~
	Anru Zhang\footnote{Assistant Professor, Department of Statistics, University of Wisconsin-Madison, Madison, WI 53706. E-mail: anruzhang@stat.wisc.edu.},~
	Guang Cheng\footnote{Professor, Department of Statistics, Purdue University, West Lafayette, IN 47906. E-mail: chengg@purdue.edu. Research Sponsored by NSF CAREER Award DMS-1151692, DMS-1418042, DMS-1712907 and Office of Naval Research ONR N00014-15-1-2331.}
\end{center}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\appendix
\bigskip



This supplementary contains five parts: (1) Section \ref{supp_sec:additional-proofs-main} provides additional proofs for the main theoretical results of this paper; (2) Section \ref{supp_sec:proof} contains detailed proofs for the theoretical developments in the main theorems; (3) Section \ref{sec:non_symmetric} covers the pseudo-code, conditions and main proofs of non-symmetric tensor estimation; (4) Section \ref{supp_sec:sgd} discusses the matrix form of gradient function and stochastic gradient descent; (5) Section \ref{sec:tech_lemma} provides several technical lemmas and their proofs.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Additional Proofs for main results}\label{supp_sec:additional-proofs-main}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proof of Theorem \ref{thm:initial_symmetric}: Initialization Effect}\label{subsec:proof_ini}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Theorem \ref{thm:initial_symmetric} gives an approximation error upper bound for the sparse-tensor-decomposition-based initial estimator. %To provide such theoretical guarantee, we propose a symmetric sparse eigenvalue decomposition in (\ref{alg:sparse_svd_sym}).  %we need a slightly better starting point than random starting. In this paper, 
%This could be used as the starting point to guarantee the theoretical performance of sparse tensor decomposition. 
%By using sparse eigenvalue decomposition as a starting point for tensor decomposition, we can present theoretical guarantee for symmetric sparse tensor decomposition. 
In Step I of Section \ref{sec:procedure-symmetric}, the original problem can be reformatted to a version of tensor denoising:
\begin{eqnarray}
\label{eqn:denoising_model}
\cT_s = \mT^*+\cE, \quad\text{where} \quad \cE = \cT_s - \mathbb E(\cT_s).
\end{eqnarray}
The key difference between our model \eqref{eqn:denoising_model} and recent work is that $\cE$ arises from empirical moment approximation, rather than the random observation noise considered in \cite{AGJ14} and \cite{Sun2016}. %In general, the observation error is hard to quantify without any specific assumption. 
Next lemma gives an upper bound for the approximation error.
\begin{Lemma}[(Approximation error of $\mathcal{T}_s$)]\label{lemma:perturbation_analysis}
	Recall that $\cE = \cT_s - \mathbb E(\cT_s)$, where $\cT_s$ is defined in (\ref{eqn:moment_tensor_sym}). Suppose Condition \ref{con:noise} is satisfied and $s\leq d \leq Cs$. Then
	\begin{eqnarray}\label{ineq:perturbation_error}
	\|\cE\|_{s+d} &\leq& 2C_1 \sum_{k=1}^K\eta_k^*\Big(\sqrt{\frac{s^3\log^3(p/s)}{n^2}}+\sqrt{\frac{s\log(p/s)}{n}}\Big)(\log n)^4
	\end{eqnarray}
	with probability at least $1-5/n$ for some uniform constant $C_1$. 
\end{Lemma}
%The proof of Lemma \ref{lemma:perturbation_analysis} is deferred to Section \ref{proof_perturbation}. This lemma illustrates the convergence rate of approximation error $\cE$. As long as the sample size is of order $\cO(K^2s^2)$, this error can be controlled.

Next we denote the following quantity for simplicity,
\begin{eqnarray}\label{def:gamma}
\gamma = C_2\min\Big\{\frac{R^{-1}}{6}-\frac{\sqrt{K}}{s}, \frac{R^{-1}}{4\sqrt{5}}-\frac{2}{\sqrt{s}}\Big(1+\sqrt{\frac{K}{s}}\Big)^2\}, %\ \varepsilon_R = \frac{D_2}{\eta_{\min}^*}\|\cE\|_{s+d} + \sqrt{K}\Gamma^2,
\end{eqnarray}
where $R$ is the singular value ratio, $K$ is the CP-rank, $s$ is the sparsity parameter, $\Gamma$ is the incoherence parameter and $C_2$ is uniform constant. 

Next lemma provides theoretical guarantees for sparse tensor decomposition method.
\begin{Lemma}\label{lemma:ini_sym}
	Suppose that the symmetric tensor denoising model (\ref{eqn:denoising_model}) satisfies Conditions \ref{con:ident}, \ref{con:parameter} and \ref{con:incoherence_sym} (i.e., the identifiability, parameter space and incoherence). Assume the number of initializations $L \geq K^{C_3\gamma^{-4}}$ and the number of iterations $N\geq C_4\log \left(\gamma/\left(\frac{1}{\eta_{\min}^*}\|\cE\|_{s+d} + \sqrt{K}\Gamma^2\right)\right)$ for constants $C_3,C_4$, the truncation parameter $s\leq d \leq Cs$. Then the sparse-tensor-decomposition-based initialization satisfies 
	\begin{eqnarray}
	\label{ineq:initial_error}
	\max\left\{\|\bbeta_k^{(0)} - \bbeta_k^*\|_2, |\eta_k^{(0)} - \eta_k^*|\right\}\leq  \frac{C_4}{\eta_{\min}^*}\|\cE\|_{s+d} + \sqrt{K}\Gamma^2,
	\end{eqnarray}
	for any $k\in[K]$.
\end{Lemma}

%Similar conclusions for non-symmetric version was provided in \cite{Sun2016}. We omit the detail proof here since there is no big difference in proof for symmetric and non-symmetric case for this lemma. 
%\Botao{Note that \eqref{ineq:initial_error} is kind of deterministic result since all the randomness are absorbed into approximation error $\cE$.} 
The proof of Lemma \ref{lemma:ini_sym} essentially follows Theorem 3.9  in \cite{Sun2016}, we thus omit the detailed proof here. The upper bound in \eqref{ineq:initial_error} contains two terms: $\frac{C_4}{\eta^\ast_{\min}}\|\cE\|_{s+d}$ and $\sqrt{K}\Gamma^2$, which are due to the empirical moment approximation and the incoherence among different $\bbeta_k$, respectively. %Combining with Lemma \ref{lemma:ini_sym}, it's not hard to see that with the sample size $n$ increasing, this upper bound is dominated first by approximation error and then by the incoherence error. %In the case of $K\geq 2$ which typically the incoherence parameter is greater than zero, the sparse tensor decomposition could not offer a consistency estimation. In the case of rank-one tensor recovery, the incoherence parameter is equal to zero. However, the convergence rate \eqref{ineq:perturbation_error} is far from the minimax optimal rate we derive in Theorem \eqref{th:lower_bound}.

Although the sparse tensor decomposition is not optimal in statistical rate, it does offer a reasonable initial estimation provided enough samples. Equipped with \eqref{ineq:perturbation_error} and Condition \ref{con:parameter}, the right side of \eqref{ineq:initial_error} reduces to 
\begin{eqnarray*}
	&&\frac{C_4}{\eta_{\min}^*}\|\cE\|_{s+d} + \sqrt{K}\Gamma^2 \\
	&\leq& 2 C_1C_4KR\Big(\sqrt{\frac{s^3\log^3(p/s)}{n^2}}+\sqrt{\frac{s\log(p/s)}{n}}\Big)(\log n)^4+\sqrt{K}\Gamma^2,
\end{eqnarray*} 
with probability at least $1-5/n$. Denote $C_0=4\cdot 2160\cdot C_1C_4$. Using Conditions \ref{con:incoherence_sym} and \ref{con:sample}, we reach the conclusion that
$$\max\left\{\|\bbeta_k^{(0)} - \bbeta_k^*\|_2, |\eta_k^{(0)} - \eta_k^*|\right\}\leq  K^{-1}R^{-2}/2160,$$
with probability at least $1-5/n$. \hfill $\blacksquare$\\	

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proof of Theorem \ref{thm:symmetric_main}: Gradient Update}
\label{subsec:gradient-update-proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%The proof of Theorem \ref{thm:symmetric_main} evaluates the effect of thresholded gradient update. The major difference of theoretical guarantee between symmetric tensor recovery and non-symmetric tensor recovery lies on the source of non-convexity.
%For non-symmetric tensor recovery problem, the non-convexity comes from the tri-convexity. This allows us to use similar technique in analyzing gradient descent algorithm. However, in symmetric tensor recovery problem, the non-convexity comes from the cube structure insider least square. To overcome this obstacle, we adopt the analysis in \cite{CLM16} with novel concentration result. 

We first introduce the following lemma to illustrate the improvement of one step thresholded gradient update under suitable conditions. %This lemma quantifies the estimation error of all factors after one iteration of update. 
The error bound includes two parts: the optimization error that describes one step effect for gradient update, and the statistical error that reflects the random noise effect. %The reason we consider to bound a weighted estimator $\sqrt[3]{\eta_k}\bbeta_k^{(t+1)}$ is due to the un-normalization in the algorithm. 
The proof of Lemma \ref{lemma:onestep_update_sym} is given in Section \ref{proof:onestep_update_sym} in the supplementary materials. For notation simplicity, we drop the superscript of $\eta_k^{(0)}$ in the following proof.

\begin{Lemma}
	\label{lemma:onestep_update_sym}
	Let $t\geq 0$ be an integer. Suppose Conditions \ref{con:ident}-\ref{con:sample} hold and $\{\bbeta_k^{(t)}, \eta_k\}$ satisfies the following upper bound
	\begin{equation}\label{con:initial_input}
	\sum_{k=1}^K\Big\|\sqrt[3]{\eta_k}\bbeta_k^{(t)}-\sqrt[3]{\eta_k^*}\bbeta_k^*\Big\|_2^2\leq 4K\eta_{\max}^{*\tfrac{2}{3}}\varepsilon_0^2, \ \max_{k\in[K]}\Big|\eta_k-\eta_k^*\Big|\leq \varepsilon_0,
	\end{equation}
	with probability at least $1-\cO(K/n)$, where $\varepsilon_0= K^{-1}R^{-\tfrac{4}{3}}/2160$. As long as the step size $\mu$ satisfies
	\begin{equation}\label{eqn:mu_0}
	0<\mu\leq \mu_0= \frac{32 R^{-20/3}}{3K[220+270K]^2},%n\geq (18(C_1e)^{-1/3}K^{1/2}R^{8/3}(\log n)^3)^2.
	\end{equation}
	then $\{\bbeta_k^{(t+1)}\}$ can be upper bounded as
	\begin{equation*}
	\begin{split}
	&\sum_{k=1}^K\Big\|\sqrt[3]{\eta_k}\bbeta_k^{(t+1)}-\sqrt[3]{\eta_k^*}\bbeta_k^*\Big\|_2^2\\
	&\leq \underbrace{\Big(1-32\mu K^{-2}R^{-\tfrac{8}{3}}\Big)\sum_{k=1}^K\Big\|\sqrt[3]{\eta_k}\bbeta_k^{(t)}-\sqrt[3]{\eta_k^*}\bbeta_k^*\Big\|_2^2}_{\text{optimization error}}+\underbrace{2C_0\mu^2K^{-2}R^{-\tfrac{8}{3}}\eta_{\min}^{*-\tfrac{4}{3}}\frac{\sigma^2s\log p}{n}}_{\text{statistical error}},
	\end{split}
	\end{equation*}
	with probability at least $1-\cO(Ks/n)$. 
\end{Lemma}


In order to apply Lemma \ref{lemma:onestep_update_sym}, we prove that the required condition \eqref{con:initial_input} holds at every iteration step $t$ by induction. When $t=0$, by \eqref{ineq:initial} and Condition \ref{con:parameter},
\begin{eqnarray*}
	\Big\|\bbeta_k^{(0)}-\bbeta_k^*\Big\|_2\leq \varepsilon_0, \ \Big|\eta_k-\eta_k^*\Big|\leq \varepsilon_0, \ \text{for} \ k\in[K],
\end{eqnarray*}
holds with probability at least $1-\cO(1/n)$. Since the initial estimator output by first stage is normalized, i.e., $\|\bbeta_k^{(0)}\|_2 = \|\bbeta_k^\ast\|_2 = 1$, by triangle inequality we have 
\begin{eqnarray*}
	\Big\|\sqrt[3]{\eta_k}\bbeta_k^{(0)} -\sqrt[3]{\eta_k^*}\bbeta_k^{*} \Big\|_2&\leq& \Big\|\sqrt[3]{\eta_k}\bbeta_k^{(0)} - \sqrt[3]{\eta_k^*}\bbeta_k^{(0)} + \sqrt[3]{\eta_k^*}\bbeta_k^{(0)} -\sqrt[3]{\eta_k^*}\bbeta_k^{*} \Big\|_2\\
	&\leq& |\sqrt[3]{\eta_k}-\sqrt[3]{\eta_k^*}|+\sqrt[3]{\eta_k^*}\Big\|\bbeta_k^{(0)} -\bbeta_k^{*} \Big\|_2.
\end{eqnarray*}
Note that $$\Big|\sqrt[3]{\eta_k}-\sqrt[3]{\eta_k^*}\Big|\leq \frac{\varepsilon_0}{(\sqrt[3]{\eta_k})^2+\sqrt[3]{\eta_k\eta_k^*}+(\sqrt[3]{\eta_k^*})^2}\leq \varepsilon_0\sqrt[3]{\eta_k^*}.$$
This implies
\begin{eqnarray*}
	\Big\|\sqrt[3]{\eta_k}\bbeta_k^{(0)} - \sqrt[3]{\eta_k^*}\bbeta_k^*\Big\|_2\leq2\sqrt[3]{\eta_k^*}\varepsilon_0,
\end{eqnarray*}
with probability at least $1-\cO(1/n)$.
Taking the summation over $k\in[K]$, we have
\begin{equation*}
\sum_{k=1}^K\Big\|\sqrt[3]{\eta_k}\bbeta_k^{(0)} - \sqrt[3]{\eta_k^*}\bbeta_k^*\Big\|_2^2 \leq \sum_{k=1}^K4\eta_k^{*\tfrac{2}{3}}\varepsilon_0^2\leq 4 K\eta_{\max}^{*\tfrac{2}{3}}\varepsilon_0^2,
\end{equation*}
with probability at least $1-\cO(K/n)$, which means \eqref{con:initial_input} holds for $t= 0$.

Suppose \eqref{con:initial_input} holds at the iteration step $t-1$, which implies 
\begin{equation*}
\begin{split}
&\sum_{k=1}^{K}\Big\|\sqrt[3]{\eta_k}\bbeta_k^{(t)} -\sqrt[3]{\eta_k^*}\bbeta_k^{*} \Big\|_2^2\\
\leq& \Big(1-32\mu K^{-2}R^{-\tfrac{8}{3}}\Big)\sum_{k=1}^K\Big\|\sqrt[3]{\eta_k}\bbeta_k^{(t-1)} -\sqrt[3]{\eta_k^*}\bbeta_k^{*} \Big\|_2^2+\mu2C_0K^{-2}R^{-\tfrac{8}{3}}\eta_{\min}^{*\tfrac{4}{3}}\frac{\sigma^2s\log p}{n}\\
\leq& 4K\eta_{\max}^{*\tfrac{2}{3}}\varepsilon_0^2-\mu\Big(128KR^{-\tfrac{8}{3}}\eta_{\max}^{*\tfrac{2}{3}}\varepsilon_0^2-2C_0K^{-2}R^{-\tfrac{8}{3}}\eta_{\min}^{*\tfrac{4}{3}}\frac{\sigma^2s\log p}{n}\Big).
\end{split}
\end{equation*}
Since Condition \ref{con:sample} automatically implies
\begin{equation*}
\frac{n}{s\log p}\geq \frac{C_0\sigma^2R^{-\tfrac{2}{3}}\eta_{\min}^{*\tfrac{2}{3}}K}{64\varepsilon_0^2},
\end{equation*}
for a sufficiently large $C_0$, we can obtain
\begin{eqnarray*}
	\sum_{k=1}^{K}\Big\|\sqrt[3]{\eta_k}\bbeta_k^{(t)} -\sqrt[3]{\eta_k^*}\bbeta_k^{*} \Big\|_2^2\leq 4K\eta_{\max}^{*\tfrac{2}{3}}\varepsilon_0^2.
\end{eqnarray*}
By induction, \eqref{con:initial_input} holds at each iteration step.

Now we are able to use Lemma \ref{lemma:onestep_update_sym} recursively to complete the proof. Repeatedly using Lemma \ref{lemma:onestep_update_sym}, we have for $t=1,2,\ldots,$
\begin{equation*}
\begin{split}
&\sum_{k=1}^{K}\Big\|\sqrt[3]{\eta_k}\bbeta_k^{(t+1)} -\sqrt[3]{\eta_k^*}\bbeta_k^{*} \Big\|_2^2\\
&\leq \Big(1-32\mu K^{-2}R^{-\tfrac{8}{3}}\Big)^t\sum_{k=1}^K\Big\|\sqrt[3]{\eta_k}\bbeta_k^{(0)} -\sqrt[3]{\eta_k^*}\bbeta_k^{*} \Big\|_2^2+\frac{C_0\eta_{\min}^{*-\tfrac{4}{3}}}{16}\frac{\sigma^2s\log p}{n},
\end{split}
\end{equation*}
with probability at least $1-\cO(tKs/n)$. This concludes the first part of Theorem \ref{thm:symmetric_main}. 

%The above upper bound provides the compromise between optimization and statistical error. With the number of iterations increasing, the optimization error decreases while the statistical error remains the same. This illustrates that at the beginning of the algorithm, the optimization error will dominate the whole error bound. When the number of iterations is large enough, the statistical error will dominate the error bound finally. Quantitatively, 

When the total number of iterations is no smaller than 
\begin{eqnarray*}
	T^* = \frac{\log(C_3\eta_{\min}^{*-4/3}\sigma^2s\log p)-\log(64\eta_{\max}^{*2/3}K\varepsilon_0 n)}{\log(1-32\mu K^{-2}R^{-8/3})},
\end{eqnarray*}
the statistical error will dominate the whole error bound in the sense that
\begin{eqnarray}
\label{eqn:factor_error_sym}
\sum_{k=1}^{K}\Big\|\sqrt[3]{\eta_k}\bbeta_k^{(T^*)} -\sqrt[3]{\eta_k^*}\bbeta_k^{*} \Big\|_2^2\leq \frac{C_3\eta_{\min}^{*-\tfrac{4}{3}}}{8}\frac{\sigma^2s\log p}{n},
\end{eqnarray}
with probability at least $1-\cO(T^*Ks/n)$. 

%The next lemma shows that the transformation of Frobenius norm between two tensors to the square norm between their corresponding factorization under CP low-rank assumption. The proof is postponed to Section \ref{proof:error_transfer}.
The next lemma shows that the Frobenius norm distance between two tensors can be bounded by the distances between each factors in their CP decomposition. The proof of this lemma is provided in Section \ref{proof:error_transfer}.
\begin{Lemma}\label{lemma:error_transfer}%[Error Transfer]
	Suppose $\mT$ and $\mT^*$ have CP-decomposition $\mT = \sum_{k=1}^K\eta_k\bbeta_k\circ \bbeta_k\circ \bbeta_k$ and $\mT^* = \sum_{k=1}^K\eta_k^*\bbeta_k^*\circ \bbeta_k^*\circ \bbeta_k^*$. If $|\eta_k-\eta_k^*|\leq c$, then %the distance between $\mT$ and $\mT^*$ under tensor Frobenius norm can be transferred as following,
	\begin{equation*}
	\Big\|\mT-\mT^*\Big\|_F^2\leq 9(1+c)\Big(\sum_{k=1}^K\Big\|\sqrt[3]{\eta_k}\bbeta_k - \sqrt[3]{\eta_k^*}\bbeta_k^*\Big\|_2^2\Big)\Big(\sum_{k=1}^K(\sqrt[3]{\eta_k^*})^4\Big)
	\end{equation*}
\end{Lemma}


Denote $\hat{\mT} = \sum_{k=1}^K \eta_k\bbeta_k^{(T^*)}\circ \bbeta_k^{(T^*)}\circ \bbeta_k^{(T^*)} $. Combing  \eqref{eqn:factor_error_sym} and Lemma \ref{lemma:error_transfer},
we have
\begin{eqnarray*}
	\Big\|\hat{\mT}-\mT^*\Big\|_F^2&\leq& 9(1+\varepsilon_0)\frac{C_3\eta_{\min}^{*-\tfrac{4}{3}}}{8}\frac{\sigma^2s\log p}{n}K\eta_{\max}^{*\tfrac{4}{3}},\\
	&=&\frac{9C_3R}{4}\frac{\sigma^2Ks\log p}{n},
\end{eqnarray*}
with probability at least $1-\cO(TKs/n)$.  By setting $C_1 = 9C_2/4$, we complete the proof of Theorem \ref{thm:symmetric_main}. \hfill $\blacksquare$\\



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proofs of Theorems \ref{th:lower_bound} and \ref{th:lower_bound_asymmetric}: Minimax Lower Bounds} \label{proof:thm_minimax}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We first consider the proof for Theorem \ref{th:lower_bound_asymmetric} on non-symmetric tensor estimation. Without loss of generality we assume $p = \max\{p_1, p_2, p_3\} $. We uniformly randomly generate $\{\Omega^{(k, m)}\}_{\substack{m=1,\ldots, M\\k=1,\ldots, K}}$ as $MK$ subsets of $\{1,\ldots, p\}$ with cardinality of $s$. Here $M>0$ is a large integer to be specified later. Then we construct $\{\bbeta^{(k, m)}\}_{\substack{m=1,\ldots, M\\k=1,\ldots, K}}\subseteq \mathbb{R}^{p}$ as
\begin{equation*}
\bbeta^{(k, m)}_j = \left\{\begin{array}{ll}
\sqrt{\lambda}, & \text{ if } j\in \Omega^{(k, m)};\\
0, & \text{ if } j\notin \Omega^{(k, m)}.\\	
\end{array}\right.
\end{equation*}
$\lambda>0$ will also be specified a little while later. Clearly, $\|\bbeta^{(k, m_1)} - \bbeta^{(k, m_2)}\|_2^2 \leq 2s\lambda$ for any $1\leq k \leq K$, $1\leq m_1, m_2\leq M$. Additionally, $|\Omega^{(k, m_1)}\cap \Omega^{(k, m_2)}|$ satisfies the hyper-geometric distribution: 
$\mathbb P\left(\left|\Omega^{(k, m_1)}\cap \Omega^{(k, m_2)}\right| = t\right) = \frac{\binom{s}{t}\binom{p-s}{s-t}}{\binom{p}{s}}$. 

Let $w^{(k, m_1, m_2)} = \left|\Omega^{(k, m_1)}\cap \Omega^{(k, m_2)}\right|$, then for any $s/2\leq t \leq s$, 
\begin{equation*}
\begin{split}
& \mathbb{P}\left(w^{(k, m_1, m_2)} = t\right) = \frac{\frac{s\cdots (s-t+1)}{t!} \cdot \frac{(p-s)\cdots (p-2s+t+1)}{(s-t)!}}{\frac{p\cdots (p-s+1)}{s!}} \leq \binom{s}{t}\cdot \left(\frac{s}{p-s+1}\right)^t\\
\leq & 2^s\left(\frac{s}{p-s+1}\right)^t \leq \left(\frac{4s}{p-s+1}\right)^t.
\end{split}
\end{equation*}
Thus, if $\eta >0$, the moment generating function of $w^{(k, m_1, m_2)} - \frac{s}{2}$ satisfies
\begin{equation*}
\begin{split}
& \mathbb{E}\exp\left(\eta \left(w^{(k, m_1, m_2)} - \frac{s}{2}\right)\right) \\
\leq & \exp(0)\cdot \mathbb P\left(w^{(k, m_1, m_2)}\leq \frac{s}{2}\right) + \sum_{t=\lfloor s/2\rfloor +1}^s \exp\left(\eta \left(t-\frac{s}{2}\right)\right)\cdot \mathbb P\left(w^{(k, m_1, m_2)} = t\right)\\
\leq & 1 + \sum_{t=\lfloor s/2\rfloor +1}^{s} \left(4s/(p-s+1)\right)^t\exp\left(\eta (t-s/2)\right)\\
\leq & 1 + \left(4s/(p-s+1) \right)^{s/2} \frac{1}{1 - 4s/(p-s+1)\cdot e^\eta}.
\end{split}
\end{equation*}
By setting $\eta = \log((p-s+1)/(8s))$, we have
\begin{equation*}
\begin{split}
& \mathbb P\left(\sum_{k=1}^K w^{(k, m_1, m_2)} \geq \frac{3sK}{4}\right) = \mathbb P\left(\sum_{k=1}^K w^{(k, m_1, m_2)} - \frac{sK}{2} \geq \frac{sK}{4}\right)\\
\leq & \frac{ \mathbb{E}\exp\left(\eta(\sum_{k=1}^K w^{(k, m_1, m_2)}-\frac{sK}{2})\right)}{\exp\left(\eta\cdot \frac{sK}{4}\right)} = \frac{\prod_{k=1}^K \mathbb{E}\exp\left(\eta(w^{(k, m_1, m_2)}-\frac{s}{2})\right)}{\exp(\eta\cdot \frac{sK}{4})}\\
\leq & \left(1 + (4s/(p-s+1))^{s/2}\cdot 2 \right)^K\exp\left(-\frac{sK}{4}\log\left(\frac{p-s+1}{8s}\right)\right)\\
\leq & \exp\left(-c_0sK\log(p/s)\right)
\end{split}
\end{equation*}
for some small uniform constant $c_0>0$.
%Additionally,
%		\begin{equation}
%		\begin{split}
%		& \mP\left(\|\bbeta^{(m_1)} - \bbeta^{(m_2)}\|_2^2\leq s\lambda\right) = \mP\left(\left|\Omega^{(m_1)} \cap \Omega^{(m_2)}\right| \geq \frac{s}{2}\right) = \sum_{t = \lceil\frac{s}{2}\rceil}^s \mP\left(|\Omega_i \cap \Omega_j| = t\right)\\
%		= & \sum_{t = \lceil\frac{s}{2}\rceil}^s \frac{\binom{s}{t} \binom{p-s}{s-t}}{\binom{p}{s}} = \sum_{t = \lceil\frac{s}{2}\rceil}^s \frac{\frac{s\cdots (s-t+1)}{t!}\cdot \frac{(p-s)\cdots (p-2s+t+1)}{(s-t)!}}{\frac{p\cdots (p-s+1)}{s!}} \leq \sum_{t = \lceil\frac{s}{2}\rceil}^s \binom{s}{t} \left(\frac{s}{p-s+1}\right)^t\\
%		\leq & \sum_{t = \lceil\frac{s}{2}\rceil}^s \binom{s}{t} \left(\frac{s}{p-s+1}\right)^{s/2} \leq \left(\frac{4s}{p-s+1}\right)^{s/2}
%		\end{split}
%		\end{equation}

Next, we choose $M = \lfloor\exp(c_0/2\cdot sK\log(p/s))\rfloor$. Note that 
\begin{equation*}
\begin{split}
& \|\bbeta^{(k, m_1)} - \bbeta^{(k, m_2)}\|_2^2 = \lambda\cdot \left(\left|\Omega^{(k, m_1)}\setminus \Omega^{(k, m_2)}\right| + \left|\Omega^{(k, m_2)}\setminus \Omega^{(k, m_1)}\right|\right)\\
= & \lambda \left(\left|\Omega^{(k, m_1)}\right| + \left|\Omega^{(k, m_2)}\right| - 2\left|\Omega^{(k, m_1)}\cap \Omega^{(k, m_2)}\right|\right) \\
=& 2\lambda\left(s - \left|\Omega^{(k, m_1)}\cap \Omega^{(k, m_2)}\right|\right),
\end{split}
\end{equation*}
then we further have
\begin{equation*}
\begin{split}
& \mP\left(\sum_{k=1}^K\|\bbeta^{(k, m_1)} - \bbeta^{(k, m_2)}\|_2^2 \geq \frac{sK\lambda}{2}, \forall 1\leq m_1 < m_2 \leq M\right)\\
= & \mP\left(\sum_{k=1}^Kw^{(k, m_1, m_2)} \leq \frac{3K}{4}, \forall 1\leq m_1, < m_2 \leq M\right)\\
\geq &  1 - \frac{M(M-1)}{2}\exp\left(-c_0sK\log(p/s)\right)\\
> & 1 - M^2 \exp\left(-c_0sK\log(p/s)\right) \geq 0,
\end{split}
\end{equation*}
which means there are positive probability that $\left\{\bbeta^{(k, m)}\right\}_{\substack{k=1,\ldots, K\\m=1,\ldots, M}}$ satisfy
\begin{equation}\label{ineq:beta^m_1-beta^m_2}
\begin{split}
&\frac{sK\lambda}{2} \leq \min_{1\leq m_1< m_2\leq M} \sum_{k=1}^K\left\|\bbeta^{(k, m_1)}-\bbeta^{(k, m_2)}\right\|_2^2 \\
&\leq \max_{1\leq m_1< m_2\leq M} \sum_{k=1}^K\left\|\bbeta^{(k, m_1)}-\bbeta^{(k, m_2)}\right\|_2^2 \leq 2sK\lambda.
\end{split}
\end{equation}
For the rest of the proof, we fix $\left\{\bbeta^{(k, m)}\right\}_{\substack{k=1,\ldots, K\\m=1,\ldots, M}}$ to be the set of vectors satisfying \eqref{ineq:beta^m_1-beta^m_2}.

Next, recall the canonical basis $\be_{k} = (0,\ldots, \overbrace{1}^{k\text{-th}}, 0, \cdots, 0)\in \mathbb{R}^{p}$. Define
$$\mT^{(m)} = \sum_{k=1}^{K} \bbeta^{(k, m)}\circ \be_{k} \circ \be_{k},\quad 1\leq m \leq M.$$ 
For each tensor $\mT^{(m)}$ and $n$ i.i.d. Gaussian sketches $\bu_i, \bv_i, \bw_i\in \mathbb{R}^{p}$, we denote the response
$$\by^{(m)} = \left\{y_i^{(m)}\right\}_{i=1}^n, \quad y^{(m)}_i = \langle \bu_i\circ \bv_i\circ \bw_i, \mT^{(m)}\rangle + \epsilon_i, $$
where $\epsilon_i \overset{iid}{\sim} N(0, \sigma^2), \quad i=1,\ldots, n.$ Clearly, $\left(\by^{(m)}, \bu, \bv, \bw\right)$ follows a joint distribution, which may vary based on different values of $m$. 

In this step, we analyze the Kullback-Leibler divergence between different distribution pairs:
\begin{equation*}
\begin{split}
& D_{KL}\left((\by^{(m_1)}, \bu, \bv, \bw), (\by^{(m_2)}, \bu, \bv, \bw)\right) := \mathbb{E}_{(\by^{(m_1)}, \bu, \bv, \bw)} \frac{p(\by^{(m_1)}, \bu, \bv, \bw)}{p(\by^{(m_2)}, \bu, \bv, \bw)}.\\
\end{split}
\end{equation*}
Note that conditioning on fixed values of $\bu, \bv, \bw$, 
$$y^{(m)}_i\sim N\left(\sum_{k=1}^K(\bbeta^{(k, m)\top}\bu_i )\cdot (\be^{(k)\top} \bv_i) \cdot (\be^{(k)\top}\bw_i), \sigma^2\right).$$ By the KL-divergence formula for Gaussian distribution,
\begin{equation*}
\begin{split}
& \mathbb{E}_{(\by^{(m_1)}, \bu, \bv, \bw)} \left(\frac{p(\by^{(m_1)}, \bu, \bv, \bw)}{p(\by^{(m_2)}, \bu, \bv, \bw)}\Big| \bu, \bv, \bw\right) \\
= & \frac{1}{2} \sum_{i=1}^n\left(\sum_{k=1}^K \left(\left(\bbeta^{(k,m_1)} - \bbeta^{(k,m_2)}\right)^\top \bu_i\right)\left(\be^{(k)\top} \bv_i\right)\left(\be^{(k)\top} \bw_i\right)\right)^2\sigma^{-2}. 
\end{split}
\end{equation*}
Therefore, for any $m_1 \neq m_2$,
\begin{equation*}
\begin{split}
& D_{KL}\left((\by^{(m_1)}, \bu, \bv, \bw), (\by^{(m_2)}, \bu, \bv, \bw)\right)\\
= & \mathbb{E}_{\bu, \bv, \bw} \frac{1}{2} \sum_{i=1}^n\left(\sum_{k=1}^K (\bbeta^{(k,m_1)} - \bbeta^{(k,m_2)})^\top \bu_i)(\be^{(k)\top} \bv_i)(\be^{(k)\top} \bw_i)\right)^2\sigma^{-2}\\
= & \frac{\sigma^{-2}}{2}\sum_{i=1}^n \sum_{k=1}^K \mathbb{E}_{\bu}((\bbeta^{(k,m_1)} - \bbeta^{(k,m_2)})^\top \bu_i)^2\mathbb{E}_{\bv}(\be^{(k)\top} \bv_i)^2\mathbb{E}_{\bw}(\be^{(k)\top} \bw_i)^2\\
= & \frac{n\sigma^{-2}}{2}\sum_{k=1}^K\|\bbeta^{(k, m_1)} - \bbeta^{(k, m_2)}\|_2^2 \leq \sigma^{-2}nKs\lambda. \\
\end{split}
\end{equation*}

Meanwhile, for any $1\leq m_1 < m_2 \leq M$,
\begin{equation*}
\begin{split}
\|\mT^{(m_1)} - \mT^{(m_2)}\|_F = & \left\|\sum_{k=1}^K(\bbeta^{(k, m_1)}-\bbeta^{(k, m_2)})\circ \be^{(k)} \circ \be^{(k)}\right\|_F\\
= & \sqrt{\sum_{k=1}^K\left\|\bbeta^{(k, m_1)}-\bbeta^{(k, m_2)}\right\|_2^2} \overset{\eqref{ineq:beta^m_1-beta^m_2}}{\geq} \sqrt{\frac{sK\lambda}{2}}.
\end{split}
\end{equation*}
By generalized Fano's Lemma (see, e.g., \cite{yu1997assouad}),
\begin{equation*}
\inf_{\hat{\mT}} \sup_{\mT \in \mathcal{F}} \mathbb{E}\|\hat{\mT} - \mT\|_F \geq \sqrt{\frac{sK\lambda}{2}}\left(1 - \frac{\sigma^{-2}nKs\lambda + \log 2}{\log M}\right).
\end{equation*}
Finally we set $\lambda = \frac{c\sigma^2}{n}\log(p/s)$ for some small constant $c>0$, then
\begin{equation*}
\inf_{\hat{\mT}} \sup_{\mT \in \mathcal{F}} \mathbb{E}\|\hat{\mT} - \mT\|_F^2 \geq \left(\inf_{\hat{\mT}} \sup_{\mT \in \mathcal{F}} \mathbb{E}\|\hat{\mT} - \mT\|_F\right)^2 \geq \frac{c\sigma^2 sK\log(p/s)}{n}.
\end{equation*}
which has finished the proof of Theorem \ref{th:lower_bound_asymmetric}.

For the proof for Theorem \ref{th:lower_bound}, without loss of generality we assume $K$ is a multiple of 3. We first partition $\{1,\ldots, p\}$ into two subintervals: $I_1  = \{1,\ldots, p-K/3\}, I_2 = \{p-K/3+1,\ldots, p\}$, randomly generate $\{\Omega^{(k, m)}\}_{\substack{m=1,\ldots, M\\k=1,\ldots, K/3}}$ as $(MK/3)$ subsets of $\{1,\ldots, p-K/3\}$, and construct $\{\bbeta^{(k,m)}\}_{\substack{m=1,\ldots, M\\k=1,\ldots, K}}\subseteq \mathbb{R}^{p-K/3}$ as
\begin{equation*}
\bbeta^{(k, m)} = \left\{\begin{array}{ll}
\sqrt{\lambda}, & \text{if } j \notin \Omega^{(k, m)};\\
0, & \text{if } j \notin \Omega^{(k, m)}.
\end{array}\right.
\end{equation*}
With $M = \exp(csK\log(p/s))$ and similar techniques as previous proof, one can show there exists positive possibility that
\begin{equation*}
\begin{split}
&\frac{sK\lambda}{6} \leq \min_{1\leq m_1 < m_2\leq M}\sum_{k=1}^{K/3}\|\bbeta^{(k, m_1)} - \bbeta^{(k, m_2)}\|_2^2 \\
&\leq \max_{1\leq m_1 < m_2\leq M}\sum_{k=1}^{K/3}\|\bbeta^{(k, m_1)} - \bbeta^{(k, m_2)}\|_2^2 \leq \frac{2sK}{3}\lambda.
\end{split}
\end{equation*}

We then construct the following candidate symmetric tensors by blockwise design,
\begin{equation*}
\cT^{(m)}\in \mathbb{R}^{p\times p\times p}, \quad \left\{\begin{array}{ll}
\cT^{(m)}_{[I_1, I_2, I_2]} = \sum_{k=1}^{K/3}\bbeta^{(k, m)}\circ \be^{(k)}\circ \be^{(k)},\\ 
\cT^{(m)}_{[I_2, I_1, I_2]} = \sum_{k=1}^{K/3}\be^{(k)}\circ \bbeta^{(k, m)}\circ \be^{(k)},\\
\cT^{(m)}_{[I_2, I_2, I_1]} = \sum_{k=1}^{K/3}\be^{(k)}\circ \be^{(k)} \circ \bbeta^{(k, m)},\\
\cT^{(m)}_{[I_1, I_1, I_1]}, \cT^{(m)}_{[I_1, I_1, I_2]}, \cT^{(m)}_{[I_1, I_2, I_1]}, \cT^{(m)}_{[I_2, I_1, I_1]}, \cT^{(m)}_{[I_2, I_2, I_2]} \text{ are all zeros}.
\end{array}\right.
\end{equation*}
Then we can see for any $\bu\in \mathbb{R}^p$,
\begin{equation*}
\langle \cT^{(m)}, \bu\circ\bu\circ\bu \rangle = 3\sum_{k=1}^{K/3}\left(\bbeta^{(k, m)\top}\bu_{I_1}\right)\cdot\left(\be^{(k)\top}\bu_{I_2}\right)^2.
\end{equation*}
The rest of the proof essentially follows from the proof of Theorem \ref{th:lower_bound_asymmetric}.
\hfill $\blacksquare$\\

\subsection{Proof of Theorem \ref{thm:steins_higher}: High-order Stein's Lemma}\label{proof:stein_higher}
The proof of this theorem follows from the one of Theorem 6 in \cite{janzamin2014score}. For the sake of completeness, we restate the detail here. Applying the recursion representation of score function \eqref{eqn:recursive_form}, we have
\begin{eqnarray*}
\mathbb E\Big[G(\bx)\cS_3(\bx)\Big] &=& \mathbb E\Big[G(\bx)\Big(-\cS_2(\bx)\circ \nabla_{\bx}\log p(\bx)-\nabla_{\bx} \cS_2(\bx)\Big)\Big]\\
&=& -\mathbb E\Big[G(\bx)\cS_2(\bx)\circ \nabla_{\bx}\log p(\bx)\Big]-\mathbb E\Big[G(\bx)\nabla_{\bx} \cS_2(\bx)\Big)\Big].
\end{eqnarray*}
Then, we apply the first-order Stein's lemma (see Lemma  \ref{lemma:stein_lemma}) on function $G(\bx)\cS_2(\bx)$ and obtain
\begin{eqnarray*}
    \mathbb E\Big[G(\bx)\cS_3(\bx)\Big] &=& \mathbb E\Big[\nabla_{\bx}\Big(G(\bx)\cS_2(\bx)\Big)\Big]-\mathbb E\Big[G(\bx)\nabla_{\bx} \cS_2(\bx)\Big)\Big]\\
    &=& \mathbb E\Big[\nabla_{\bx}G(\bx)\cS_2(\bx)+\nabla_{\bx}\cS_2(\bx)G(\bx)\Big]-\mathbb E\Big[G(\bx)\nabla_{\bx} \cS_2(\bx)\Big)\Big]\\
    &=&\mathbb E\Big[\nabla_{\bx}G(\bx)\cS_2(\bx)\Big].
\end{eqnarray*}
Repeating the above argument two more times, we reach the conclusion. \hfill $\blacksquare$\\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Proofs of Several Lemmas}\label{sec:proof_lemmas} \label{supp_sec:proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proofs of Lemmas \ref{lemma:moment_asy}, \ref{lemma:moment_symmetric}, and \ref{lemma:moment_interaction}: Moment Calculation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this subsection, we present the detail proofs of moment calculation, including non-symmetric case, symmetric case, and interaction model. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Proof of Lemma \ref{lemma:moment_asy}}\label{proof_moment_asy}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 By the definition of $\{y_i\}$ in \eqref{eq:model_asymmetric} \& \eqref{eq:low_rank_nonsym}, we have
\begin{equation}
\label{equation:non-symmetric}
\begin{split}
&\mathbb E\Big(\frac{1}{n}\sum_{i=1}^n y_i\bu_i\circ\bv_i\circ\bw_i\Big) = \mathbb E\Big(\frac{1}{n}\sum_{i=1}^n\epsilon_i\bu_i\circ \bv_i\circ \bw_i\Big)\\
&+\mathbb E\Big(\frac{1}{n}\sum_{i=1}^n \sum_{k=1}^K\eta_k^*(\bbeta_{1k}^{*\top}\bu_i)(\bbeta_{2k}^{*\top}\bv_i)(\bbeta_{3k}^{*\top}\bw_i)\bu_i\circ\bv_i\circ\bw_i\Big). 
\end{split}
\end{equation}
First, we observe $\mathbb E(\epsilon_i\bu_i\circ \bv_i\circ \bw_i )=0$ due to the independence between $\epsilon_i$ and $\{\bu_i, \bv_i, \bw_i\}$. Then, we consider a single component from a single observation 
$$M=\mathbb E((\bbeta_{1k}^{*\top}\bu_i)(\bbeta_{2k}^{*\top}\bv_i)(\bbeta_{3k}^{*\top}\bw_i)\bu_i\circ\bv_i\circ\bw_i), \ i\in[n], k\in[K].
$$ For notation simplicity, we drop the subscript $i$ for $i$-th observation and $k$ for $k$-th component such that
\begin{eqnarray}
\label{equation:M_nonsymmetric}
M = \mathbb E \Big((\bbeta_1^{*\top}\bu)(\bbeta_2^{*\top}\bv)(\bbeta_3^{*\top}\bw)\bu\circ\bv\circ\bw\Big)\in\mathbb R^{p_1\times p_2\times p_3}.
\end{eqnarray}
Each entry of $M$ can be calculated as follows
\begin{eqnarray*}
	M_{ijk} &=& \mathbb E \Big((\bbeta_1^{*\top}\bu)(\bbeta_2^{*\top}\bv)(\bbeta_3^{*\top}\bw)u_iv_jw_k\Big)\\
	&=&\mathbb E\Big((\beta_{1i}^*u_i+\sum_{m\neq i}\beta_{1m}^*u_m)u_i\Big)\mathbb E\Big((\beta_{2j}^*u_i+\sum_{m\neq j}\beta_{2m}^*v_m)v_j\Big)\\
	&&\times\mathbb E\Big((\beta_{3k}^*w_k+\sum_{m\neq k}\beta_{3m}^*w_m)w_k\Big)\\
	&=& \beta_{1i}^*\beta_{2j}^*\beta_{3k}^*,
\end{eqnarray*}
which implies $M = \bbeta_1\circ\bbeta_2\circ\bbeta_3$. Combining with $n$ observations and $K$ components, we can obtain
\begin{eqnarray*}
	\mathbb E\big(\cT\big) = \frac{1}{n}\sum_{i=1}^n \sum_{k=1}^K\eta_k^* \bbeta_{1k}\circ\bbeta_{2k}\circ\bbeta_{3k}.
\end{eqnarray*}
This finished our proof. \hfill $\blacksquare$\\


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Proof of Lemma \ref{lemma:moment_symmetric}} \label{proof_moment_sym}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


In this subsection, we provide an alternative and more direct proof for Lemma \ref{lemma:moment_symmetric}. We consider a similar single component of (\ref{equation:M_nonsymmetric}) but with a symmetric structure, namely, $M_s = \mathbb E \Big((\bbeta^{*\top}\bx)^3\bx\circ\bx\circ\bx\Big)$. Based on the symmetry of both underlying tensor and sketchings, we will verify the following three cases:
\begin{itemize}
	\item When $i=j=k$, then
	\begin{eqnarray*}
		M_{s_{iii}} &=& \mathbb E\Big(\beta_{i}^*x_i+\sum_{m\neq i}\beta_m^*x_m\Big)^3x_i^3\\
		&=&\mathbb E\Big(\beta_{i}^{*3}x_i^3+3\beta_{i}^{*2}x_i^2\big(\sum_{m\neq i}\beta_{m}^*x_m\big)\\
		&&+3\beta_{i}^*x_i\big(\sum_{m\neq i}\beta_m^*x_m\big)^2+\big(\sum_{m\neq i}\beta_m^* x_m\big)^3\Big)x_i^3\\
		&=& 15 \beta_i^{*3}+9\beta_i^*\sum_{m\neq i}\beta_m^{*2} = 9\beta_i^*+6\beta_i^{*3}.
	\end{eqnarray*}
	The last equation is due to $\|\bbeta^*\|_2=1$.
	\item  When $i\neq j\neq k$, then
	\begin{eqnarray*}
		M_{s_{ijk}} &=& \mathbb E\Big(\beta_{i}^*x_i+ \beta_{j}^*x_j + \beta_{k}^*x_k+\sum_{m\neq i,j,k}\beta_m^*x_m\Big)^3x_ix_jx_k\\
		&=& \mathbb E\big(\beta_{i}^*x_i+ \beta_{j}^*x_j + \beta_{k}^*x_k\big)^3x_ix_jx_k\\
		&=& 6\beta_i^*\beta_j^*\beta_k^*.
	\end{eqnarray*}
	\item When $i=j\neq k$, then
	\begin{eqnarray*}
		M_{s_{iik}} &=&  \mathbb E\Big(\beta_{i}^*x_i + \beta_{k}^*x_k+\sum_{m\neq i,k}\beta_m^*x_m\Big)^3x_i^2x_k\\
		&=& 9\beta_i^{*2}\beta_k^*+3\beta_k^{*3}+3\beta_k^*\big(\sum_{m\neq i,k}
		\beta_m^{*2}\big)\\
		&=&  9\beta_i^{*2}\beta_k^*+3\beta_k^*\big(\sum_{m\neq i}\beta_m^{*2}\big)\\
		&=& 3\beta_k^* + 6\beta_i^{*2}\beta_k^*.
	\end{eqnarray*}
\end{itemize}
Therefore, it is sufficient to calculate $M_s$ by
\begin{equation*}
\begin{split}
M_s =& 3\sum_{k=1}^{K}\eta_k^*\Big(\sum_{m=1}^p\bbeta_k^*\circ \be_m\circ \be_m+ \be_m\circ\bbeta_k^*\circ \be_m+  \be_m\circ \be_m\circ\bbeta_k^*\Big)\nonumber\\
&+6\sum_{k=1}^K \eta_k^*\bbeta_k^*\circ\bbeta_k^*\circ\bbeta_k^*.\nonumber
\end{split}
\end{equation*}
The first term is the bias term due to correlations among symmetric sketchings. Denote $M_1 = \frac{1}{n}\sum_{i=1}^ny_i\bx_i$ and note that  $\mathbb E\Big(\frac{1}{n}\sum_{i=1}^ny_i\bx_i\Big)=3\sum_{k=1}^K\eta_k^*\bbeta_k^*$. Therefore, the empirical first-order moment $M_1$ could be used to remove the bias term as follows
\begin{eqnarray*}
	&&\mathbb E \Big(M_s - \sum_{m=1}^{p}\Big(M_1\circ \be_m\circ \be_m+ \be_m\circ M_1\circ \be_m+  \be_m\circ \be_m\circ M_1\Big)\Big)\\
	 &=& 6\sum_{k=1}^K \eta_k^*\bbeta_k^*\circ\bbeta_k^*\circ\bbeta_k^*.
\end{eqnarray*}
This finishes our proof. \hfill $\blacksquare$\\


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Proof of Lemma \ref{lemma:moment_interaction}}\label{proof_moment_inter}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

As before, consider a single component first. For notation simplicity, we drop the subscript $l$ for $l$-th observation and $k$ for $k$-th component. Since each component is normalized, the entry-wise expectation of $(\bbeta^{\top}\bx)^3\bx\circ \bx\circ \bx$ can be calculated as
\begin{eqnarray*}
	&&\Big[\mathbb E(\bbeta^{\top}\bx)^3\bx\circ \bx\circ \bx\Big]_{0,0,0} = 3\beta_0-2\beta_0^3\\
	&&\Big[\mathbb E(\bbeta^{\top}\bx)^3\bx\circ \bx\circ \bx\Big]_{0,0,i} = 3\beta_i\\
	&&\Big[\mathbb E(\bbeta^{\top}\bx)^3\bx\circ \bx\circ \bx\Big]_{0,i,i} = 6\beta_0\beta_i^2+3\beta_0\\
	&&\Big[\mathbb E(\bbeta^{\top}\bx)^3\bx\circ \bx\circ \bx\Big]_{0,i,j} = 6\beta_0\beta_i\beta_j\\
	&&\Big[\mathbb E(\bbeta^{\top}\bx)^3\bx\circ \bx\circ \bx\Big]_{i,i,i} = 6\beta_i^3+9\beta_i\\
	&&\Big[\mathbb E(\bbeta^{\top}\bx)^3\bx\circ \bx\circ \bx\Big]_{i,i,j} = 6\beta_i^2\beta_j+3\beta_j\\
	&&\Big[\mathbb E(\bbeta^{\top}\bx)^3\bx\circ \bx\circ \bx\Big]_{i,j,k} = 6\beta_i\beta_j\beta_k.
\end{eqnarray*}
Due to the symmetric structure and non-randomness of first coordinate, there are bias appearing for each entry. For $i,j,k\neq 0$, we could use $ \sum_{m=1}^p(\ba\circ \be_m\circ \be_m+ \be_m\circ \ba \circ \be_m+\be_m\circ \be_m\circ \ba)$ to remove the bias as shown in the previous proof of Lemma \ref{lemma:moment_symmetric}. For the subscript involving 0, the following two calculations work for removing the bias,
\begin{eqnarray*}
	&&\mathbb E\Big(\frac{1}{3}\cT_s - \frac{1}{6}(\sum_{k=1}^p\cT_{s,[k,k,i]} - (p+1)\ba_i)\Big) = \beta_0^2\beta_i.\\
	&&\mathbb E\Big(\frac{1}{2p-2}(\sum_{k=1}^p\cT_{s[0,k,k]}-(p+2)\cT_{s[0,0,0]})\Big) = \beta_0^3.
\end{eqnarray*} 
This ends the proof. \hfill $\blacksquare$\\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proof of Lemma \ref{lemma:psi_moment_bound}}\label{proof_psi_moment_bound}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Without loss of generality, we assume $\|X_i\|_{\psi_{\alpha}}=1$ and $\mathbb{E}X_i = 0$ throughout this proof. Let $\beta = (\log 2)^{1/\alpha}$ and $Z_i=(|X_i|-\beta)_{+}$, where $(x)_{+} = x$ if $x\geq 0$ and $(x)_{+}=0$ if else. For notation simplicity, we define $ \|X\|_p = (\mathbb E|X|^p)^{1/p}$ for a random variable $X$. The following step is to estimate the moment of linear combinations of variables $\{X_i\}_{i=1}^n$.

According to the symmetrization inequality (e.g., Proposition 6.3 of \cite{ledoux2013probability}), we have 
\begin{equation}\label{ineqn:contration}
    \Big\|\sum_{i=1}^n a_iX_i\Big\|_p\leq 2\Big\|\sum_{i=1}^n a_i\varepsilon_i X_i\Big\|_p = 2\Big\|\sum_{i=1}^na_i\varepsilon_i|X_i|\Big\|_p,
\end{equation}
where $\{\varepsilon_i\}_{i=1}^n$ are independent Rademacher random variables and we notice that $\varepsilon_i X_i$ and $\varepsilon_i|X_i|$ are identically distributed. Moreover, if $|X_i|\geq \beta$, the definition of $Z_i$ implies that $|X_i| = Z_i+\beta$. And if $|X_i|<\beta$, we have $Z_i=0$. Thus, we have $|X_i|\leq Z_i+\beta$ at any time and it leads to
\begin{eqnarray}\label{ineqn:contration_1}
2\Big\|\sum_{i=1}^na_i\varepsilon_i|X_i|\Big\|_p &\leq& 2\Big\|\sum_{i=1}^n a_i\varepsilon_i(\beta+Z_i)\Big\|_p.
\end{eqnarray}
By triangle inequality, 
\begin{eqnarray}\label{ineqn:contration_2}
2\Big\|\sum_{i=1}^n a_i\varepsilon_i(\beta+Z_i)\Big\|_p \leq 2\Big\|\sum_{i=1}^n a_i\varepsilon_iZ_i\Big\|_p + 2\Big\|\sum_{i=1}^n a_i\varepsilon_i\beta\Big\|_p.
\end{eqnarray}

Next, we will bound the second term of the RHS of \eqref{ineqn:contration_2}. In particular, we will utilize Khinchin-Kahane inequality, whose formal statement is included in Lemma \ref{lemma:Khi} for the sake of completeness. From Lemma \ref{lemma:Khi} we have
\begin{eqnarray}\label{ineqn:contration_3}
    \Big\|\sum_{i=1}^n a_i\varepsilon_i\beta\Big\|_p &\leq& \Big(\frac{p-1}{2-1}\Big)^{1/2} \Big\|\sum_{i=1}^n a_i\varepsilon_i\beta\Big\|_2\nonumber\\
    &\leq& \beta\sqrt{p}\Big\|\sum_{i=1}^n a_i\varepsilon_i\Big\|_2.
\end{eqnarray}
Since $\{\varepsilon_i\}_{i=1}^n$ are independent Rademacher random variables, some simple calculations implies
\begin{eqnarray}\label{ineqn:contration_4}
    \Big(\mathbb E\Big(\sum_{i=1}^n \varepsilon_i a_i\Big)^2\Big)^{1/2}&=& \Big(\mathbb E\Big(\sum_{i=1}^n \varepsilon_i^2 a_i^2+2\sum_{1\leq i<j\leq n}\varepsilon_i\varepsilon_j a_i a_j\Big)\Big)^{1/2}\nonumber\\
    &=& \Big(\sum_{i=1}^n a_i^2\mathbb E\varepsilon_i^2 + 2\sum_{1\leq i<j\leq n}a_ia_j\mathbb E\varepsilon_i\mathbb E\varepsilon_j\Big)^{1/2}\nonumber\\
    &=& \Big(\sum_{i=1}^n a_i^2\Big)^{1/2} = \|\ba\|_2.
\end{eqnarray}
Combining inequalities \eqref{ineqn:contration_1}-\eqref{ineqn:contration_4},
\begin{eqnarray}\label{eqn:proof_1}
2\Big\|\sum_{i=1}^na_i\varepsilon_i|X_i|\Big\|_p \leq 2\Big\|\sum_{i=1}^n a_i\varepsilon_iZ_i\Big\|_p + 2\beta \sqrt{p}\|\ba\|_2.
\end{eqnarray}
Let $\{Y_i\}_{i=1}^n$ are independent symmetric random variables satisfying $\mathbb P(|Y_i|\geq t)=\exp(-t^{\alpha})$ for all $t\geq 0$. Then we have 
\begin{equation*}
\begin{split}
\mathbb P(Z_i\geq t) \leq& \mathbb P(|X_i|\geq t+\beta) = \mathbb P\left(\exp(|X_i|^\alpha)\geq \exp((t+\beta)^\alpha)\right) \\
\leq& (\mathbb{E} |X_i|^{\alpha}) \cdot \exp(-(t+\beta)^\alpha) \leq 2\exp(-(t+\beta)^{\alpha})\\
\leq& 2\exp(-t^{\alpha}-\beta^{\alpha}) = \mathbb P(|Y_i|\geq t),
\end{split}
\end{equation*}
which implies
\begin{equation}\label{eqn:proof_2}
    \Big\|\sum_{i=1}^n a_i\varepsilon_iZ_i\Big\|_p\leq \Big\|\sum_{i=1}^n a_i \varepsilon_i Y_i\Big\|_p = \Big\|\sum_{i=1}^n a_i  Y_i\Big\|_p,
\end{equation}
since $\varepsilon_i Y_i$ and $Y_i$ have the same distribution due to symmetry. 
Combining \eqref{eqn:proof_1} and \eqref{eqn:proof_2} together, we reach
\begin{equation}\label{eqn:proof_B1}
    \Big\|\sum_{i=1}^n a_iX_i\Big\|_p\leq 2\beta \sqrt{p}\|\ba\|_2 + 2\Big\|\sum_{i=1}^n a_iY_i\Big\|_p.
\end{equation}

For $0<\alpha <1$, it follows Lemma \ref{lemma:alpha2} that
\begin{equation}\label{eqn:proof_B2}
    \Big\|\sum_{i=1}^n a_i Y_i\Big\|_p \leq C_1(\alpha)(\sqrt{p}\|\ba\|_2 + p^{1/\alpha}\|\ba\|_{\infty}),
\end{equation}
where $C_1(\alpha)$ is some absolute constant only depending on $\alpha$.

For $\alpha\geq 1$, we will combine Lemma \ref{lemma:alpha_1} and the method of the integration by parts to pass from tail bound result to moment bound result. Recall that for every non-negative random variable $X$, integration by parts yields the identity 
\begin{equation*}
    \mathbb E X = \int_{0}^{\infty}\mathbb P(X\geq t)dt.
\end{equation*}
Applying this to $X = |\sum_{i=1}^n a_i Y_i|^p$ and changing the variable $t = t^p$, then we have 
\begin{eqnarray}\label{ineqn:integral}
    \mathbb E|\sum_{i=1}^n a_iY_i|^p &=& \int_{0}^{\infty} \mathbb P\Big(|\sum_{i=1}^n a_iY_i|\geq t\Big) p t^{p-1}dt\nonumber\\
    &\leq &\int_0^{\infty} 2\exp\Big(-c\min\Big(\frac{t^2}{\|\ba\|_2^2}, \frac{t^{\alpha}}{\|\ba\|_{\alpha^*}^{\alpha}}\Big)\Big)pt^{p-1}dt,
\end{eqnarray}
where the inequality is from Lemma \ref{lemma:alpha_1} for all $p\geq 2$ and $1/\alpha+1/\alpha^* = 1$.
In this following, we bound the integral in three steps:
\begin{enumerate}
    \item If $\frac{t^2}{\|\ba\|_2^2}\leq \frac{t^{\alpha}}{\|\ba\|_{\alpha^*}^{\alpha}}$, \eqref{ineqn:integral} reduces to
    \begin{equation*}
          \mathbb E|\sum_{i=1}^n a_iY_i|^p\leq 2p\int_{0}^{\infty}\exp\Big(-c\frac{t^2}{\|\ba\|_2^2}\Big)\Big)t^{p-1}dt.
    \end{equation*}
    Letting $t' = ct^2/\|\ba\|_2^2$, we have 
    \begin{eqnarray*}
        2p\int_{0}^{\infty}\exp\Big(-c\frac{t^2}{\|\ba\|_2^2}\Big)\Big)t^{p-1}dt& =& \frac{p\|\ba\|_2^p}{c^{p/2}}\int_0^{\infty}e^{-t'}t'^{p/2-1}dt'\\
        &=&\frac{p\|\ba\|_2^p}{c^{p/2}} \Gamma(\frac{p}{2})\leq \frac{p\|\ba\|_2^p}{c^{p/2}} (\frac{p}{2})^{p/2},
    \end{eqnarray*}
    where the second equation is from the density of Gamma random variable. Thus,
    \begin{equation}\label{ineqn:moment1}
        \Big(\mathbb E|\sum_{i=1}^n a_iY_i|^p\Big) ^{\tfrac{1}{p}} \leq \frac{p^{1/p}}{(2c)^{1/2}}\sqrt{p}\|\ba\|_2 \leq \frac{\sqrt{2}}{\sqrt{c}}\sqrt{p}\|\ba\|_2.
    \end{equation}
    
    
    \item If $\frac{t^2}{\|\ba\|_2^2}> \frac{t^{\alpha}}{\|\ba\|_{\alpha^*}^{\alpha}}$, \eqref{ineqn:integral} reduces to
    \begin{equation*}
         \mathbb E|\sum_{i=1}^n a_iY_i|^p\leq 2p\int_{0}^{\infty}\exp\Big(-c\frac{t^{\alpha}}{\|\ba\|_{\alpha^*}^{\alpha}}\Big)\Big)t^{p-1}dt.
    \end{equation*}
    Letting $t' = ct^{\alpha}/\|\ba\|_{\alpha^*}^{\alpha}$, we have
    \begin{eqnarray*}
        2p\int_{0}^{\infty}\exp\Big(-c\frac{t^{\alpha}}{\|\ba\|_{\alpha^*}^{\alpha}}\Big)\Big)t^{p-1}dt& =& \frac{2p\|\ba\|_{\alpha^*}^p}{\alpha c^{p/{\alpha}}}\int_0^{\infty}e^{-t'}t'^{p/{\alpha}-1}dt'\\
        &=&\frac{2}{\alpha}\frac{p\|\ba\|_{\alpha^*}^p}{c^{p/{\alpha}}} \Gamma(\frac{p}{{\alpha}})\leq \frac{2}{\alpha}\frac{p\|\ba\|_{\alpha^*}^p}{c^{p/{\alpha}}} (\frac{p}{{\alpha}})^{p/{\alpha}}.
    \end{eqnarray*}
    Thus, 
     \begin{equation}\label{ineqn:moment2}
        \Big(\mathbb E|\sum_{i=1}^n a_iY_i|^p\Big) ^{\tfrac{1}{p}} \leq \frac{{2p}^{1/p}}{(c\alpha)^{1/\alpha}}p^{1/\alpha}\|\ba\|_{\alpha^*} \leq \frac{4}{(c\alpha)^{1/\alpha}}p^{1/\alpha}\|\ba\|_{\alpha^*} .
    \end{equation}
    \item Overall, we have the following by combining \eqref{ineqn:moment1} and \eqref{ineqn:moment2},
    \begin{eqnarray*}
    \Big(\mathbb E|\sum_{i=1}^n a_iY_i|^p\Big) ^{\tfrac{1}{p}}\leq \max\Big(\sqrt{\frac{2}{c}},\frac{4}{(c\alpha)^{1/\alpha}}\Big)\Big(\sqrt{p}\|\ba\|_2 + p^{1/\alpha}\|\ba\|_{\alpha^*} \Big).
    \end{eqnarray*}
    After denoting $C_2(\alpha) = \max\Big(\sqrt{\frac{2}{c}},\frac{4}{(c\alpha)^{1/\alpha}}\Big)$, we reach
    \begin{equation}\label{eqn:proof_B3}
         \Big\|\sum_{i=1}^n a_i Y_i\Big\|_p \leq C_2(\alpha)\Big(\sqrt{p}\|\ba\|_2 + p^{1/\alpha}\|\ba\|_{\alpha^*} \Big).
    \end{equation}
\end{enumerate}
Since $0 < \beta < 1$, the conclusion can be reached by combining \eqref{eqn:proof_B1},\eqref{eqn:proof_B2} and \eqref{eqn:proof_B3}. \hfill $\blacksquare$\\




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proof of Lemma \ref{lemma:perturbation_analysis}}\label{proof_perturbation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Firstly, let us consider the non-symmetric perturbation error analysis. According to Lemma \ref{lemma:moment_asy}, the exact form of $\cE=\cT- \mathbb E(\cT)$ is given by
\begin{eqnarray*}
	\cE = \frac{1}{n}\sum_{i=1}^n y_i\bu_i\circ\bv_i\circ \bw_i - \sum_{k=1}^K\eta_k^*\bbeta_{1k}^*\circ\bbeta_{2k}^*\circ\bbeta_{3k}^*.
\end{eqnarray*}
We decompose it by a concentration term $(\cE_1)$ and a noise term $(\cE_2)$ as follows,
\begin{equation*}
\begin{split}
	\cE =& \underbrace{\frac{1}{n}\sum_{i=1}^n\langle\bu_i\circ\bv_i\circ\bw_i, \sum_{k=1}^K\eta_k^*\bbeta_{1k}^*\circ\bbeta_{2k}^*\circ\bbeta_{3k}^*\rangle\bu_i\circ\bv_i\circ\bw_i-\sum_{k=1}^K\eta_k^*\bbeta_{1k}^*\circ\bbeta_{2k}^*\circ\bbeta_{3k}^*}_{\cE_1}\\
	&+\underbrace{\frac{1}{n}\sum_{i=1}^n\epsilon_i \bu_i\circ \bv_i\circ \bw_i}_{\cE_2}.
	\end{split}
\end{equation*}

\noindent\textbf{Bounding $\cE_1$:} For $k$-th componet of $\cE_1$, we denote 
$$\cE_{1k} = \frac{1}{n}\sum_{i=1}^n\langle\bu_i\circ\bv_i\circ\bw_i, \bbeta_{1k}^*\circ\bbeta_{2k}^*\circ\bbeta_{3k}^*\rangle\bu_i\circ\bv_i\circ\bw_i - \bbeta_{1k}^*\circ\bbeta_{2k}^*\circ\bbeta_{3k}^*.
$$
By using Lemma \ref{lemma:tensor_spectral} and $s\leq d\leq Cs$, it suffices to have for some absolute constant $C_{11}$,
$$
\|\cE_{1k}\|_{s+d} \leq  C_{11}\delta_{n,p,s}, \ \text{where} \ \delta_{n,p,s} = (\log n)^3\Big(\sqrt{\frac{s^3\log^3(p/s)}{n^2}} + \sqrt{\frac{s\log (p/s)}{n}}\Big),
$$ 
with probability at least $1-10/n^3$, where $\|\cdot\|_{s+d}$ is the sparse tensor spectral norm defined in \eqref{def:sparse_spectral}. Equipped with the triangle inequality, the sparse tensor spectral norm for $\cE_1$ can be bounded by 
\begin{equation}
\label{eqn:epsilon_1}
\|\cE_1\|_{s+d} \leq  C_{11}\delta_{n,p,s}\sum_{k=1}^K\eta_k^*,
\end{equation}
with probability at least $1-10K/n^3$.

\noindent\textbf{Bounding $\cE_2$:} Note that the random noise $\{\epsilon_i\}_{i=1}^n$ is independent of sketching vector $\{\bu_i,\bv_i, \bw_i\}$. For fixed $\{\epsilon_i\}_{i=1}^n$, applying Lemma \ref{lemma:tensor_concentration}, we have for some absolute constant $C_{12}$
\begin{eqnarray*}
	\Big\|\frac{1}{n}\sum_{i=1}^n\epsilon_i \bu_i\circ \bv_i\circ \bw_i\Big\|_{s+d} \leq C_{12}\|\bepsilon\|_{\infty} C_{11}\delta_{n,p,s},
\end{eqnarray*}
with probability at least $1-1/p$. According to Lemma \ref{lemma:sub_exp}, we have
\begin{equation}
\label{eqn:epsilon_2}
\mathbb P\Big(\|\cE_2\|_{s+d}\geq C_{12}\sigma\log n\delta_{n,p,s}\Big)\leq  \frac{1}{p}+\frac{3}{n}\leq \frac{4}{n}.
\end{equation}

\noindent\textbf{Bounding $\cE$:}
Putting \eqref{eqn:epsilon_1} and \eqref{eqn:epsilon_2} together, we obtain
\begin{eqnarray*}
	\|\cE\|_{s+d}\leq\Big(C_{11}\sum_{k=1}^K\eta_k^* + C_{12}\sigma\log n\Big)\delta_{n,p,s},
\end{eqnarray*}
with probability at least $1-5/n$. Under Condition \ref{con:noise_non}, we have
\begin{eqnarray*}
	\|\cE\|_{s+d} \leq 2C_1 \sum_{k=1}^K\eta_k^* \delta_{n,p,s}\log n,
\end{eqnarray*}
with probability at least $1-5/n$. 

The perturbation error analysis for the symmetric tensor estimation model and the interaction effect model is similar since the empirical-first-order moment converges much faster than the empirical-third-order moment. So we omit the detailed proof here. \hfill $\blacksquare$\\




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proof of Lemma \ref{lemma:onestep_update_sym}}\label{proof:onestep_update_sym}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Lemma \ref{lemma:onestep_update_sym} quantifies one step update for thresholded gradient update. The proof consists of two parts. 

First, we evaluate an oracle estimator $\{\tilde{\bbeta}_k^{(t+1)}\}_{k=1}^K$ with known support information, which is defined as
\begin{eqnarray}\label{def:oracle_est}
\tilde{\bbeta}_k^{(t+1)} = \varphi_{\frac{\mu}{\phi}h(\bbeta_k^{(t)})}\Big(\bbeta_k^{(t)}-\frac{\mu}{\phi}\nabla_k\cL(\bbeta_k^{(t)})_{F^{(t)}}\Big).
\end{eqnarray}
Here,
\begin{itemize}
	\item $h(\bbeta_k^{(t)})$ is the $k$-th component of $h(\bB^{(t)})$ defined in \eqref{eqn:threshold_level_symmetric}.
	\item $\nabla_{\bB}\cL(\bB) = (\nabla_1\cL(\bbeta_1), \cdots, \nabla_K\cL(\bbeta_K)).$
	\item $F^{(t)}= \cup_{k=1}^K F_k^{(t)}$, where $F_k^{(t)} = \supp(\bbeta_k^*)\cup \supp(\bbeta_k^{(t)})$. 
	\item For a vector $\bx\in\mathbb R^p$ and a subset $A\subset \{1,\ldots, p\}$, we denote $\bx_{A}\in \mathbb R^p$ by keeping the coordinates of $\bx$ with indices in $A$ unchanged, while changing all other components to zero.
\end{itemize}
We will show that $\tilde{\bbeta}_k^{(t+1)}$ converges as a geometric rate for optimization error and an optimal rate for statistical error. See Lemma \ref{lemma:oracle_update_sym} for details. 

Second, we aim to prove that $\tilde{\bbeta}_k^{(t+1)}$ and $\bbeta_k^{(t+1)}$ are almost equivalent with high probability. See Lemma \ref{lemma:oracle_equivalence_sym} for details. For simplicity, we drop the superscript of $\bbeta_k^{(t)}, F^{(t)}$ in the following proof, and denote $\tilde{\bbeta}_k^{(t+1)}$, $\bbeta_k^{(t+1)}$ and $F^{(t+1)}$ by $\tilde{\bbeta}_k^+$, $\tilde{\bbeta}_k^+$ and $F^+$, respectively.


\begin{Lemma}
	\label{lemma:oracle_update_sym}
	Suppose Conditions \ref{con:ident}-\ref{con:sample} hold. Assume \eqref{con:initial_input} is satisfied and $|F|\lesssim Ks$. As long as the step size $\mu\leq 32 R^{-20/3}/(3K[220+270K]^2)$, we obtain the upper bound for $\{\tilde{\bbeta}_k^+\}$,
	\begin{equation}
	\begin{split}
	\sum_{k=1}^K\Big\|\sqrt[3]{\eta_k}\tilde{\bbeta}_k^+-\sqrt[3]{\eta_k^*}\bbeta_k^*\Big\|_2^2\leq&\Big(1-32\mu \frac{R^{-\tfrac{8}{3}}}{K^2}\Big)\sum_{k=1}^K\Big\|\sqrt[3]{\eta_k}\bbeta_k-\sqrt[3]{\eta_k^*}\bbeta_k^*\Big\|_2^2\\
	&+2C_3\mu^2R^{-\tfrac{8}{3}}\eta_{\min}^{*-\tfrac{4}{3}}\frac{\sigma^2K^{-2}s\log p}{n},
	\end{split}
	\end{equation}
	with probability at least $1-(21K^2+11K+4Ks)/n$. 
	\end{Lemma}


%Plugging in $y_i=(\bu_i^{\top}\bbeta_1^*)(\bv_i^{\top}\bbeta_2^*)(\bw_i^{\top}\bbeta_3^*)+\epsilon_i$.



The proof of Lemma \ref{lemma:oracle_update_sym} is postponed to the Section \ref{proof:one-step_sym}. Next lemma guarantees that with high probability, $\{\bbeta_k^+\}_{k=1}^K$ is equivalent to the oracle update $\{\tilde{\bbeta}_k^+\}_{k=1}^K$ with high probability. 
\begin{Lemma}
	\label{lemma:oracle_equivalence_sym}
	Recall that the truncation level $h(\bbeta_k)$ is defined as 
	\begin{equation}\label{def:truncation_level}
	h(\bbeta_k) = \frac{\sqrt{4\log np}}{n}\sqrt{\sum_{i=1}^n\Big(\sum_{k=1}^K\eta_k(\bx_i^{\top}\bbeta_k)^3-y_i\Big)^2\Big(\eta_k(\bx_i^{\top}\bbeta_k)^2\Big)^2}.
	\end{equation}	 
	If $|F|\lesssim Ks$, we have $\bbeta_k^{+}=\tilde{\bbeta}_k^+$ for any $k\in[K]$ with probability at least $1-(n^2p)^{-1}$ and $F^+\subset F$.
\end{Lemma}

The proof of Lemma \ref{lemma:oracle_equivalence_sym} is postponed to the Section \ref{proof:one-step_sym}. By using Lemma \ref{lemma:oracle_equivalence_sym} and induction, we have 
\begin{eqnarray*}
	F^{(t+1)}\subset \cdots F^{(1)}\subset F^{(0)} = \cup_{k=1}^K\supp(\bbeta_k^*)\cup\supp(\bbeta_k^{(0)}).
\end{eqnarray*} 
It implies for every $t$, we have $|F^{(t)}|\lesssim Ks$. Combining with Lemmas \ref{lemma:oracle_update_sym} and \ref{lemma:oracle_equivalence_sym} together, we obtain with probability at least $1-(21K^2+11K+4Ks)/n$,
\begin{equation}
\begin{split}
\sum_{k=1}^K\Big\|\sqrt[3]{\eta_k}\bbeta_k^+-\sqrt[3]{\eta_k^*}\bbeta_k^*\Big\|_2^2\leq &\Big(1-32\mu K^{-2}R^{-\tfrac{8}{3}}\Big)\sum_{k=1}^K\Big\|\sqrt[3]{\eta_k}\bbeta_k-\sqrt[3]{\eta_k^*}\bbeta_k^*\Big\|_2^2\\
&+2C_3\mu^2R^{-\tfrac{8}{3}}\eta_{\min}^{*-\tfrac{4}{3}}\frac{\sigma^2K^{-2}s\log p}{n},
\end{split}
\end{equation}
This ends the proof.
\hfill $\blacksquare$\\



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proof of Lemma \ref{lemma:error_transfer}}\label{proof:error_transfer}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

 Based on the CP low-rank structure of true tensor parameter $\mT^*$, we can explicitly write down the distance between $\mT$ and $\mT^*$ under tensor Frobenius norm as follows
\begin{eqnarray*}
	\Big\|\mT - \mT^*\Big\|_F^2 = \sum_{i_1, i_2, i_3}\Big(\sum_{k=1}^{K}\eta_k\beta_{ki_1}\beta_{ki_2}\beta_{ki_3}-\sum_{k=1}^K\eta_k^*\beta_{ki_1}^*\beta_{ki_2}^*\beta_{ki_3}^*\Big)^2.
\end{eqnarray*}
For notation simplicity, denote $\bar{\bbeta}_k=\sqrt[3]{\eta_k}\bbeta_k, \bar{\bbeta}_k^*=\sqrt[3]{\eta_k^*}\bbeta_k^*$. Then
\begin{equation*}
\begin{split}
	\Big\|\mT - \mT^*\Big\|_F^2=&\sum_{i_1, i_2, i_3}\Big(\sum_{k=1}^{K}\bar{\beta}_{ki_1}\bar{\beta}_{ki_2}\bar{\beta}_{ki_3}-\sum_{k=1}^K\bar{\beta}_{ki_1}^*\bar{\beta}_{ki_2}^*\bar{\beta}_{ki_3}^*\Big)^2\\
	=&\sum_{i_1, i_2, i_3}\Big(\sum_{k=1}^{K}(\bar{\beta}_{ki_1}-\bar{\beta}_{ki_1}^*)\bar{\beta}_{ki_2}^*\bar{\beta}_{ki_3}^*+\sum_{k=1}^{K}\bar{\beta}_{ki_1}(\bar{\beta}_{ki_2}-\bar{\beta}_{ki_2}^*)\bar{\beta}_{ki_3}^*\\
	&+\sum_{k=1}^{K}\bar{\beta}_{ki_1}\bar{\beta}_{ki_2}(\bar{\beta}_{ki_3}-\bar{\beta}_{ki_3}^*)\Big)^2 = \text{RHS}.
	\end{split}
\end{equation*}
Since $(a+b+c)^2\leq 3(a^2+b^2+c^2)$, we have 
\begin{equation*}
\begin{split}
	\text{RHS}\leq& 3\sum_{i_1, i_2, i_3}\Big[(\sum_{k=1}^{K}(\bar{\beta}_{ki_1}-\bar{\beta}_{ki_1}^*)\bar{\beta}_{ki_2}^*\bar{\beta}_{ki_3}^*)^2+(\sum_{k=1}^{K}\bar{\beta}_{ki_1}(\bar{\beta}_{ki_2}-\bar{\beta}_{ki_2}^*)\bar{\beta}_{ki_3}^*)^2\\
	&+(\sum_{k=1}^{K}\bar{\beta}_{ki_1}\bar{\beta}_{ki_2}(\bar{\beta}_{ki_3}-\bar{\beta}_{ki_3}^*))^2\Big].
	\end{split}
\end{equation*}
Equipped with Cauchy-Schwarz inequality, RHS can be further bounded by
\begin{eqnarray*}
	\text{RHS}
	&\leq& 3\sum_{i_1,i_2,i_3}\Big[\sum_{k=1}^{K}(\bar{\beta}_{ki_1}-\bar{\beta}_{ki_1}^*)^2\sum_{k=1}^K\bar{\beta}_{ki_2}^{*2}\bar{\beta}_{ki_3}^{*2}\\
	&&+\sum_{k=1}^{K}(\bar{\beta}_{ki_2}-\bar{\beta}_{ki_2}^*)^2\sum_{k=1}^K\bar{\beta}_{ki_1}^{2}\bar{\beta}_{ki_3}^{*2}\\
	&&+\sum_{k=1}^{K}(\bar{\beta}_{ki_3}-\bar{\beta}_{ki_3}^*)^2\sum_{k=1}^K\bar{\beta}_{ki_2}^{2}\ \bar{\beta}_{ki_1}^{2}\Big]
\end{eqnarray*}
At the same time, using $\eta_k\leq (1+c)\eta_k^*$ for $k\in[K]$,
\begin{eqnarray*}
	\Big\|\mT - \mT^*\Big\|_F^2&\leq& 3\Big[\sum_{i_1=1}^p\sum_{k=1}^{K}(\bar{\beta}_{ki_1}-\bar{\beta}_{ki_1}^*)^2(\sum_{i_2=1}^p\sum_{i_3=1}^p\sum_{k=1}^K\bar{\beta}_{ki_2}^{*2}\bar{\beta}_{ki_3}^{*2})\\
	&&+\sum_{i_2=1}^p\sum_{k=1}^{K}(\bar{\beta}_{ki_2}-\bar{\beta}_{ki_2}^*)^2(\sum_{i_1=1}^p\sum_{i_3=1}^p\sum_{k=1}^K\bar{\beta}_{ki_1}^{2}\bar{\beta}_{ki_3}^{*2})\\
	&&+\sum_{i_3=1}^p\sum_{k=1}^{K}(\bar{\beta}_{ki_3}-\bar{\beta}_{ki_3}^*)^2(\sum_{i_2=1}^p\sum_{i_1=1}^p\sum_{k=1}^K\bar{\beta}_{ki_2}^{2}\bar{\beta}_{ki_1}^{2})\Big]\\
	&=&3\Big(\sum_{k=1}^K\|\bar{\bbeta}_k-\bar{\bbeta}_k^*\|_2^2\Big)\Big(\sum_{k=1}^K(\sqrt[3]{\eta_k^*})^4+\sum_{k=1}^K(\sqrt[3]{\eta_k^*})^2(\sqrt[3]{\eta_k})^2+\sum_{k=1}^K(\sqrt[3]{\eta_k})^4\Big)\\
	&\leq& 9(1+c) \Big(\sum_{k=1}^K\|\bar{\bbeta}_k-\bar{\bbeta}_k^*\|_2^2\Big)\Big(\sum_{k=1}^K(\sqrt[3]{\eta_k^*})^4\Big).
\end{eqnarray*}

For the non-symmetric tensor estimation model, we have
\begin{eqnarray*}
	\Big\|\mT - \mT^*\Big\|_F^2 = \sum_{i_1, i_2, i_3}\Big(\sum_{k=1}^{K}\eta_k\beta_{1ki_1}\beta_{2ki_2}\beta_{3ki_3}-\sum_{k=1}^K\eta_k^*\beta_{1ki_1}^*\beta_{2ki_2}^*\beta_{3ki_3}^*\Big)^2.
\end{eqnarray*}
Following the same strategy above, we obtain
\begin{equation*}
\begin{split}
	\Big\|\mT - \mT^*\Big\|_F^2\leq& 3(1+c) \Big(\sum_{k=1}^K\|\bar{\bbeta}_{1k}-\bar{\bbeta}_{1k}^*\|_2^2+\sum_{k=1}^K\|\bar{\bbeta}_{2k}-\bar{\bbeta}_{2k}^*\|_2^2\\
	&+\sum_{k=1}^K\|\bar{\bbeta}_{3k}-\bar{\bbeta}_{3k}^*\|_2^2\Big)\Big(\sum_{k=1}^K(\sqrt[3]{\eta_k^*})^4\Big).
\end{split}
\end{equation*}
This ends the proof. \hfill $\blacksquare$\\



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proof of Lemma \ref{lemma:oracle_update_sym}}\label{proof:one-step_sym}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

First of all, let us state a lemma to illustrate the effect of weight $\phi$. 
\begin{Lemma}\label{lemma:marginal_effect}
	Consider $\{y_i\}_{i=1}^n$ come from either non-symmetric tensor estimation model \eqref{eq:model_asymmetric} or symmetric tensor estimation model \eqref{eq:model}. Suppose Conditions \ref{con:incoherence_sym}-\ref{con:sample} hold. Then $\phi=\frac{1}{n} \sum_{i=1}^n y_i^2$ is upper and lower bounded by  
	\begin{equation*}
	(16-6\Gamma^3-9\Gamma)(\sum_{k=1}^K\eta_k^*)^2\leq \frac{1}{n}\sum_{i=1}^{n}y_i^2\leq (16+6\Gamma^3+9\Gamma)(\sum_{k=1}^K\eta_k^*)^2, 
	\end{equation*}
	with probability at least $1-(K^2+K+3)/n$, where $\Gamma$ is the incoherence parameter.
\end{Lemma}


According to Lemma \ref{lemma:marginal_effect}, $\frac{1}{n}\sum_{i=1}^ny_i^2$ approximates $(\sum_{k=1}^K\eta_k^*)^2$ up to some constants with high probability. Moreover, we know that from \eqref{con:initial_input}, $\max_{k}|\eta_k-\eta_k^*|\leq \varepsilon_0$ for some small $\varepsilon_0$. Based on those two facts described above, we replace $\eta_k$ by $\eta_k^*$ and $\phi$ by $(\sum_{k=1}^K\eta_k^*)^{2}$ for the sake of completeness. Note that this change could only result in some constant scale changes for final results. Similar simplification was used in matrix recovery scenario \citep{Tu2015}. Therefore, we define the weighted estimator and weighted true parameter as $\bar{\bbeta}_k = \sqrt[3]{\eta_k^*}\bbeta_k$, $\bar{\bbeta}_k^* = \sqrt[3]{\eta_k^*}\bbeta_k^*$.  Correspondingly, define the gradient function $\nabla_k\cL(\bar{\bbeta}_k)$ on $F$ as
\begin{eqnarray*}
	\nabla_k\cL(\bar{\bbeta}_k)_{F}=\frac{6\sqrt[3]{\eta_k^*}}{n}\sum_{i=1}^n\Big(\sum_{k'=1}^K(\bx_{i_{F}}^{\top}\bar{\bbeta}_{k'})^3-y_i\Big)(\bx_{i_{F}}^{\top}\bar{\bbeta}_k)^2\bx_{i_{F}},
\end{eqnarray*}
and its noiseless version as
\begin{equation}
\label{def:noiseless_gradient}
\nabla_k\tilde{\cL}(\bar{\bbeta}_k)_{F}=\frac{6\sqrt[3]{\eta_k^*}}{n}\sum_{i=1}^n\Big(\sum_{k'=1}^K(\bx_{i_{F}}^{\top}\bar{\bbeta}_{k'})^3-\sum_{k'=1}^K(\bx_{i_{F}}^{\top}\bar{\bbeta}^*_{k'})^3\Big)(\bx_{i_F}^{\top}\bar{\bbeta}_k)^2\bx_{i_{F}}.
\end{equation}
According to the definition of thresholding function \eqref{eqn:thresholding}, $\tilde{\bbeta}_k^+$ can be written as 
\begin{equation*}
\tilde{\bbeta}_k^+=\bbeta_k-\frac{\mu}{\phi}\nabla_k\cL(\bar{\bbeta}_k)_{F} +\frac{\mu}{\phi}h(\bar{\bbeta}_k)\bgamma_k,
\end{equation*}
where $\bgamma_k\in \mathbb R^p$ satisfies $\supp(\bgamma_k)\subset F$, $\|\bgamma_k\|_{\infty}\leq 1$ and $h(\bar{\bbeta}_k)$ is defined as
\begin{equation}
\label{def:thresholded_function_sym}
h(\bar{\bbeta}_k) = \frac{\sqrt{4\log(np)}}{n}\sqrt{\sum_{i=1}^n\Big(\sum_{k=1}^K (\bx_{i_{F}}^{\top}\bar{\bbeta}_k)^3-y_i\Big)^2\eta_k^{*\tfrac{2}{3}}(\bx_{i_{F}}^{\top}\bar{\bbeta}_k)^2}.
\end{equation}
Moreover, we denote $\bz_k = \bar{\bbeta}_k-\bar{\bbeta}_k^*$.  With a little abuse of notations, we also drop the subscript $F$ in this section for notation simplicities. 

We expand and decompose the sum of square error by three parts as follows:
\begin{equation}\label{eqn:error_decom}
\begin{split}
&\sum_{k=1}^K\Big\|\sqrt[3]{\eta_k^*}\tilde{\bbeta}_k^+-\sqrt[3]{\eta_k^*}\bbeta^*_k\Big\|_2^2 \\
&= \sum_{k=1}^K\Big\|\bz_k - \frac{\mu\sqrt[3]{\eta_k^*}}{\phi}\nabla_k\cL(\bar{\bbeta}_k) +\frac{\mu\sqrt[3]{\eta_k^*}}{\phi}h(\bar{\bbeta}_k)\bgamma_k\Big\|_2^2\\
&=  \underbrace{\sum_{k=1}^K\Big\|\bz_k-\mu\frac{\sqrt[3]{\eta_k^*}}{\phi}\nabla_k\cL(\bar{\bbeta}_k)\Big\|_2^2}_{\text{A: gradient update effect}}+\underbrace{\sum_{k=1}^K\Big\|\frac{\mu\sqrt[3]{\eta_k^*}}{\phi}h(\bar{\bbeta}_k)\gamma_k\Big\|_2^2}_{\text{B: threshoding effect}}\\
&+\underbrace{\sum_{k=1}^K\Big\langle\bz_k-\mu\frac{\sqrt[3]{\eta_k^*}}{\phi}\nabla_k\cL(\bar{\bbeta}_k), \frac{\mu\sqrt[3]{\eta_k}}{\phi}h(\bar{\bbeta}_k)\gamma_k\Big\rangle}_{\text{C: cross term}}.
\end{split}
\end{equation}
In the following proof, we will bound three parts sequentially. 

\subsubsection{Bounding gradient update effect}
In order to separate the optimization error and statistical error, we use the noiseless gradient $\nabla_k \tilde{\cL}(\bar{\bbeta}_k)$ as a bridge such that $A$ can be decomposed as
\begin{equation}
\label{eqn:symmetric_A}
\begin{split}
A=&\sum_{k=1}^K\|\bz_k\|_2^2- 2\mu\sum_{k=1}^K\Big\langle\frac{\sqrt[3]{\eta_k^*}}{\phi}\nabla_k\cL(\bar{\bbeta}_k), \bz_k\Big\rangle+\mu^2\sum_{k=1}^K\Big\|\frac{\sqrt[3]{\eta_k^*}}{\phi}\nabla_k\cL(\bar{\bbeta}_k)\Big\|_2^2\\
\leq&\sum_{k=1}^K\|\bz_k\|_2^2-2\mu\underbrace{\sum_{k=1}^K\Big\langle\frac{\sqrt[3]{\eta_k^*}}{\phi}\nabla_k\tilde{\cL}(\bar{\bbeta}_k), \bz_k\Big\rangle}_{A_1}+2\mu^2\underbrace{\sum_{k=1}^K\Big\|\frac{\sqrt[3]{\eta_k^*}}{\phi}\nabla_k\tilde{\cL}(\bar{\bbeta}_k)\Big\|_2^2}_{A_2}\\
& + 2\mu^2\underbrace{\sum_{k=1}^K \Big\|\frac{\sqrt[3]{\eta_k^*}}{\phi}\Big(\nabla_k\tilde{\cL}(\bar{\bbeta}_k)-\nabla_k\cL(\bar{\bbeta}_k)\Big)\Big\|_2^2}_{A_3}\\
&+2\mu\underbrace{\sum_{k=1}^K\Big\langle\bz_k, \frac{\sqrt[3]{\eta_k^*}}{\phi}\Big(\nabla_k\tilde{\cL}(\bar{\bbeta}_k)-\nabla_k\cL(\bar{\bbeta}_k)\Big)\Big\rangle}_{A_4},
\end{split}
\end{equation}
where $A_1$ and $A_2$ quantify the optimization error, $A_3$ quantifies the statistical error, and $A_4$ is a cross term which can be negligible comparing with the rate of the statistical error. The lower bound for $A_1$ and upper bound for $A_2$ together coincide with the verification of regularity conditions in the matrix recovery case \citep{CLS15}. 

~\\
\noindent \textbf{Step One: Lower bound for $A_1$.} Plugging in $\phi = (\sum_{k=1}^K\eta_k^*)^{2}$, we have
\begin{eqnarray}\label{ineqn:weight}
K^{-2}R^{-\tfrac{2}{3}}\eta_{\max}^{*-\tfrac{4}{3}}\leq\frac{(\sqrt[3]{\eta_k^*})^2}{\phi} = \frac{(\sqrt[3]{\eta_k^*})^2}{(\sum_{k=1}^K\eta_k^*)^{2}}\leq K^{-2}R^{\tfrac{2}{3}}\eta_{\min}^{*-\tfrac{4}{3}}.
\end{eqnarray}
According to the definition of noiseless gradient $\nabla_k \tilde{\cL}(\bbeta_k)$ and $\bz_k$, $A_1$ can be expanded and decomposed sequentially by nine terms,
\begin{equation}\label{eqn:decomposition}
\begin{split}
A_1 \geq&K^{-2}R^{-\tfrac{2}{3}}\eta_{\max}^{*-\tfrac{4}{3}}\Big[\frac{6}{n}\sum_{i=1}^n\Big(\sum_{k'=1}^K 3(\bx_i^{\top}\bz_{k'})(\bx_i^{\top}\bar{\bbeta}_{k'})^2\sum_{k=1}^K(\bx_i^{\top}\bz_k)(\bx_i^{\top}\bar{\bbeta}_k^*)^2\Big)\Leftarrow \ A_{11}\\
&+\frac{6}{n}\sum_{i=1}^n\Big(\sum_{k'=1}^K 3(\bx_i^{\top}\bz_{k'})(\bx_i^{\top}\bar{\bbeta}_{k'})^2\sum_{k=1}^K2(\bx_i^{\top}\bz_k)^2(\bx_i^{\top}\bar{\bbeta}_k^*)\Big)\Leftarrow \ A_{12}\\
&+\frac{6}{n}\sum_{i=1}^n\Big(\sum_{k'=1}^K 3(\bx_i^{\top}\bz_{k'})(\bx_i^{\top}\bar{\bbeta}_{k'})^2\sum_{k=1}^K(\bx_i^{\top}\bz_k)^3\Big)\Leftarrow \ A_{13}\\
&+\frac{6}{n}\sum_{i=1}^n\Big(\sum_{k'=1}^K 3(\bx_i^{\top}\bz_{k'})^2(\bx_i^{\top}\bar{\bbeta}_{k'})\sum_{k=1}^K(\bx_i^{\top}\bz_k)(\bx_i^{\top}\bar{\bbeta}_k^*)^2\Big)\Leftarrow \ A_{14}\\
&+\frac{6}{n}\sum_{i=1}^n\Big(\sum_{k'=1}^K 3(\bx_i^{\top}\bz_{k'})^2(\bx_i^{\top}\bar{\bbeta}_{k'})\sum_{k=1}^K2(\bx_i^{\top}\bz_k)^2(\bx_i^{\top}\bar{\bbeta}_k^*)\Big)\Leftarrow \ A_{15}\\
&+\frac{6}{n}\sum_{i=1}^n\Big(\sum_{k'=1}^K 3(\bx_i^{\top}\bz_{k'})^2(\bx_i^{\top}\bar{\bbeta}_{k'})\sum_{k=1}^K(\bx_i^{\top}\bz_k)^2(\bx_i^{\top}\bar{\bbeta}_k^*)\Big)\Leftarrow \ A_{16}\\
&+\frac{6}{n}\sum_{i=1}^n\Big(\sum_{k'=1}^K 3(\bx_i^{\top}\bz_{k'})^3\sum_{k=1}^K(\bx_i^{\top}\bz_k)(\bx_i^{\top}\bar{\bbeta}_k^*)^2\Big)\Leftarrow \ A_{17}\\
&+\frac{6}{n}\sum_{i=1}^n\Big(\sum_{k'=1}^K 3(\bx_i^{\top}\bz_{k'})^3\sum_{k=1}^K2(\bx_i^{\top}\bz_k)^2(\bx_i^{\top}\bar{\bbeta}_k^*)\Big)\Leftarrow \ A_{18}\\
&+\frac{6}{n}\sum_{i=1}^n\Big(\sum_{k'=1}^K 3(\bx_i^{\top}\bz_{k'})^3\sum_{k=1}^K(\bx_i^{\top}\bz_k)^3\Big)\Big]\Leftarrow \ A_{19},
\end{split}
\end{equation}
where $A_{11}$ is the main term according to the order of $\bar{\bbeta}_k^*$, while $A_{12}$ to $A_{19}$ are remainder terms. The proof of lower bound for $A_{11}$ to $A_{19}$ follows two steps:
\begin{enumerate}
	\item Calculate and lower bound the expectation of each term through Lemma \ref{cor:expectation_gaussian_vector}: high-order Gaussian moment;
	\item Argue that the empirical version is concentrated around their expectation with high probability through Lemma \ref{cor:concentr_high_order}: high-order concentration inequality.
\end{enumerate}

\textbf{Bounding $A_{11}$.} Note that $A_{11}$ involves the product of dependent Gaussian vectors. This brings difficulties on both the calculation of expectations and the use of concentration inequality.  According to the high-order Gaussian moment results in Lemma \ref{cor:expectation_gaussian_vector}, the expectation of $A_{11}$ can be calculated explicitly as  
\begin{equation}\label{eqn:expectation_A11}
\begin{split}
\mathbb E(A_{11}) &= 36 \sum_{k=1}^K\sum_{k'=1}^K (\bar{\bbeta}_{k'}^{*\top}\bar{\bbeta}_k^*)^2(\bz_{k'}^{\top}\bz_k) \Leftarrow \ I_{1}\\
&+72 \sum_{k=1}^K\sum_{k'=1}^K (\bar{\bbeta}_{k'}^{*\top}\bar{\bbeta}_k^*)(\bz_{k'}^{\top}\bar{\bbeta}_k^*)(\bz_k^{\top}\bar{\bbeta}_{k'}^*) \Leftarrow \ I_{2}\\
&+108 \sum_{k=1}^K\sum_{k'=1}^K (\bar{\bbeta}_{k'}^{*\top}\bar{\bbeta}_k^*)(\bz_{k'}^{\top}\bar{\bbeta}_{k'}^*)(\bz_k^{\top}\bar{\bbeta}_k^*)\Leftarrow \ I_{3}\\
&+54 \sum_{k=1}^K\sum_{k'=1}^K (\bar{\bbeta}_{k'}^{*\top}\bar{\bbeta}_{k'}^*)(\bar{\bbeta}_{k}^{*\top}\bar{\bbeta}_{k}^*)(\bz_{k'}^{\top}\bz_k)\Leftarrow \ I_{4}.
\end{split}
\end{equation}
Note that $I_1$ to $I_4$ involve the summation of $K^2$ term. To use incoherence Condition  \ref{con:incoherence_sym},  we isolate $K$ terms with $k=k'$. Then, $I_1$ to $I_4$ could be lower bounded as 
\begin{equation*}
\begin{split}
I_1&\geq 36\eta_{\min}^{*4/3}\Big[\sum_{k=1}^K \|\bz_k\|_2^2- \Gamma^2\Big(\sum_{k=1}^K\|\bz_k\|_2\Big)^2\Big]\\
I_2&\geq 72\eta_{\min}^{*4/3}\Big[\sum_{k=1}^K (\bz_k^{\top}\bar{\bbeta}_k^*)^2- \Gamma\Big(\sum_{k=1}^K\|\bz_k\|_2\Big)^2\Big]\\
I_3&\geq 108\eta_{\min}^{*4/3}\Big[\sum_{k=1}^K (\bz_k^{\top}\bar{\bbeta}_k^*)^2- \Gamma\Big(\sum_{k=1}^K\|\bz_k\|_2\Big)^2\Big]\\
I_4&\geq 54\eta_{\min}^{*4/3}\Big\|\sum_{k=1}^{K}\bz_k\Big\|_2^2\geq 0,
\end{split}
\end{equation*}
where $\Gamma$ is the incoherence parameter. Putting the above four bounds together, they jointly provide
\begin{equation}\label{ineqn:S4}
\mathbb E(A_{11})\geq 36\eta_{\min}^{*4/3}\sum_{k=1}^K \|\bz_k\|_2^2 - \Big(36\eta_{\min}^{*4/3}\Gamma^2 +180\eta_{\min}^{*4/3}\Gamma\Big)\Big(\sum_{k=1}^K\|\bz_k\|_2\Big)^2.
\end{equation}



On the other hand, repeatedly using Lemma \ref{cor:concentr_high_order}, we obtain that with probability at least $1-1/n$,
\begin{equation*}
\begin{split}
	&\Big|\frac{1}{n}\sum_{i=1}^n\Big((\bx_i^{\top}\bz_{k'})(\bx_i^{\top}\bar{\bbeta}_{k'}^*)^2(\bx_i^{\top}\bz_k)(\bx_i^{\top}\bar{\bbeta}_k^*)^2-\mathbb E(\bx_i^{\top}\bz_{k'})(\bx_i^{\top}\bar{\bbeta}_{k'}^*)^2(\bx_i^{\top}\bz_k)(\bx_i^{\top}\bar{\bbeta}_k^*)^2\Big)\Big|\\
	&\leq C\frac{(\log n)^3}{\sqrt{n}}(\sqrt[3]{\eta_{\max}^*})^4\|\bz_{k'}\|_2\|\bz_k\|_2.
	\end{split}
\end{equation*}
Taking the summation over $k,k'\in[K]$, it could further imply that for some absolute constant $C$,
\begin{eqnarray} \label{ineqn:S5}
\Big|A_{11}-\mathbb E(A_{11})\Big|\leq 18C\frac{(\log n)^3}{\sqrt{n}}(\sqrt[3]{\eta_{\max}^*})^4\Big(\sum_{k=1}^{K}\|\bz_{k}\|_2\Big)^2,
\end{eqnarray}
with probability at least $1-K^2/n$. Combining \eqref{ineqn:S4} and \eqref{ineqn:S5}, we obtain with probability at least $1-K^2/n$,
\begin{equation}\label{eqn:bound_A11}
\begin{split}
&K^{-2}R^{-\tfrac{2}{3}}\eta_{\max}^{*-\tfrac{4}{3}}A_{11}\\
\geq &\Big[36K^{-2}R^{-\tfrac{8}{3}}-K^{-\tfrac{3}{2}} \Big(216R^{-\tfrac{8}{3}}\Gamma+18C\frac{(\log n)^3}{\sqrt{n}}\Big)\Big]\sum_{k=1}^K \|\bz_k\|_2^2,
\end{split}
\end{equation}
where $R = \eta_{\max}^*/\eta_{\min}^*$. Here, we use the fact $\Gamma \leq 1$ and $(\sum_{k=1}^K\|\bz_k\|_2)^2\leq K(\sum_{k=1}^K\|\bz_k\|_2^2)$.

\textbf{Bounding $A_{12}$ to $A_{19}$:} For remainder terms, we follow the same proof strategy. According to Lemma \ref{cor:expectation_gaussian_vector}, the expectation of $A_{12}$ can be calculated as 
\begin{eqnarray*}
	\mathbb E(A_{12}) &=& 36 \sum_{k=1}^K\sum_{k'=1}^K (\bz_k^{\top}\bar{\bbeta}_{k'}^{*\top})^2(\bz_{k'}^{\top}\bar{\bbeta}_k^*) \Leftarrow \ I_{1}\\
	&&+72 \sum_{k=1}^K\sum_{k'=1}^K (\bz_k^{\top}\bar{\bbeta}_{k'}^*)(\bar{\bbeta}_{k'}^{*\top}\bar{\bbeta}_k^*)(\bz_{k'}^{\top}\bz_k) \Leftarrow \ I_{2}\\
	&&+108 \sum_{k=1}^K\sum_{k'=1}^K (\bz_k^{\top}\bar{\bbeta}_{k'})(\bz_{k'}^{\top}\bar{\bbeta}_{k'}^*)(\bz_k^{\top}\bar{\bbeta}_k^*)\Leftarrow \ I_{3}\\
	&&+54 \sum_{k=1}^K\sum_{k'=1}^K (\bar{\bbeta}_{k'}^{*\top}\bar{\bbeta}_{k'}^*)(\bz_{k'}^{\top}\bar{\bbeta}_{k}^*)(\bz_{k}^{\top}\bz_k)\Leftarrow \ I_{4}.
\end{eqnarray*}
Let us analyze $I_1$ first. Under \eqref{con:initial_input}, $\|\bz_k\|_2\leq \varepsilon_0\sqrt[3]{\eta_k^*}$, it suffices to show that 
\begin{eqnarray*}
	\sum_{k=1}^K\sum_{k'=1}^K(\bz_k^{\top}\bar{\bbeta}_{k'})^2(\bz_{k'}^{\top}\bar{\bbeta}_k^*)&\geq& -\sum_{k=1}^K\sum_{k'=1}^{K}\|\bz_k\|_2^2\|\bar{\bbeta}_{k'}^*\|_2^2\|\bz_k'\|_2\|\bar{\bbeta}_{k}^*\|_2\\
	&\geq& -\eta_{\max}^{*\tfrac{4}{3}}\varepsilon_0\Big(\sum_{k=1}^K\|\bz_k\|_2\Big)^2.
\end{eqnarray*}
This immediately implies a lower bound for $\mathbb E(A_{12})$ after we bound similarly for $I_2,I_3$ and $I_4$,
\begin{equation}
\mathbb E(A_{12})\geq -270\eta_{\max}^{*\tfrac{4}{3}}\varepsilon_0\Big(\sum_{k=1}^K\|\bz_k\|_2\Big)^2.
\end{equation}
By Lemma \ref{cor:concentr_high_order}, we obtain for some absolute constant $C$,
\begin{equation}\label{eqn:bound_A12}
\begin{split}
&K^{-2}R^{-\tfrac{2}{3}}\eta_{\max}^{*-\tfrac{4}{3}}A_{12}\\
 \geq& K^{-2}R^{-\tfrac{2}{3}}\eta_{\max}^{*-\tfrac{4}{3}}\Big[\mathbb E(A_{12}) - 18C\eta_{\max}^{*\tfrac{4}{3}}\varepsilon_0\Big(\sum_{k=1}^K\|\bz_k\|_2\Big)^2\frac{(\log n)^3}{\sqrt{n}}\Big]\\
\geq&-K^{-1}R^{-\tfrac{2}{3}}\varepsilon_0 \Big(270+18C\frac{(\log n)^3}{\sqrt{n}}\Big)\Big(\sum_{k=1}^K\|\bz_k\|_2^2\Big),
\end{split}
\end{equation}
with probability at least $1-K^2/n$. The detail derivation is the same as in \eqref{eqn:bound_A11}, so we omit here.

Similarly, the lower bounds of $A_{13}$ to $A_{19}$ can be derived as follows 
\begin{equation}\label{eqn:boundrest}
\begin{split}
&K^{-\tfrac{1}{2}}\eta_{\max}^{*-\tfrac{4}{3}}A_{14}\geq -K^{\tfrac{1}{2}}\varepsilon_0 \Big(270+18C\frac{(\log n)^3}{\sqrt{n}}\Big)\Big(\sum_{k=1}^K\|\bz_k\|_2^2\Big)\\
&K^{-\tfrac{1}{2}}\eta_{\max}^{*-\tfrac{4}{3}}A_{13}, A_{15}, A_{17}\geq -K^{\tfrac{1}{2}}\varepsilon_0^2 \Big(270+18C\frac{(\log n)^3}{\sqrt{n}}\Big)\Big(\sum_{k=1}^K\|\bz_k\|_2^2\Big)\\
&K^{-\tfrac{1}{2}}\eta_{\max}^{*-\tfrac{4}{3}}A_{16},A_{18}\geq -K^{\tfrac{1}{2}}\varepsilon_0^3 \Big(270+18C\frac{(\log n)^3}{\sqrt{n}}\Big)\Big(\sum_{k=1}^K\|\bz_k\|_2^2\Big)\\
&K^{-\tfrac{1}{2}}\eta_{\max}^{*-\tfrac{4}{3}}A_{19}\geq -K^{\tfrac{1}{2}}\varepsilon_0^4 \Big(270+18C\frac{(\log n)^3}{\sqrt{n}}\Big)\Big(\sum_{k=1}^K\|\bz_k\|_2^2\Big).
\end{split}
\end{equation}
Putting  \eqref{eqn:bound_A11}, \eqref{eqn:bound_A12} and \eqref{eqn:boundrest} together, we have with probability at least $1-9K^2/n$,
\begin{eqnarray*}
	A_1&\geq& \Big[36K^{-2}R^{-\tfrac{8}{3}}-K^{-\tfrac{3}{2}}\Big(2160R^{-\tfrac{3}{3}}\Gamma+18C\frac{(\log n)^3}{\sqrt{n}}\Big) \\
	&&- 8\varepsilon_0K^{-1}R^{-\tfrac{2}{3}}\Big(270+18C\frac{(\log n)^3}{\sqrt{n}}\Big)\Big]\Big(\sum_{k=1}^K\|\bz_k\|_2^2\Big).
\end{eqnarray*}
For the above bound,
\begin{itemize}
	\item When the sample size satisfies $n\geq (18CK^{1/2}R^{8/3}(\log n)^3)^2$, we have
	\begin{equation*}
	\max\Big\{ 18K^{-\tfrac{3}{2}}C\frac{(\log n)^3}{\sqrt{n}},8\varepsilon_0 K^{-1}R^{-\tfrac{2}{3}}18C\frac{(\log n)^3}{\sqrt{n}}\Big\}\leq K^{-2}R^{-\tfrac{8}{3}}.
	\end{equation*}
	\item When $\varepsilon_0\leq K^{-1}R^{-2}/2160$, we have
	\begin{equation*}
	8\varepsilon_0 K^{-1}R^{-\tfrac{2}{3}}270\leq K^{-2}R^{-\tfrac{8}{3}}.
	\end{equation*}
	\item When the incoherence parameter satisfies $\Gamma\leq K^{-1/2}/216$, we have
	\begin{equation*}
	K^{-\tfrac{3}{2}}2160R^{-\tfrac{8}{3}}\Gamma\leq K^{-2}R^{-\tfrac{8}{3}}.
	\end{equation*}
\end{itemize} 
Note that those above conditions can be fulfilled by Conditions \ref{con:incoherence_sym}, \ref{con:sample} and \eqref{con:initial_input}. Thus,  we are able to simplify $A_1$ by
\begin{equation}\label{ineqn:bound_A1}
A_1\geq 32K^{-2}R^{-\tfrac{8}{3}}\Big(\sum_{k=1}^{K}\|\bz_k\|_2^2\Big),
\end{equation}
with probability at least $1-9K^2/n$.


~\\
\noindent  \textbf{Step Two: Upper bound for $A_2$.}
We observe the fact that
\begin{equation}\label{eqn:def:A2}
\begin{split}
A_2=&\sum_{k=1}^K\Big\|\frac{1}{\phi}\sqrt[3]{\eta_k^*}\nabla_k\tilde{\cL}(\bar{\bbeta}_k)\Big\|_2^2\\
=&\sup_{\bw\in\mathbb S^{Ks-1}}\Big|\Big\langle\sum_{k=1}^{K}\frac{\sqrt[3]{\eta_k^*}}{\phi}\nabla_k\tilde{\cL}(\bar{\bbeta}_k), \bw\Big\rangle\Big|^2,
\end{split}
\end{equation} 
where $\mathbb S$ is a unit sphere. It is equivalent to show for any $\bw\in\mathbb S^{Ks-1}$, $A'_2 =|\langle\sum_{k=1}^{K}\frac{\sqrt[3]{\eta_k^*}}{\phi}\nabla_k\tilde{\cL}(\bar{\bbeta}_k), \bw\rangle| $ is upper bounded. According to the definition of noiseless gradient \eqref{def:noiseless_gradient}, $A_2'$ is explicitly written as
\begin{equation*}
A_2' = \frac{6}{n}\sum_{i=1}^n\Big(\sum_{k'=1}^K(\bx_i^{\top}\bar{\bbeta}_{k'})^3-\sum_{k'=1}^{K}(\bx_i^{\top}\bar{\bbeta}_{k'}^*)^3\Big)\Big(\sum_{k=1}^K\frac{(\sqrt[3]{\eta_k^*})^2}{\phi}(\bx_i^{\top}\bar{\bbeta}_k)^2(\bx_i^{\top}\bw)\Big).
\end{equation*}
Following by \eqref{ineqn:weight} and \eqref{eqn:decomposition}, similar decomposition can be made for $A_2'$ as follows, where the only difference is that we replace one $\bx_i^{\top}\bz_k$ by $\bx_i^{\top}\bw$.
\begin{eqnarray*}
	A_2' &\leq&K^{-2}R^{\tfrac{2}{3}}\eta_{\min}^{*-\tfrac{4}{3}}\Big[\frac{6}{n}\sum_{i=1}^n\Big(\sum_{k'=1}^K 3(\bx_i^{\top}\bz_{k'})(\bx_i^{\top}\bar{\bbeta}_{k'})^2\sum_{k=1}^K(\bx_i^{\top}\bw)(\bx_i^{\top}\bar{\bbeta}_k^*)^2\Big)\Leftarrow \ A_{21}'\\
	&&+\frac{6}{n}\sum_{i=1}^n\Big(\sum_{k'=1}^K 3(\bx_i^{\top}\bz_{k'})(\bx_i^{\top}\bar{\bbeta}_{k'})^2\sum_{k=1}^K2(\bx_i^{\top}\bz_k)(\bx_i^{\top}\bw)(\bx_i^{\top}\bar{\bbeta}_k^*)\Big)\Leftarrow \ A_{22}'\\
	&&+\frac{6}{n}\sum_{i=1}^n\Big(\sum_{k'=1}^K 3(\bx_i^{\top}\bz_{k'})(\bx_i^{\top}\bar{\bbeta}_{k'})^2\sum_{k=1}^K(\bx_i^{\top}\bz_k)^2(\bx_i^{\top}\bw)\Big)\Leftarrow \ A_{23}'\\
	&&+\frac{6}{n}\sum_{i=1}^n\Big(\sum_{k'=1}^K 3(\bx_i^{\top}\bz_{k'})^2(\bx_i^{\top}\bar{\bbeta}_{k'})\sum_{k=1}^K(\bx_i^{\top}\bw)(\bx_i^{\top}\bar{\bbeta}_k^*)^2\Big)\Leftarrow \ A_{24}'\\
	&&+\frac{6}{n}\sum_{i=1}^n\Big(\sum_{k'=1}^K 3(\bx_i^{\top}\bz_{k'})^2(\bx_i^{\top}\bar{\bbeta}_{k'})\sum_{k=1}^K2(\bx_i^{\top}\bz_k)(\bx_i^{\top}\bw)(\bx_i^{\top}\bar{\bbeta}_k^*)\Big)\Leftarrow \ A_{25}'\\
	&&+\frac{6}{n}\sum_{i=1}^n\Big(\sum_{k'=1}^K 3(\bx_i^{\top}\bz_{k'})^2(\bx_i^{\top}\bar{\bbeta}_{k'})\sum_{k=1}^K(\bx_i^{\top}\bz_k)(\bx_i^{\top}\bw)(\bx_i^{\top}\bar{\bbeta}_k^*)\Big)\Leftarrow \ A_{26}'\\
	&&+\frac{6}{n}\sum_{i=1}^n\Big(\sum_{k'=1}^K 3(\bx_i^{\top}\bz_{k'})^3\sum_{k=1}^K(\bx_i^{\top}\bw)(\bx_i^{\top}\bar{\bbeta}_k^*)^2\Big)\Leftarrow \ A_{27}'\\
	&&+\frac{6}{n}\sum_{i=1}^n\Big(\sum_{k'=1}^K 3(\bx_i^{\top}\bz_{k'})^3\sum_{k=1}^K2(\bx_i^{\top}\bz_k)(\bx_i^{\top}\bw)(\bx_i^{\top}\bar{\bbeta}_k^*)\Big)\Leftarrow \ A_{28}'\\
	&&+\frac{6}{n}\sum_{i=1}^n\Big(\sum_{k'=1}^K 3(\bx_i^{\top}\bz_{k'})^3\sum_{k=1}^K(\bx_i^{\top}\bz_k)^2(\bx_i^{\top}\bw)\Big)\Big].\Leftarrow \ A_{29}'\\
\end{eqnarray*}


Let's bound $A_{21}'$ first. By using the same technique when calculating $\mathbb E(A_{11})$ in \eqref{eqn:expectation_A11}, we derive an upper bound for $\mathbb E(A_{21}')$,
\begin{eqnarray*}
	\mathbb E(A_{21}')&\leq& 36\eta_{\max}^{*\tfrac{4}{3}}\Big(\sum_{k=1}^{K}\|\bz_k\|_2+(K-1)\sum_{k=1}^{K}\Gamma \|\bz_k\|_2\Big)\\
	&+&180\eta_{\max}^{*\tfrac{4}{3}}\Big(\sum_{k=1}^{K}\|\bz_k\|_2+(K-1)\sum_{k=1}^{K}\Gamma\|\bz_k\|_2\Big)
	 +54\eta_{\max}^{*\tfrac{4}{3}}\Big(K\sum_{k=1}^{K}\|\bz_k\|_2\Big).
\end{eqnarray*}
Equipped with Lemma \ref{lemma:tensor_spectral} and the definition of tensor spectral norm \eqref{def:sparse_spectral}, it suffices to bound $A_{21}'$ by
\begin{eqnarray*}
	R^{\tfrac{2}{3}}\eta_{\min}^{*-\tfrac{4}{3}}K^{-\tfrac{1}{2}}A_{21}'\leq K^{-2}R^{2}\Big[216+54K+216K\Gamma+18CK\delta_{n,p,s}\Big]\Big(\sum_{k=1}^{K}\|\bz_k\|_2\Big)
\end{eqnarray*} 
with probability at least $1-10K^2/n^3$, where $\delta_{n,p,s}$ is defined in \eqref{eqn:initial_stat_rate}.

The upper bounds for $A_{22}'$ to $A_{29}'$ follow similar forms. Combining them together, we can derive an upper bound for $A_2'$ as follows
\begin{eqnarray*}
	A_2'&\leq& K^{-2}R^{2}\Big[216+270K+18CK\delta_{n,p,s}\Big]\Big(\sum_{k=1}^{K}\|\bz_k\|_2\Big)\\
	&\leq& K^{-2}R^{2}\Big[220+270K\Big]\Big(\sum_{k=1}^{K}\|\bz_k\|_2\Big),
\end{eqnarray*} 
with probability at least $1-90K^2/n^3$, where the second inequality utilizes Condition \ref{con:sample}. Therefore, the upper bound of $A_2$ is given as follows
\begin{equation}\label{ineqn:bound_A2}
A_2\leq K^{-1}R^{4}[220+270K]^2\Big(\sum_{k=1}^K\|\bz_k\|_2^2\Big),
\end{equation} 
with probability at least $1-90K^2/n^3$.





~\\
\noindent  \textbf{Step Three: Upper bound for $A_3$.}
By the definition of noisy gradient and noiseless gradient, $A_3$ is explicitly written as
\begin{eqnarray*}
	A_3 &=& \sum_{k=1}^K\Big\|\frac{(\sqrt[3]{\eta_k^*})^2}{\phi}\frac{6}{n}\sum_{i=1}^n\epsilon_i(\bx_i^{\top}\bar{\bbeta}_k)^2\bx_i\Big\|_2^2\\
	&\leq& K^{-4}R^{\tfrac{4}{3}}\eta_{\min}^{*-\tfrac{8}{3}}\sum_{k=1}^{K}\Big(\sqrt{Ks}\max_j\frac{6}{n}\sum_{i=1}^n\epsilon_i(\bx_i^{\top}\bar{\bbeta}_k)^2x_{ij}\Big)^2,
\end{eqnarray*} 
where the second inequality comes from \eqref{ineqn:weight}. For fixed $\{\epsilon_i\}_{i=1}^n$, applying Lemma \ref{cor:concentr_high_order}, we have
\begin{eqnarray*}
	\Big|\sum_{i=1}^n\epsilon_i(\bx_i^{\top}\bar{\bbeta}_k)^2x_{ij} - \mathbb E\Big(\sum_{i=1}^n\epsilon_i(\bx_i^{\top}\bar{\bbeta}_k)^2x_{ij}\Big)\Big|\leq C(\log n)^{\tfrac{3}{2}}\|\bepsilon\|_2\|\bar{\bbeta}_k\|_2^2,
\end{eqnarray*}
with probability at least $1-1/n$. Together with Lemma \ref{lemma:sub_exp}, we obtain for any $j\in[Ks]$, 
\begin{eqnarray*}
	\Big|\frac{6}{n}\sum_{i=1}^n \epsilon_i(\bx_i^{\top}\bar{\bbeta}_k)^2x_{ij}\Big|\leq 6CC_0\sigma \|\bar{\bbeta}_k\|_2^2\frac{(\log n)^{3/2}}{\sqrt{n}},
\end{eqnarray*}
with probability at least $1-4/n$, where $\sigma$ is the noise level. According to \eqref{con:initial_input}, 
\begin{eqnarray*}
	\Big\|\bar{\bbeta}_k-\bar{\bbeta}_k^*\Big\|_2^2\leq \sum_{k=1}^K\Big\|\bar{\bbeta}_k-\bar{\bbeta}_k^*\Big\|_2^2\leq K\eta_{\max}^{*\tfrac{2}{3}}\varepsilon_0^2,
\end{eqnarray*}
which further implies $\|\bar{\bbeta}_k\|_2^2\leq (1+K^{\tfrac{1}{2}}\varepsilon_0)^2\eta_{\max}^{*\tfrac{2}{3}}$. Equipped with union bound over $j\in[Ks]$,
\begin{eqnarray*}
	\max_{j\in[Ks]}\Big|\frac{6}{n}\sum_{i=1}^n \epsilon_i(\bx_i^{\top}\bar{\bbeta}_k)^2x_{ij}\Big|\leq 6CC_0\sigma (1+K^{\tfrac{1}{2}}\varepsilon_0)^2(\sqrt[3]{\eta_{\max}^*})^2\frac{(\log n)^{3/2}}{\sqrt{n}},
\end{eqnarray*}
with probability at least $1-4Ks/n$. Letting $C=6C_0(Ce)^{-2/3}(1+K^{\tfrac{1}{2}}\varepsilon_0)^2$,
\begin{eqnarray}\label{ineqn:bound_A3}
A_3\leq C\eta_{\min}^{*-\tfrac{4}{3}}R^{\tfrac{8}{3}}\sigma^2K^{-2}\frac{s(\log n)^3}{n},
\end{eqnarray}
with probability at least $1-4Ks/n$.








~\\
\noindent  \textbf{Step Four: Upper bound for $A_4$.} This cross term can be written as 
\begin{eqnarray*}
	A_4 = 2\sum_{k=1}^{K}\frac{\mu}{\phi}(\sqrt[3]{\eta_k^*})^2\Big(\frac{1}{n}\sum_{i=1}^n\epsilon_i(\bx_i^{\top}\bar{\bbeta}_k)^2(\bx_i^{\top}\bz_k)\Big).
\end{eqnarray*}
To bound this term, we take the same step in Step Three which fixes the noise term $\{\epsilon_i\}_{i=1}^n$ first. Similarly, we obtain with probability at least $1-4K/n$, 
\begin{eqnarray}\label{ineqn:bound_A4}
A_4\leq 2C\sigma \frac{(\log n)^{\tfrac{3}{2}}}{\sqrt{n}}K^{-1}R^{\tfrac{4}{3}}\eta_{\min}^{*-\tfrac{2}{3}}.
\end{eqnarray} 
This term is negligible in terms of the order when comparing with \eqref{ineqn:bound_A3}.

~\\
\noindent  \textbf{Summary.} Putting the bounds \eqref{ineqn:bound_A1}, \eqref{ineqn:bound_A2}, \eqref{ineqn:bound_A3} and \eqref{ineqn:bound_A4} together, we achieve an upper bound for gradient update effect as follows,
\begin{equation}\label{upper_bound:gradient}
\begin{split}
A\leq &\Big(1-64\mu K^{-2}R^{-\tfrac{8}{3}}+2\mu^2K^{-1}R^4[220+270K]^2\Big)\sum_{k=1}^K\|\bz_k\|_2^2\\
&+4\mu CK^{-2}\eta_{\min}^{*-\tfrac{4}{3}}R^{\tfrac{8}{3}}\frac{\sigma^2s(\log n)^3}{n},
\end{split}
\end{equation}
with probability at least $1-(18K^2+4K+4Ks)/n$.\hfill $\blacksquare$\\	


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Bounding thresholding effect}\label{subsubsection_threshold}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The thresholding effect term in \eqref{eqn:error_decom} can also be decomposed into optimization error and statistical error. Recall that $B$ can be explicitly written as
\begin{eqnarray*}
	B = \sum_{k=1}^K\Big\|\mu \frac{\eta_k^{*\tfrac{2}{3}}}{\phi}\frac{4\sqrt{\log (np)}}{n}\sqrt{\sum_{i=1}^n\Big(\sum_{k'=1}^K(\bx_i^{\top}\bar{\bbeta}_{k'})^3-y_i\Big)^2(\bx_i^{\top}\bar{\bbeta}_k)^4}\gamma_k\Big\|_2^2,
\end{eqnarray*}
where $\supp(\gamma_k)\subset F_k$ and $\|\gamma_k\|_{\infty}\leq 1$. By using $(a+b)^2\leq 2(a^2+b^2)$, we have
\begin{equation*}
\begin{split}
	B\leq& \mu^2 \frac{64Ks\log p}{n}\Big[\underbrace{\frac{1}{n}\sum_{i=1}^n\Big(\sum_{k'=1}^K(\bx_i^{\top}\bar{\bbeta}_{k'})^3-\sum_{k'=1}^K(\bx_i^{\top}\bar{\bbeta}_{k'}^*)^3\Big)\Big(\sum_{k=1}^K\frac{\eta_k^{*\tfrac{4}{3}}}{\phi^2}(\bx_i^{\top}\bar{\bbeta}_k)^4\Big)}_{B_1:\text{optimization error}}\\
	&+\underbrace{\frac{1}{n}\sum_{i=1}^n\epsilon_i^2\sum_{k=1}^K\frac{\eta_k^{*\tfrac{4}{3}}}{\phi^2}(\bx_i^{\top}\bar{\bbeta}_k)^4}_{B_2:\text{statistical error}}\Big]. 
	\end{split}
\end{equation*}

~\\
\noindent  \textbf{Bounding $B_1$.} This optimization error term shares similar structure with \eqref{eqn:def:A2} but with higher order. Therefore, we follow the same idea as we did in bounding \eqref{eqn:def:A2}. Following by \eqref{ineqn:weight} and some basic expansions and inequalities, 
\begin{equation*}
\begin{split}
	B_1\leq& K^{-2}R^{\tfrac{4}{3}}\eta_{\min}^{*-\tfrac{8}{3}}\frac{1}{n}\Big(\sum_{k'=1}^K(\bx_i^{\top}\bar{\bbeta}_{k'})^3-\sum_{k'=1}^K(\bx_i^{\top}\bar{\bbeta}_{k'}^*)^3\Big)\Big(\sum_{k=1}^K(\bx_i^{\top}\bar{\bbeta}_k)^4\Big)\\
	\leq& K^{-2}R^{\tfrac{4}{3}}\eta_{\min}^{*-\tfrac{8}{3}}\Big[\frac{1}{n}\sum_{i=1}^n\Big(\sum_{k=1}^K3K(\bx_i^{\top}\bz_k)^6+9K(\bx_i^{\top}\bz_k)^4(\bx_i^{\top}\bar{\bbeta}_k^*)^2\\
	&+9K(\bx_i^{\top}\bz_k)^2(\bx_i^{\top}\bar{\bbeta}_k^*)^4\Big)\sum_{k'=1}^K(\bx_i^{\top}\bar{\bbeta}_{k'})^4\Big].
	\end{split}
\end{equation*}
The main term is $(\bx_i^{\top}\bz_k)^2(\bx_i^{\top}\bar{\bbeta}_k^*)^4$ according to the order of $\bar{\bbeta}_k^*$. We bound the main term first. Note that there exists some positive large constant $C$ such that 
\begin{eqnarray*}
	\mathbb E\Big(\frac{1}{n}\sum_{i=1}^n(\bx_i^{\top}\bz_k)^2(\bx_i^{\top}\bar{\bbeta}_{k'}^*)^4(\bx_i^{\top}\bar{\bbeta}_{k'})^4\Big)\leq C\|\bz_k\|_2^2\|\bar{\bbeta}_k^*\|_2^4\|\bar{\bbeta}_{k'}\|_2^4.
\end{eqnarray*}
Together with Lemma \ref{cor:concentr_high_order} and \eqref{con:initial_input}, we have
\begin{equation*}
\begin{split}
	&\sum_{k=1}^K\sum_{k'=1}^K\Big(\frac{1}{n}\sum_{i=1}^n(\bx_i^{\top}\bz_k)^2(\bx_i^{\top}\bar{\bbeta}_{k'}^*)^4(\bx_i^{\top}\bar{\bbeta}_{k'})^4\Big)\\
	\leq& C\Big(1+\frac{(\log n)^5}{\sqrt{n}}\Big)K^2\eta_{\max}^{*\tfrac{8}{3}}(1+K^{\tfrac{1}{2}}\varepsilon_0)^4\sum_{k=1}^K\|\bz_k\|_2^2.
	\end{split}
\end{equation*}
with probability at least $1-3K^2/n$. Overall, the upper bound of $B_1$ takes the form 
\begin{equation}\label{ineqn:bound_B1}
\begin{split}
B_1\leq& K^{-2}R^{\tfrac{4}{3}}\eta_{\min}^{*-\tfrac{8}{3}}\Big[18C\Big(1+\frac{(\log n)^5}{\sqrt{n}}\Big)K^2\eta_{\max}^{*\tfrac{8}{3}}(1+K^{\tfrac{1}{2}}\varepsilon_0)^4\sum_{k=1}^K\|\bz_k\|_2^2\Big]\\
\leq& R^{4}18C\Big(1+\frac{(\log n)^5}{\sqrt{n}}\Big)(1+K^{\tfrac{1}{2}}\varepsilon_0)^4\sum_{k=1}^K\|\bz_k\|_2^2,
\end{split}
\end{equation}
with probability at least $1-3K^2/n$.

~\\
\noindent  \textbf{Bounding $B_2$.} We rewrite $B_2$ by 
\begin{eqnarray*}
	B_2 = \sum_{k=1}^K\frac{\eta_k^{*\tfrac{4}{3}}}{\phi^2}\Big(\frac{1}{n}\sum_{i=1}^n\epsilon_i^2(\bx_i^{\top}\bar{\bbeta}_k)^4\Big).
\end{eqnarray*}
For fixed $\{\epsilon_i\}_{i=1}^n$, accordingly to Lemma \ref{cor:concentr_high_order}, we have
\begin{eqnarray*}
	\Big|\sum_{i=1}^n\epsilon_i^2(\bx_i^{\top}\bar{\bbeta}_k)^4-\mathbb E\Big(\sum_{i=1}^n\epsilon_i^2(\bx_i^{\top}\bar{\bbeta}_k)^4\Big)\Big|\leq C(\log n)^2\|\bepsilon^2\|_2\|\bar{\bbeta}_k\|_2^4.
\end{eqnarray*}
Note that $\mathbb E((\bx_i^{\top}\bar{\bbeta}_k)^4) = 3\|\bar{\bbeta}_k\|_2^4$. It will reduce to
\begin{eqnarray*}
	\frac{1}{n}\sum_{i=1}^n\epsilon_i^2(\bx_i^{\top}\bar{\bbeta}_k)^4\leq \Big(\frac{3}{n}\sum_{i=1}^n\epsilon_i^2+C\frac{(\log n)^2}{n}\|\bepsilon^2\|_2\Big)\|\bar{\bbeta}_k\|_2^4.
\end{eqnarray*}
From Lemma \ref{lemma:sub_exp}, with probability at least $1-3/n$, 
\begin{eqnarray*}
	|\frac{1}{n}\sum_{i=1}^n\epsilon_i^2|\leq C_0\sigma^2, \ \frac{1}{n}\|\bepsilon^2\|_2\leq C_0 \frac{\sigma^2}{\sqrt{n}}.
\end{eqnarray*}
Combining the above two inequalities, we obtain
\begin{eqnarray}
\Big|\frac{1}{n}\sum_{i=1}^n\epsilon_i^2(\bx_i^{\top}\bar{\bbeta}_k)^4\Big|\leq 6C_0\sigma^2\|\bar{\bbeta}_k\|_2^4,
\end{eqnarray}
with probability at least $1-7/n$.
Plugging in the definition of $\phi$ and \eqref{con:initial_input}, $B_2$ is upper bounded by
\begin{equation}\label{ineqn:bound_B2}
B_2\leq 6C_0\sigma^2(1+K^{\tfrac{1}{2}}\varepsilon_0)^4\eta_{\min}^{*-\tfrac{4}{3}}R^{\tfrac{8}{3}}K^{-3},
\end{equation}
with probability at least $1-7K/n$.  	

~\\
\noindent  \textbf{Summary.} Putting the bounds \eqref{ineqn:bound_B1} and \eqref{ineqn:bound_B2} together, we have similar upper bound for thresholded effect,
\begin{equation}\label{upper_bound:threhsholding}
B\leq C_2\mu^2 R^{4}\sum_{k=1}^K\|\bz_k\|_2^2 + C_3\mu^2\eta_{\min}^{*-\tfrac{4}{3}}R^{\tfrac{8}{3}}K^{-2}\frac{\sigma^2s\log p}{n},
\end{equation}
with probability at least $1-(3K^2+7K)/n$. \hfill $\blacksquare$\\

\subsubsection{Ensemble}
From the definition of $\gamma_k$, it's not hard to see actually the cross term $C$ is equal to zero. Combining the upper bound of gradient update effect \eqref{upper_bound:gradient} and thresholding effect \eqref{upper_bound:threhsholding} together, we obtain 
\begin{equation*}
\begin{split}
&\sum_{k=1}^K\Big\|\sqrt[3]{\eta_k}\tilde{\bbeta}_k^+-\sqrt[3]{\eta_k^*}\bbeta_k^*\Big\|_2^2\\
\leq&\Big(1-64\mu K^{-2}R^{-\tfrac{8}{3}}+3\mu^2K^{-1}R^4[220+270K]^2\Big)\Big(\sum_{k=1}^K\|\bz_k\|_2^2\Big)\\
&+2C_3\mu^2R^{\tfrac{8}{3}}\eta_{\min}^{*-\tfrac{4}{3}}\frac{\sigma^2K^{-2}s\log p}{n}.
\end{split}
\end{equation*}
As long as the step size $\mu$ satisfies
\begin{equation*}
0<\mu\leq \frac{32 R^{-20/3}}{3K[220+270K]^2},
\end{equation*}
we reach the conclusion
\begin{equation}
\begin{split}
&\sum_{k=1}^K\Big\|\sqrt[3]{\eta_k}\tilde{\bbeta}_k^+-\sqrt[3]{\eta_k^*}\bbeta_k^*\Big\|_2^2\\
\leq &\Big(1-32\mu K^{-2}R^{-\tfrac{8}{3}}\Big)\sum_{k=1}^K\Big\|\sqrt[3]{\eta_k}\bbeta_k-\sqrt[3]{\eta_k^*}\bbeta_k^*\Big\|_2^2\\
&+2C_3\mu^2R^{-\tfrac{8}{3}}\eta_{\min}^{*-\tfrac{4}{3}}\frac{\sigma^2K^{-2}s\log p}{n},
\end{split}
\end{equation}
with probability at least $1-4Ks/n$.\hfill $\blacksquare$



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proof of Lemma \ref{lemma:oracle_equivalence_sym}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



Let us consider $k$-th component first. Without loss of generality, suppose $F\subset\{1,2,\ldots,Ks\}$. For $j = Ks+1, \ldots,p$,
\begin{equation}
\frac{\partial}{\partial \beta_{kj}}\cL(\bbeta_k) = \frac{2}{n}\sum_{i=1}^n\Big(\sum_{k=1}^K\eta_k(\bx_i^{\top}\bbeta_k)^3-y_i\Big)\eta_k(\bx_i^{\top}\bbeta_k)^2x_{ij},
\end{equation} 
and it's not hard to see the independence between $\{\bx_i^{\top}\bbeta_k, y_i\}$ and $x_{ij}$. Applying standard Hoeffding's inequality, we have with probability at least $1-\tfrac{1}{n^2p^2}$,
\begin{eqnarray*}
	\Big|\frac{\partial}{\partial \beta_{kj}}\cL(\bbeta_k)\Big|\leq \frac{\sqrt{4\log(np)}}{n}\sqrt{\sum_{i=1}^n(\sum_{k=1}^K\eta_k(\bx_i^{\top}\bbeta_k)^3-y_i)^2(\eta_k(\bx_i^{\top}\bbeta_k))^2}=h(\bbeta_k).
\end{eqnarray*}
Equipped with union bound, with probability at least $1-\tfrac{1}{n^2p}$,
\begin{equation*}
\max_{Ks+1\leq j\leq p} \Big|\frac{\partial}{\partial \beta_{kj}}\cL(\bbeta_k)\Big|\leq h(\bbeta_k).
\end{equation*}
Therefore, according to the definition of thresholding function $\varphi(\bx)$, we obtain the following equivalence, 
\begin{equation}\label{eqn:equivalence}
\varphi_{\frac{\mu}{\phi}h(\bbeta_k)}\Big(\bbeta_k-\frac{\mu}{\phi}\nabla_{\bbeta_k}\cL(\bbeta_k)\Big) = \varphi_{\frac{\mu}{\phi}h(\bbeta_k)}\Big(\bbeta_k-\frac{\mu}{\phi}\nabla_{\bbeta_k}\cL(\bbeta_k)_F\Big),
\end{equation}
holds for $k\in[K]$, with probability  at least $1-\tfrac{1}{n^2p}$. \eqref{eqn:equivalence} also provides that $\supp(\bbeta_k^+)\subset F$ for every $k\in[K]$, which further implies $F^+\subset F$. Now we end the proof. \hfill $\blacksquare$













%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proof of Lemma \ref{lemma:marginal_effect}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

First, we consider symmetric case. According to the definition of $\{y_i\}_{i=1}^n$ from symmetric tensor estimation model \eqref{eq:model}, we separate the random noise  $\epsilon_i$ by the following expansion,
\begin{eqnarray}
\label{eqn:y_n}
\frac{1}{n}\sum_{i=1}^n y_i^2 &=& \frac{1}{n}\sum_{i=1}^{n}\Big[\sum_{k=1}^{K}\eta_k^*(\bx_i^{\top}\bbeta_k^*)^3+\epsilon_i\Big]^2\nonumber\\
&=&\underbrace{\frac{1}{n}\sum_{i=1}^{n}(\sum_{k=1}^{K}\eta_k^*(\bx_i^{\top}\bbeta_k^*)^3)^2}_{I_1}+\underbrace{\frac{2}{n}\sum_{i=1}^{n}\epsilon_i\sum_{k=1}^{K}\eta_k^*(\bx_i^{\top}\bbeta_k^*)^3}_{I_2}+\underbrace{\frac{1}{n}\sum_{i=1}^{n}\epsilon_i^2}_{I_3}.
\end{eqnarray}

~\\
\noindent\textbf{Bounding $I_1$.} We expand $i$-th component of $I_1$ as follows
\begin{equation}
\label{eqn:marginal_1}
\begin{split}
&(\sum_{k=1}^{K}\eta_k^*(\bx_i^{\top}\bbeta_k^*)^3)^2 \\
=& \sum_{k=1}^{K}\eta_k^*(\bx_i^{\top}\bbeta_k^*)^6 + 2 \sum_{k_i< k_j}\eta_{k_i}^*\eta_{k_j}^*(\bx_i^{\top}\bbeta_{k_i}^*)^3(\bx_i^{\top}\bbeta_{k_j}^*)^3.
\end{split}
\end{equation}
As shown in Corollary \ref{cor:expectation_gaussian_vector}, the expectations of above two parts takes forms of 
\begin{eqnarray*}
	 && \mathbb E(\bx_i^{\top}\bbeta_{k_i}^*)^3(\bx_i^{\top}\bbeta_{k_j}^*)^3 = 6(\bbeta_{k_i}^{*\top}\bbeta_{k_j}^*)^3 + 9(\bbeta_{k_i}^{*\top}\bbeta_{k_j}^*)\|\bbeta_{k_i}^*\|_2^2\|\bbeta_{k_j}^*\|_2^2\\
	 &&\mathbb E(\bx_i^{\top}\bbeta_k^*)^6 = 15\|\bbeta_k^*\|_2^2.
\end{eqnarray*} 
Recall that $\|\bbeta_k^*\|_2=1$ for any $k\in[K]$ and Condition \ref{con:incoherence_sym} implies for any $k_i\neq k_j$,
$|\bbeta_{k_i}^{*\top}\bbeta_{k_j}^*|\leq \Gamma,$
where $\Gamma$ is the incoherence parameter. Thus, $\mathbb E(\bx_i^{\top}\bbeta_{k_i}^*)^3(\bx_i^{\top}\bbeta_{k_j}^*)^3$ is upper bounded by
\begin{eqnarray}\label{eqn:marginal_2}
\Big|\mathbb E(\bx_i^{\top}\bbeta_{k_i}^*)^3(\bx_i^{\top}\bbeta_{k_j}^*)^3\Big| \leq 6\Gamma^3 +9\Gamma, \ \text{for any} \ k_i\neq k_j.
\end{eqnarray}
By using the concentration result in Lemma \ref{cor:concentr_high_order}, we have with probability at least $1-1/n$
\begin{equation}
\label{eqn:marginal_3}
\begin{split}
&\Big|\frac{1}{n}\sum_{i=1}^n(\bx_i^{\top}\bbeta_k^*)^6-\mathbb E(\frac{1}{n}\sum_{i=1}^n(\bx_i^{\top}\bbeta_k^*)^6)\Big|\leq C_1\frac{(\log n)^3}{\sqrt{n}},\\
&\Big|\frac{1}{n}\sum_{i=1}^n(\bx_i^{\top}\bbeta_{k_i}^*)^3(\bx_i^{\top}\bbeta_{k_j}^*)^3 -\mathbb E(\frac{1}{n}\sum_{i=1}^n(\bx_i^{\top}\bbeta_{k_i}^*)^3(\bx_i^{\top}\bbeta_{k_j}^*)^3)\Big|\leq C_1\frac{(\log n)^3}{\sqrt{n}}.
\end{split}
\end{equation}
Putting \eqref{eqn:marginal_1},\eqref{eqn:marginal_2} and \eqref{eqn:marginal_3} together, this essentially provides an upper bound for $I_1$, namely
\begin{equation}
\label{eqn:marginal_I1}
\frac{1}{n}\sum_{i=1}^{n}(\sum_{k=1}^{K}\eta_k^*(\bx_i^{\top}\bbeta_k^*)^3)^2\leq \Big(15+6\Gamma^3+9\Gamma+2 C_1\frac{(\log n)^3}{\sqrt{n}}\Big) (\sum_{k=1}^{K}\eta_k^*)^2,
\end{equation}
with probability at least $1-K^2/n$.

~\\
\noindent\textbf{Bounding $I_2$.} Since the random noise $\{\epsilon_i\}_{i=1}^n$ is of mean zero and independent of $\{\bx_i\}$, we have
$$\mathbb E(\epsilon_i\sum_{k=1}^{K}\eta_k^*(\bx_i^{\top}\bbeta_k^*)^3) = 0.$$
By using the independence and Corollary \ref{cor:concentr_high_order}, we have
\begin{eqnarray*}
	&&\mathbb P\Big(\frac{1}{n}\sum_{i=1}^{n}\epsilon_i(\bx_i^{\top}\bbeta_k^*)^3\geq C_2\frac{(\log n)^{\tfrac{3}{2}}}{n}\sqrt{n} \sigma\Big)\\
	&&\leq \mathbb P\Big(\frac{1}{n}\sum_{i=1}^{n}\epsilon_i(\bx_i^{\top}\bbeta_k^*)^3\geq C_2\frac{(\log n)^{\tfrac{3}{2}}}{n}\sqrt{n} \sigma\Big|\|\bepsilon\|_2\leq C_0\sigma \sqrt{n}\Big) +\mathbb P\Big(\|\bepsilon\|_2\geq C_0\sqrt{n}\sigma\Big)\\
	&&\leq \frac{1}{n}+\frac{3}{n} = \frac{4}{n}.
\end{eqnarray*}
This further implies that 
\begin{eqnarray}
\label{eqn:marginal_I2}
\frac{1}{n}\sum_{i=1}^n\sum_{k=1}^{K}\eta_k^*(\bx_i^{\top}\bbeta_k^*)^3\epsilon_i\leq (\sum_{k=1}^K\eta_k^*)C_2\frac{(\log n)^{\tfrac{3}{2}}}{\sqrt{n}}\sigma,
\end{eqnarray}
with probability at least $1-4K/n$. 

~\\
\noindent\textbf{Bounding $I_3$.} As shown in Lemma \ref{lemma:sub_exp}, the random noise $\epsilon_i$ with sub-exponential tail satisfies 
\begin{eqnarray}
\label{eqn:marginal_I3}
\frac{1}{n}\sum_{i=1}^n\epsilon_i^2 \leq C_3 \sigma^2 .
\end{eqnarray}
with probability at least $1-3/n$.

Overall, putting \eqref{eqn:marginal_I1}, \eqref{eqn:marginal_I2} and \eqref{eqn:marginal_I3} together, we have with probability at least $1-(K^2+4K+3)/n$,
\begin{equation*}
\frac{\frac{1}{n}\sum_{i=1}^{n}y_i^2}{(\sum_{k=1}^K\eta_k^*)^2}
\leq 15 + 6\Gamma^3+9\Gamma+2 C_1\frac{(\log n)^3}{\sqrt{n}} + \frac{2 C_2\sigma}{(\sum_{k=1}^K\eta_k^*)}\frac{(\log n)^{\tfrac{3}{2}}}{\sqrt{n}} + \frac{C_3 \sigma^2 }{(\sum_{k=1}^K\eta_k^*)^2}.
\end{equation*}
Under Conditions \ref{con:noise} \& \ref{con:sample}, the above bound reduces to
\begin{equation*}
\frac{1}{n}\sum_{i=1}^{n}y_i^2\leq (16+6\Gamma^3+9\Gamma)(\sum_{k=1}^K\eta_k^*)^2, 
\end{equation*}
with probability at least $1-(K^2+4K+3)/n$. The proof of lower bound is similar, and hence is omitted here.

Similar results will also hold for non-symmetric tensor estimation model. Throughout the proof, the only difference is that $$\mathbb E(\bu_i^{\top}\bbeta_{1k}^*)^2(\bv_i^{\top}\bbeta_{2k}^*)^2(\bw_i^{\top}\bbeta_{3k}^*)^2=1.$$ \hfill $\blacksquare$\\


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Non-symmetric Tensor Estimation}\label{sec:non_symmetric}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Conditions and Algorithm}\label{con_alg_nonsym}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this subsection, we provide several essential conditions for Theorem \ref{thm:main_nym} and the detail algorithm for non-symmetric tensor estimation.
\begin{Condition}[(Uniqueness of CP-decomposition)]\label{con:ident_nym}
	The CP-decomposition form \eqref{eq:low_rank_nonsym} is unique in the sense that if there exists another CP-decomposition $\mT^* = \sum_{k=1}^{K'} \eta_k^{*'}\bbeta_{1k}^{*'}\circ\bbeta_{2k}^{*'}\circ\bbeta_{3k}^{*'}$, it must have $K=K'$ and be invariant up to a permutation of $\{1,\ldots, K\}$.
\end{Condition}
\begin{Condition}[(Parameter space)]\label{con:parameter_nym}
	The CP-decomposition of $\mT^* = \sum_{k=1}^K \eta_k^*\bbeta_{1k}^*\circ\bbeta_{2k}^*\circ\bbeta_{3k}^*$ satisfies
	$$\|\mT^*\|_{op}\leq C_1\eta_{\max}^*, \quad K=\cO(s), \quad \text{and}\quad R =\eta_{\max}^*/\eta_{\min}^*\leq C_2
	$$
	for some absolute constants $C_1,C_2$.
\end{Condition}
\begin{Condition}[(Parameter incoherence)]
	\label{con:incoherence_nym}
	The true tensor components are incoherent such that
	\begin{eqnarray*}
		\Gamma:=\max_{k_i\neq k_j}\Big\{|\langle\bbeta_{1k_i}^*, \bbeta_{1k_j}^*\rangle|, |\langle\bbeta_{2k_i}^*, \bbeta_{2k_j}^*\rangle|,|\langle\bbeta_{3k_i}^*, \bbeta_{3k_j}^*\rangle|\Big\}\leq C\min\{K^{-\tfrac{3}{4}}R^{-1},s^{-\tfrac{1}{2}}\}.
	\end{eqnarray*}
\end{Condition}
\begin{Condition}[(Random noise)]\label{con:noise_non}
	We assume the random noise $\{\epsilon_i\}_{i=1}^n$ follows a sub-exponential tail with parameter $\sigma$ satisfying $0<\sigma<C\sum_{k=1}^K\eta_k^*$. 
\end{Condition}

\begin{algorithm}\label{alg:overall_nonsymmetric}
	\small
	\caption{Non-symmetric tensor estimation via cubic sketchings}
	\begin{algorithmic}[1]
		\REQUIRE response $\{y_i\}_{i=1}^n$, sketching vector $\{\bu_i,\bv_i,\bw_i\}_{i=1}^n$, truncation level $d$, step size $\mu$, rank $K$, stopping error $\epsilon = 10^{-4}$.
		\STATE  \textbf{Step 1:} Calculate the moment-based tensor $\cT$ as \eqref{eq:moment_asy} and do sparse tensor decomposition on $\cT$ to get a warm-start $\{\boldsymbol{\eta}^{(0)}, \bB_1^{(0)}, \bB_2^{(0)}, \bB_3^{(0)}\}$.
		\STATE \textbf{Step 2:} Let $t=0$. \\
		\STATE \ \ \textbf{Repeat} block-wise thresholded gradient update
		\STATE \begin{itemize}
			\item Compute threshold level $\bh(\bB_k)$ as defined in Step Two.
			\item Calculated block-wise thresholded gradient descent update
			\begin{equation*}
				\begin{split}
					&\tv(\bB_1^{(t+1)}) = \varphi_{\frac{\mu\bh(\bB_1)}{\phi}}\Big(\tv(\bB_1^{(t)}) -\frac{\mu}{\phi}\nabla_{\bB_1}\cL(\bB_1^{(t)}, \bB_2^{(t)}, \bB_3^{(t)})\Big)\\
					&\tv(\bB_2^{(t+1)}) = \varphi_{\frac{\mu\bh(\bB_2)}{\phi}}\Big(\tv(\bB_2^{(t)}) -\frac{\mu}{\phi}\nabla_{\bB_2}\cL(\bB_1^{(t)}, \bB_2^{(t)}, \bB_3^{(t)})\Big)\\
					&\tv(\bB_3^{(t+1)}) = \varphi_{\frac{\mu\bh(\bB_3)}{\phi}}\Big(\tv(\bB_3^{(t)}) -\frac{\mu}{\phi}\nabla_{\bB_3}\cL(\bB_1^{(t)}, \bB_2^{(t)}, \bB_3^{(t)})\Big),
				\end{split}
			\end{equation*} 
			where $\phi=\frac{1}{n}\sum_{i=1}^ny_i^2$. The detail form of $\nabla_{\bB_1}\cL, \nabla_{\bB_2}\cL, \nabla_{\bB_3}\cL$  can refer \eqref{eqn:gradient_nonsym}
		\end{itemize}
		\STATE \ \  \textbf{Until} $\max\{\|\bB_j^{(T+1)} - \bB_j^{(T)}\|_F\}\leq \epsilon$. \\
		
		\STATE \textbf{Step 3:} Do column-wise normalization as 
		\begin{eqnarray*}
			&&\hat{\bB}_1 = \Big(\frac{\bbeta_{11}^{(T)}}{\|\bbeta_{11}^{(T)}\|_2}, \ldots, \frac{\bbeta_{1K}^{(T)}}{\|\bbeta_{1K}^{(T)}\|_2}\Big), \\
			&&\hat{\bB}_2 = \Big(\frac{\bbeta_{21}^{(T)}}{\|\bbeta_{21}^{(T)}\|_2}, \ldots, \frac{\bbeta_{2K}^{(T)}}{\|\bbeta_{2K}^{(T)}\|_2}\Big), \\
			&&\hat{\bB}_3 = \Big(\frac{\bbeta_{31}^{(T)}}{\|\bbeta_{31}^{(T)}\|_2}, \ldots, \frac{\bbeta_{3K}^{(T)}}{\|\bbeta_{3K}^{(T)}\|_2}\Big).
		\end{eqnarray*} 
		And update the weight by 
		$$\hat{\boldsymbol{\eta}} = \boldsymbol{\eta}^{(0)} * (\|\bbeta_{11}^{(T)}\|_2\|\bbeta_{21}^{(T)}\|_2\|\bbeta_{31}^{(T)}\|_2, \ldots, \|\bbeta_{1K}^{(T)}\|_2\|\bbeta_{3K}^{(T)}\|_2\|\bbeta_{3K}^{(T)}\|_2)^{\top}.
		$$ The final estimator is $\hat{\mT} = \sum_{k=1}^{K}\hat{\eta}_{k}\hat{\bbeta}_{1k}\circ \hat{\bbeta}_{2k}\circ \hat{\bbeta}_{3k}$.\\
		\RETURN non-symmetric tensor estimator $\hat{\mT}$.
	\end{algorithmic}
\end{algorithm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proof of Theorem \ref{thm:main_nym}}\label{sec:proof_asym}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The main distinguished part of the proof for non-symmetric update is Lemma \ref{lemma:onestep_update_nym}: one-step oracle estimator, which is parallel to Lemma \ref{lemma:onestep_update_sym}. For the sake of completeness, we limit our attention to rank-one case and only provide the theoretical development for one-step oracle estimator in this subsection. The generalization to general rank case follows the exact same idea in the proof of symmetric update by incorporating the incoherence condition \eqref{con:incoherence_nym}. 

For rank-one non-symmetric tensor estimation, the model \eqref{eq:model_asymmetric} reduces to
\begin{equation*}
	y_i = \langle\eta^*\bbeta_1^*\circ \bbeta_2^*\circ \bbeta_3^*, \bu_i\circ \bv_i \circ \bw_i\rangle+\epsilon_i, \ \text{for} \ i=1,\ldots,n.
\end{equation*}
Suppose $|\supp(\bbeta_1^*)|=s_1$, $|\supp(\bbeta_2^*)|=s_2$, $|\supp(\bbeta_3^*)|=s_3$ and denote $s=\max\{s_1,s_2,s_3\}$. Define $F_j^{(t)} = \supp(\bbeta_j^*)\cup\supp(\bbeta_j^{(t)})$, $F^{(t)}=\cup_{j=1}^3F_j^{(t)}$ and the oracle estimator as
\begin{equation*}
	\tilde{\bbeta}_1^{(t+1)} = \varphi_{\frac{\mu}{\phi}h(\bbeta_1^{(t)})}\Big(\bbeta_j^{(t)}-\frac{\mu}{\phi}\nabla_1\cL(\bbeta_1^{(t)}, \bbeta_2^{(t)}, \bbeta_3^{(t)})_{F^{(t)}}\Big),
\end{equation*}
where $h(\bbeta_1^{(t)})$ has the form of 
\begin{equation}\label{def:threhsold_level_nym}
\frac{\sqrt{4\log np}}{n}\sqrt{\sum_{i=1}^n\Big(\eta(\bu_i^{\top}\bbeta_1^{(t)})(\bv_i^{\top}\bbeta_2^{(t)})(\bw_i^{\top}\bbeta_3^{(t)})-y_i\Big)^2\eta^{\tfrac{2}{3}}(\bv_i^{\top}\bbeta_2^{(t)})^2(\bw_i^{\top}\bbeta_3^{(t)})^2}.
\end{equation}
The definitions of $\tilde{\bbeta}_2^{(t+1)}$ and $\tilde{\bbeta}_3^{(t+1)}$ are similar.
\begin{Lemma}
	\label{lemma:onestep_update_nym}
	Let $t\geq 0$ be an integer. Suppose Conditions \ref{con:ident_nym}-\ref{con:noise_non} hold and $\{\bbeta_j^{(t)}, \eta\}$ satisfies the following upper bound
	\begin{equation}\label{con:initial_nym}
		\max_{j=1,2,3}\|\sqrt[3]{\eta}\bbeta_j^{(t)}-\sqrt[3]{\eta^*}\bbeta_j^*\|_2\leq \sqrt[3]{\eta^*}\varepsilon_0, \ |\eta-\eta^*|\leq \varepsilon_0
	\end{equation}
	with probability at least $1-CO(1/n)$. Assume the step size $\mu$ satisfies $0<\mu<\mu_0$ for some small absolute constant $\mu_0$ and $s\leq d\leq Cs$. Then $\{\tilde{\bbeta}_j^{(t+1)}\}$ can be upper bounded as
	\begin{eqnarray*}
		&&\max_{j=1,2,3}\Big\|\sqrt[3]{\eta}\tilde{\bbeta}_j^{(t+1)}-\sqrt[3]{\eta^*}\bbeta_j^*\Big\|_2\\
		&\leq& (1-\frac{\mu}{12})\max_{j=1,2,3}\Big\|\sqrt[3]{\eta}\bbeta_j^{(t)}-\sqrt[3]{\eta^*}\bbeta_j^*\Big\|_2+\mu\frac{3\sigma}{(\sqrt[3]{\eta^*})^2}\sqrt{\frac{3s \log p}{n}},
	\end{eqnarray*}
	with probability at least $1-12s/n$.
\end{Lemma}

\emph{Proof.} We focus on $j=1$ first. To simplify the notation, we drop the superscript of iteration index $t$, and denote iteration index $t+1$ by $+$. Moreover, denote $\bar{\bbeta}_j = \sqrt[3]{\eta}\bbeta_j$, $\bar{\bbeta}_j^+=\sqrt[3]{\eta}\bbeta_j$, $\bar{\bbeta}_j^{*}=\sqrt[3]{\eta^*}\bbeta_j^*$ for $j=1,2,3$. Then, the gradient function is rewritten as
\begin{eqnarray*}
	\nabla_1\cL(\bar{\bbeta}_1,\bar{\bbeta}_2,\bar{\bbeta}_3) =\sqrt[3]{\eta} \frac{2}{n}\sum_{i=1}^n\Big((\bu_i^{\top}\bar{\bbeta}_1)(\bv_i^{\top}\bar{\bbeta}_2)(\bw_i^{\top}\bar{\bbeta}_3)\Big)(\bv_i^{\top}\bar{\bbeta}_2)(\bw_i^{\top}\bar{\bbeta}_3)\bu_i.
\end{eqnarray*}

According to the definition of thresholded function, $\tilde{\bbeta}_1^+$ can be explicitly written by
\begin{eqnarray*}
	\tilde{\bbeta}_1^+ &=& \varphi_{\frac{\mu}{\phi} h(\bar{\bbeta}_1)}\Big(\bbeta_1-\frac{\mu}{\phi}\nabla_{1}\cL(\bar{\bbeta}_1, \bar{\bbeta}_2, \bar{\bbeta}_3)_{F}\Big)\\
	&=& \bbeta_1-\frac{\mu}{\phi}\nabla_{1}\cL(\bar{\bbeta}_1, \bar{\bbeta}_2, \bar{\bbeta}_3)_{F}+\frac{\mu}{\phi} h(\bar{\bbeta}_1)\bgamma,
\end{eqnarray*}
where $\bgamma\in \mathbb R^p, \supp(\bgamma)\subset F$ and $\|\bgamma\|_{\infty}\leq 1$. Then the oracle estimation error $\|\sqrt[3]{\eta}\tilde{\bbeta}_1^+-\sqrt[3]{\eta^*}\bbeta_1^*\|_2$ can be decomposed by the gradient update effect and the thresholded effect,
\begin{equation}
	\label{eqn:main_decomposition}
	\begin{split}
	&\Big\|\sqrt[3]{\eta}\tilde{\bbeta}_1^+-\sqrt[3]{\eta^*}\bbeta_1^*\Big\|_2\\
	 = &\underbrace{\Big\|\bar{\bbeta}_1-\bar{\bbeta}_1^*-\mu\frac{\sqrt[3]{\eta}}{\phi}\nabla_{1}\cL(\bar{\bbeta}_1, \bar{\bbeta}_2, \bar{\bbeta}_3)_{F}\Big\|_2}_{\text{gradient update effect}} + \underbrace{\mu\frac{\sqrt[3]{\eta}}{\phi}\Big|h(\bar{\bbeta}_1)\Big|\sqrt{3s}}_{\text{thresholded effect}}.
	 \end{split}
\end{equation}
By using the tri-convex structure of $\cL(\bar{\bbeta}_1, \bar{\bbeta}_2, \bar{\bbeta}_3)$, we borrow the analysis tool for vanilla gradient descent \citep{Bubeck15} given sufficient good initial. Following this proof strategy, we decompose the gradient update effect in \eqref{eqn:main_decomposition} by three parts,
\begin{eqnarray*}
	\Big\|\sqrt[3]{\eta}\tilde{\bbeta}_1^+-\sqrt[3]{\eta^*}\bbeta_1^*\Big\|_2&\leq&\underbrace{\Big\|\bar{\bbeta}_1-\bar{\bbeta}_1^*-\mu \frac{\sqrt[3]{\eta}}{\phi}\nabla_{1} \tilde{\cL}(\bar{\bbeta}_1,\bar{\bbeta}_2^*,\bar{\bbeta}_3^*)_{F}\Big\|_2}_{I_1}\\
	&+&\mu \underbrace{\frac{\sqrt[3]{\eta}}{\phi}\Big\|\nabla_{1} \tilde{\cL}(\bar{\bbeta}_1,\bar{\bbeta}_2^*,\bar{\bbeta}_3^*)_{F}-\nabla_{1}\tilde{\cL}(\bar{\bbeta}_1,\bar{\bbeta}_2,\bar{\bbeta}_3)_{F}\Big\|_2}_{I_2}\\
	&+&\mu \underbrace{\frac{\sqrt[3]{\eta}}{\phi}\Big\|\nabla_{1}\tilde{\cL}(\bar{\bbeta}_1,\bar{\bbeta}_2,\bar{\bbeta}_3)_{F}-\nabla_{1}\cL(\bar{\bbeta}_1,\bar{\bbeta}_2,\bar{\bbeta}_3)_{F}\Big\|_2}_{I_3}\\
	&+&\underbrace{\mu\frac{\sqrt[3]{\eta}}{\phi}\Big|h(\bar{\bbeta}_1)\Big|\sqrt{3s}}_{I_4},
\end{eqnarray*}
where $\nabla_1\tilde{\cL}$ is the noiseless gradient as we defined in \eqref{def:noiseless_gradient}.
We will bound $I_1,I_2, I_3, I_4$ successively in the following four subsections. For simplicity, during the following proof, we drop the index subscript $F$ as we did in Section \ref{proof:one-step_sym}. And $\phi = \sum_{i=1}^ny_i^2$ approximates $\eta^{*2}$ up to constant due to Lemma \ref{lemma:marginal_effect}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Bounding $I_1$}\label{proof_gradient_effect}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this section, let us denote 
$$
\sqrt[3]{\eta}\tilde{\cL}(\bar{\bbeta}_1,\bar{\bbeta}_2^*, \bar{\bbeta}_3^*)/\phi = f(\bar{\bbeta}_1), \ \sqrt[3]{\eta}\nabla_{1}\tilde{\cL}(\bar{\bbeta}_1,\bar{\bbeta}_2^*,\bar{\bbeta}_3^*)/\phi=\nabla f(\bar{\bbeta}_1),
$$
 where $\supp(\nabla f(\bar{\bbeta}_1))=F$. When $\bbeta_2$ and $\bbeta_3$ are fixed, the update can be treated as a vanilla gradient descent update. The following proof follows three steps. The first two steps show that $f(\bar{\bbeta}_1)$ is Lipshitz differentiable and strongly convex on the constraint set $F$, and the last step utilizes the classical convex gradient analysis.

\textbf{Step One:} Verify $f(\bar{\bbeta}_1)$ is $L$-Lipschitz differentiable. For any $\bar{\bbeta}_1^{(1)}$ and $\bar{\bbeta}_1^{(2)}$ whose support belong to $F$, 
\begin{eqnarray*}
	\nabla f(\bar{\bbeta}_1^{(1)})-\nabla f(\bar{\bbeta}_1^{(2)}) = \frac{(\sqrt[3]{\eta})^2}{\phi}\frac{2}{n}\sum_{i=1}^n\Big(\bu_i^{\top}(\bar{\bbeta}_1^{(1)}-\bar{\bbeta}_1^{(2)})(\bv_i^{\top}\bar{\bbeta}_2^*)^2(\bw_i^{\top}\bar{\bbeta}_3^*)^2\Big)\bu_{i}.
\end{eqnarray*}
Then, there exist $\pi\in\mathbb S^{s-1}$ such that
\begin{eqnarray*}
	&&\Big\|\nabla f(\bar{\bbeta}_1^{(1)})-\nabla f(\bar{\bbeta}_1^{(2)})\Big\|_2 \\
	&=& \frac{(\sqrt[3]{\eta})^2}{\phi}\Big|\frac{1}{n}\sum_{i=1}^n\Big(\bu_i^{\top}(\bar{\bbeta}_1^{(1)}-\bar{\bbeta}_1^{(2)})(\bv_i^{\top}\bar{\bbeta}_2^*)^2(\bw_i^{\top}\bar{\bbeta}_3^*)^2\Big)\bu_{i}^{\top}\pi\Big|.
\end{eqnarray*}
Applying Lemma \ref{lemma:tensor_spectral} with multiplying $(\bar{\bbeta}_1^{(1)}-\bar{\bbeta}_1^{(2)}) \circ\bar{\bbeta}_2^*\circ \bar{\bbeta}_3^* $, it shows
\begin{eqnarray*}
	&&\Big|\sum_{i=1}^n\Big[(\bu_i^{\top}(\bar{\bbeta}_1^{(1)}-\bar{\bbeta}_1^{(2)})(\bu_i^{\top}\pi)(\bv_i^{\top}\bar{\bbeta}_2^*)^2(\bw_i^{\top}\bar{\bbeta}_3^*)^2)\Big]\Big|\\
	&\leq& \Big(1+\delta_{n,p,s}\Big)\Big\|\bar{\bbeta}_1^{(1)}-\bar{\bbeta}_1^{(2)}\Big\|_2\eta^{*\tfrac{4}{3}},
\end{eqnarray*}
with probability at least $1-10/n^3$, where $\delta_{n,p,s}$ is defined in \eqref{eqn:initial_stat_rate}. Under Condition \eqref{con:sample} with some constant adjustments, we obtain
\begin{eqnarray}
	\Big\|\nabla f(\bar{\bbeta}_1^{(1)})-\nabla f(\bar{\bbeta}_1^{(2)})\Big\|_2 \leq\frac{57}{16}\Big\|\bar{\bbeta}_1^{(1)}-\bar{\bbeta}_1^{(2)}\Big\|_2.
\end{eqnarray}
with probability at least $1-10/n^3$. Therefore, $f(\bar{\bbeta}_1)$ is Lipschitz differentiable with Lipschitz constant $L=\frac{57}{8}$.

\textbf{Step Two:} Verify $f(\bar{\bbeta}_1)$ is $\alpha$-strongly convex. It is equivalent to prove that $\nabla^2f(\bar{\bbeta}_1)\succeq m \mI_p$. Based on the inequality (3.3.19) in \cite{HJ88}, it shows that
\begin{equation}
	\label{minimum_eigen}
	\begin{split}
	\lambda_{\min}\big(\nabla^2(f(\bar{\bbeta}_1))\big)\geq \lambda_{\min}\big(\mathbb E(\nabla^2 f(\bar{\bbeta}_1))\big)-\lambda_{\max}\big(\nabla^2 f(\bar{\bbeta}_1)-\mathbb E(\nabla^2 f(\bar{\bbeta}_1)\big).
	\end{split}
\end{equation}
The lower bound of $\lambda_{\min}(\nabla^2(f(\bar{\bbeta}_1)))$ breaks into two parts: an lower bound for $\lambda_{\min}(\mathbb E(\nabla^2 f(\bar{\bbeta}_1)))$, and an upper bound for $\lambda_{\max}(\nabla^2 f(\bar{\bbeta}_1)-\mathbb E(\nabla^2 f(\bar{\bbeta}_1))$.
The Hessian matrix of $f(\bar{\bbeta}_1)$ is given by
\begin{eqnarray*}
	\nabla^2f(\bar{\bbeta}_1) = \frac{(\sqrt[3]{\eta})^2}{\phi}\frac{2}{n}\sum_{i=1}^n(\bv_1^{\top}\bar{\bbeta}_2^*)^2(\bw_i^{\top}\bar{\bbeta}_3^*)^2\bu_i\bu_i^{\top}.
\end{eqnarray*}
Since $\bu_i, \bv_i,\bw_i$ are independent with each other, we have $\mathbb E(\nabla^2f(\bar{\bbeta}_1)) = 2\mI$, which implies $\lambda_{\min}\big(\mathbb E(\nabla^2f(\bar{\bbeta}_1))\big)\geq2$.

 On the other hand,
\begin{eqnarray*}
	&&\lambda_{\max}\Big(\nabla^2f(\bar{\bbeta}_1)-\mathbb E(\nabla^2f(\bar{\bbeta}_1))\Big) = \Big\|\nabla^2f(\bar{\bbeta}_1)-\mathbb E(\nabla^2f(\bar{\bbeta}_1))\Big\|_2\\
	&&\leq \ba^{\top}\Big(\nabla^2f(\bar{\bbeta}_1)-\mathbb E(\nabla^2f(\bar{\bbeta}_1))\Big)\bb=\frac{2}{n}\sum_{i=1}^n (\bv_i^{\top}\bar{\bbeta}_2^*)^2(\bw_i^{\top}\bar{\bbeta}_3^*)^2(\bu_i^{\top}\ba)(\bu_i^{\top}\bb)\\
	&& - \mathbb E\Big(\sum_{i=1}^n (\bv_i^{\top}\bar{\bbeta}_2^*)^2(\bw_i^{\top}\bar{\bbeta}_3^*)^2(\bu_i^{\top}\ba)(\bu_i^{\top}\bb)\Big)\eta^{*-\tfrac{4}{3}}.
\end{eqnarray*}
where $\ba,\bb\in\mathbb S^{s-1}$. Equipped with Lemma \ref{lemma:tensor_spectral}, it yields that with probability at least $1-10/n^3$,
\begin{eqnarray*}
	\lambda_{\max}\Big(\nabla^2f(\bar{\bbeta}_1)-\mathbb E(\nabla^2f(\bar{\bbeta}_1))\Big)\leq 2\delta_{n,s,p}.
\end{eqnarray*}
 Together with the lower bound of $\lambda_{\min}(\mathbb E(\nabla^2 f(\bar{\bbeta}_1)))$, we have 
$$\lambda_{\min}(\nabla^2f(\bar{\bbeta}_1))\geq 2-2\delta_{n,p,s},
$$
Under Condition \ref{con:sample}, the minimum eigenvalue of Hessian matrix $\nabla^2f(\bar{\bbeta}_1)$ is lower bounded by $\frac{19}{10}$ with probability at least $1-10/n^3$. This guarantees that $f(\bar{\bbeta}_1)$ is strongly-convex with $\alpha= \frac{19}{10}$.

\textbf{Step Three:}
Combining the Lipschitz condition, strongly-convexity and Lemma 3.11 in \cite{Bubeck15}, it shows that
\begin{eqnarray*}
	&&\big(\nabla f(\bar{\bbeta}_1)-\nabla f(\bar{\bbeta}_1^*)^{\top}\big)\big(\bar{\bbeta}_1-\bar{\bbeta}^*\big)\\
	&\geq& \frac{\alpha L}{\alpha+L}\Big\|\bar{\bbeta}_1-\bar{\bbeta}_1^*\Big\|_2^2+\frac{1}{\alpha+L}\Big\|\nabla f(\bar{\bbeta}_1)-\nabla f(\bar{\bbeta}_1^*)\Big\|_2^2.
\end{eqnarray*}
Since the gradient vanishes at the optimal point, the above inequality times $2\mu$ simplifies to
\begin{equation}
	\label{inequality_convex}
	\begin{split}
	-2\mu \nabla f(\bar{\bbeta}_1)^{\top} (\bar{\bbeta}_1-\bar{\bbeta}_1^*)
	\leq -\frac{2\mu \alpha L}{\alpha+L}\Big\|\bar{\bbeta}_1-\bar{\bbeta}_1^*\Big\|_2^2-\frac{2\mu}{\alpha+L}\Big\|\nabla f(\bar{\bbeta}_1)\Big\|_2^2.
	\end{split}
\end{equation}
Now it's sufficient to bound $\|\bar{\bbeta}_1-\bar{\bbeta}_1^*-\mu\nabla f(\bar{\bbeta}_1)\|_2$ as follows
\begin{eqnarray*}
	&&\Big\|\bar{\bbeta}_1-\bar{\bbeta}_1^*-\mu\nabla f(\bar{\bbeta}_1)\Big\|_2^2\\
	 &=& \Big\|\bar{\bbeta}_1^{t}-\bar{\bbeta}_1^*\Big\|_2^2 + \mu^2\Big\|\nabla f(\bar{\bbeta}_1)\Big\|_2^2-2\mu\nabla f(\bar{\bbeta}_1)^{\top}(\bar{\bbeta}_1-\bar{\bbeta}^*)\\
	&\leq& \Big(1-2\mu \frac{\alpha L}{\alpha + L}\Big)\Big\|\bar{\bbeta}_1-\bar{\bbeta}_1^*\Big\|_2^2+\mu\big(\mu-\frac{2}{\alpha+L}\big)\Big\|\nabla f(\bar{\bbeta}_1)\Big\|_2^2.
\end{eqnarray*}
where $L,\alpha$ are Lipschitz constant and strongly convexity parameter, respectively. If $\mu<\frac{80}{361}$, the last term can be neglected and we obtain the desired upper bound,
\begin{equation}\label{bound:I1_nym}
	\Big\|\bar{\bbeta}_1-\bar{\bbeta}_1^*-\mu\frac{\sqrt[3]{\eta}}{\phi}\nabla_{1} \tilde{\cL}\big(\bar{\bbeta}_1, \bar{\bbeta}_2^*, \bar{\bbeta}_3^*\big)\Big\|_2 \leq \Big(1-3\mu\Big)\Big\|\bar{\bbeta}_1-\bar{\bbeta}_1^*\Big\|_2,
\end{equation}
with probability $1-20/n^3$. This ends the proof. \hfill $\blacksquare$\\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Bounding $I_2$}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


For simplicity, we write $\bz_1 = \bar{\bbeta}_1-\bar{\bbeta}_1^*$, $\bz_2 = \bar{\bbeta}_2 - \bar{\bbeta}_2^*$, $\bz_3 = \bar{\bbeta}_3 - \bar{\bbeta}_2^*$. By the definition of noiseless gradient, it suffices to decompose $I_2$ by
\begin{eqnarray*}
	&&\eta^{-\tfrac{1}{3}}\Big\|\nabla_{1}\tilde{\cL}(\bar{\bbeta}_1, \bar{\bbeta}_2^*, \bar{\bbeta}_3^*) - \nabla_{1}\tilde{\cL}(\bar{\bbeta}_1, \bar{\bbeta}_2, \bar{\bbeta}_3)\Big\|_2\\
	&\leq& \Big\|\frac{1}{n}\sum_{i=1}^n(\bu_i^{\top}\bar{\bbeta}_1)(\bv_i^{\top}\bar{\bbeta}_2)(\bv_i^{\top}\bz_2)(\bw_i^{\top}\bar{\bbeta}_3)(\bw_i^{\top}\bz_3)\bu_i\Big\|_2\\
	&&+\Big\|\frac{1}{n}\sum_{i=1}^n(\bu_i^{\top}\bar{\bbeta}_1)(\bv_i^{\top}\bar{\bbeta}_2)(\bv_i^{\top}\bz_2)(\bw_i^{\top}\bar{\bbeta}_3)(\bw_i^{\top}\bar{\bbeta}_3^*)\bu_i\Big\|_2\nonumber\\
	&&+\Big\|\frac{1}{n}\sum_{i=1}^n(\bu_i^{\top}\bar{\bbeta}_1)(\bv_i^{\top}\bar{\bbeta}_2^*)(\bv_i^{\top}\bar{\bbeta}_2)(\bw_i^{\top}\bar{\bbeta}_3)(\bw_i^{\top}\bz_3)\bu_i\Big\|_2\\
	&&+\Big\|\frac{1}{n}\sum_{i=1}^n(\bu_i^{\top}\bz_1)(\bv_i^{\top}\bar{\bbeta}_2^*)(\bv_i^{\top}\bz_2)(\bw_i^{\top}\bar{\bbeta}_3^*)(\bw_i^{\top}\bz_3)\bu_i\Big\|_2\nonumber\\
	&& +\Big\|\frac{1}{n}\sum_{i=1}^n(\bu_i^{\top}\bz_1)(\bv_i^{\top}\bar{\bbeta}_2^*)(\bv_i^{\top}\bz_2)(\bw_i^{\top}\bar{\bbeta}_3^*)^2\bu_i\Big\|_2\\
	&&+\Big\|\frac{1}{n}\sum_{i=1}^n(\bu_i^{\top}\bz_1)(\bv_i^{\top}\bar{\bbeta}_2^*)^2(\bw_i^{\top}\bar{\bbeta}_3^*)(\bw_i^{\top}\bz_3)\bu_i\Big\|_2.\nonumber
\end{eqnarray*}
Repeatedly using Lemma \ref{lemma:tensor_spectral}, we obtain
\begin{equation*}
\begin{split}
	&\eta^{-\tfrac{1}{3}}\Big\|\nabla_{1}\tilde{\cL}(\bar{\bbeta}_1, \bar{\bbeta}_2^*, \bar{\bbeta}_3^*) - \nabla_{1}\tilde{\cL}(\bar{\bbeta}_1, \bar{\bbeta}_2, \bar{\bbeta}_3)\Big\|_2\\
	&\leq \Big(1+\delta_{n,p,s}\Big)\Big[(1+\varepsilon_0)^3\varepsilon_0+(1+\varepsilon_0)^3+(1+\varepsilon_0)^3+\varepsilon_0^2+2\varepsilon_0\Big]\eta^{*\tfrac{4}{3}}\max_j\|\bz_j\|_2\\
	&\leq \frac{5}{2}\Big(1+\delta_{n,p,s}\Big)\eta^{*\tfrac{4}{3}}\max_j\|\bz_j\|_2,
	\end{split}
\end{equation*}
for sufficiently small $\varepsilon_0$ with probability at least $1-60/n^3$. Under Condition \ref{con:sample}, it suffices to get 
\begin{equation}\label{bound:I2_nym}
	\frac{\sqrt[3]{\eta}}{\phi}\Big\|\nabla_{1}\tilde{\cL}(\bar{\bbeta}_1, \bar{\bbeta}_2, \bar{\bbeta}_3) - \nabla_{1}\tilde{\cL}(\bar{\bbeta}_1, \bar{\bbeta}_2^*, \bar{\bbeta}_3^*)\Big\|_2\leq \frac{8}{3}\max_{j=1,2,3}\Big\|\bar{\bbeta}_j-\bar{\bbeta}_j^*\Big\|_2,
\end{equation}
with probability at least $1-6/n$. \hfill $\blacksquare$\\


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Bounding $I_3$}\label{proof_statistical_error}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


$I_3$ quantifies the statistical error. By the definition of noiseless gradient and noisy gradient, we have
\begin{eqnarray*}
	&&\frac{\sqrt[3]{\eta}}{\phi}\Big\|\nabla_{1}\tilde{\cL}(\bar{\bbeta}_1,\bar{\bbeta}_2,\bar{\bbeta}_3)-\nabla_{1}\cL(\bar{\bbeta}_1,\bar{\bbeta}_2,\bar{\bbeta}_3)\Big\|_2\\	&=&\frac{(\sqrt[3]{\eta})^2}{\phi}\Big\|\frac{2}{n}\sum_{i=1}^n\epsilon_i(\bv_i^{\top}\bar{\bbeta}_2)(\bw_i^{\top}\bar{\bbeta}_3)\bu_i\Big\|_2.
	%&=& \Big|\frac{\eta^*-\eta}{\eta}\Big|\cdot\underbrace{\Big\|\frac{2}{n}\sum_{i=1}^n(\bu_i^{\top}\bar{\bbeta}_1^*)(\bv_i^{\top}\bar{\bbeta}_2^*)(\bw_i^{\top}\bar{\bbeta}_3^*)(\bv_i^{\top}\bar{\bbeta}_2)(\bw_i^{\top}\bar{\bbeta}_3)\bu_i\Big\|_2}_{I_1}+\frac{1}{\eta}\underbrace{\Big\|\frac{2}{n}\sum_{i=1}^n\epsilon_i(\bv_i^{\top}\bar{\bbeta}_2)(\bw_i^{\top}\bar{\bbeta}_3) \bu_{i}\Big\|_2}_{I_2}.
\end{eqnarray*}

The proof of this part essentially coincides with the proof for symmetric tensor estimation.  Combining Lemmas \ref{cor:concentr_high_order} and \ref{lemma:sub_exp}, we have
\begin{eqnarray*}
	\Big|\frac{2}{n}\sum_{i=1}^n\epsilon_i(\bv_i^{\top}\bar{\bbeta}_2)(\bw_i^{\top}\bar{\bbeta}_3)u_{ij}\Big|\leq C(1+\varepsilon_0)^2\eta^{*\tfrac{2}{3}}\sigma\frac{(\log n)^{\tfrac{3}{2}}}{\sqrt{n}},
\end{eqnarray*}
with probability at least $1-4/n$. Applying union bound over $3s$ coordinates, it suffices to get
\begin{eqnarray*}
	\mathbb P\Big(\max_{j\in[3s]}\Big|\frac{1}{n}\sum_{i=1}^n\epsilon_i(\bv_i^{\top}\bar{\bbeta}_2)(\bw_i^{\top}\bar{\bbeta}_3)u_{ij}\Big|\geq C(1+\varepsilon_0)^2\eta^{*-\tfrac{2}{3}}\sigma\frac{(\log n)^{\tfrac{3}{2}}}{\sqrt{n}}\Big)\leq \frac{12s}{n}.
\end{eqnarray*}
Therefore, we reach
\begin{equation}\label{bound:I3_nym}
	\frac{\sqrt[3]{\eta}}{\phi}\Big\|\nabla_{1}\tilde{\cL}(\bar{\bbeta}_1,\bar{\bbeta}_2,\bar{\bbeta}_3)-\nabla_{1}\cL(\bar{\bbeta}_1,\bar{\bbeta}_2,\bar{\bbeta}_3)\Big\|_2 \leq 2C\eta^{*-\tfrac{2}{3}}\sigma\sqrt{\frac{3s(\log n)^{3}}{n}},
\end{equation}
with probability at least $1-12s/n$. \hfill $\blacksquare$\\


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Bounding $I_4$}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


According to the definition of thresholding level $h(\bbeta_1)$ in \eqref{def:threhsold_level_nym}, we can bound the square as follows,
\begin{eqnarray*}
	&&\frac{(\sqrt[3]{\eta})^2}{\phi^2}h^2(\bar{\bbeta}_1)= \frac{(\sqrt[3]{\eta})^4}{\phi^2}\frac{4 \log np}{n^2}\sum_{i=1}^n\Big((\bu_i^{\top}\bar{\bbeta}_1)(\bv_i^{\top}\bar{\bbeta}_2)(\bw_i^{\top}\bar{\bbeta}_3)\\
	&&-(\bu_i^{\top}\bar{\bbeta}_1^*)(\bv_i^{\top}\bar{\bbeta}_2^*)(\bw_i^{\top}\bar{\bbeta}_3^*)-\epsilon_i\Big)^2(\bv_i^{\top}\bar{\bbeta}_2)^2(\bw_i^{\top}\bar{\bbeta}_3)^2
\end{eqnarray*}
Based on the basic inequality $(a+b)^2\leq 2(a^2+b^2)$, we have
\begin{eqnarray*}
	&&\Big((\bu_i^{\top}\bar{\bbeta}_1)(\bv_i^{\top}\bar{\bbeta}_2)(\bw_i^{\top}\bar{\bbeta}_3)-(\bu_i^{\top}\bar{\bbeta}_1^*)(\bv_i^{\top}\bar{\bbeta}_2^*)(\bw_i^{\top}\bar{\bbeta}_3^*)-\epsilon_i\Big)^2\\
	&\leq& 2\Big((\bu_i^{\top}\bar{\bbeta}_1)(\bv_i^{\top}\bar{\bbeta}_2)(\bw_i^{\top}\bar{\bbeta}_3)-(\bu_i^{\top}\bar{\bbeta}_1^*)(\bv_i^{\top}\bar{\bbeta}_2^*)(\bw_i^{\top}\bar{\bbeta}_3^*)\Big)^2+2\epsilon_i^2.
\end{eqnarray*}
Denote $I_1$ and $I_2$ corresponding to optimization error and statistical error,
\begin{eqnarray*}
I_1 &=& \frac{(\sqrt[3]{\eta})^4}{\phi^2}\frac{4 \log np}{n^2}\sum_{i=1}^{n}\Big((\bu_i^{\top}\bar{\bbeta}_1)(\bv_i^{\top}\bar{\bbeta}_2)(\bw_i^{\top}\bar{\bbeta}_3)\\
	&&-(\bu_i^{\top}\bar{\bbeta}_1^*)(\bv_i^{\top}\bar{\bbeta}_2^*)(\bw_i^{\top}\bar{\bbeta}_3^*)\Big)^2(\bv_i^{\top}\bar{\bbeta}_2)^2(\bw_i^{\top}\bar{\bbeta}_3)^2\\
	I_2 &=& \frac{(\sqrt[3]{\eta})^4}{\phi^2}\frac{4 \log np}{n^2}\sum_{i=1}^{n}\epsilon_i^2(\bv_i^{\top}\bar{\bbeta}_2)^2(\bw_i^{\top}\bar{\bbeta}_3)^2.
\end{eqnarray*}
Next, $I_1$ is decomposed by some high-order polynomials as follows
\begin{equation}
	\label{eqn:thresholded_I1}
	\begin{split}
	I_1 =& \frac{(\sqrt[3]{\eta})^4}{\phi^2}\frac{4 \log np}{n^2}\Big(\sum_{i=1}^n(\bu_i^{\top}\bz_1)^2(\bv_i^{\top}\bz_2)^2(\bw_i^{\top}\bz_3)^2(\bv_i^{\top}\bar{\bbeta}_2)^2(\bw_i^{\top}\bar{\bbeta}_3)^2\\
	&+\sum_{i=1}^n(\bu_i^{\top}\bz_1)^2(\bv_i^{\top}\bz_2)^2(\bw_i^{\top}\bar{\bbeta}_3^*)^2(\bv_i^{\top}\bar{\bbeta}_2)^2(\bw_i^{\top}\bar{\bbeta}_3)^2\\
	&+\sum_{i=1}^n(\bu_i^{\top}\bz_1)^2(\bv_i^{\top}\bar{\bbeta}_2^*)^2(\bw_i^{\top}\bz_3)^2(\bv_i^{\top}\bar{\bbeta}_2)^2(\bw_i^{\top}\bar{\bbeta}_3)^2\\
	&+\sum_{i=1}^n(\bu_i^{\top}\bz_1)^2(\bv_i^{\top}\bar{\bbeta}_2^*)^2(\bw_i^{\top}\bar{\bbeta}_3^*)^2(\bv_i^{\top}\bar{\bbeta}_2)^2(\bw_i^{\top}\bar{\bbeta}_3)^2\\
	&+\sum_{i=1}^n(\bu_i^{\top}\bar{\bbeta}_1^*)^2(\bv_i^{\top}\bar{\bbeta}_2^*)^2(\bw_i^{\top}\bz_3)^2(\bv_i^{\top}\bar{\bbeta}_2)^2(\bw_i^{\top}\bar{\bbeta}_3)^2\\
	&+\sum_{i=1}^n(\bu_i^{\top}\bar{\bbeta}_1^*)^2(\bv_i^{\top}\bz_2)^2(\bw_i^{\top}\bar{\bbeta}_3^*)^2(\bv_i^{\top}\bar{\bbeta}_2)^2(\bw_i^{\top}\bar{\bbeta}_3)^2\\
	&+\sum_{i=1}^n(\bu_i^{\top}\bar{\bbeta}_1^*)^2(\bv_i^{\top}\bz_2)^2(\bw_i^{\top}\bz_3)^2(\bv_i^{\top}\bar{\bbeta}_2)^2(\bw_i^{\top}\bar{\bbeta}_3)^2\Big).
	\end{split}
\end{equation}
Each term contains the product of Gaussian random vectors form up to power ten. For the first term, by using Lemma \ref{cor:concentr_high_order},
\begin{eqnarray*}
	&&\frac{1}{n}\sum_{i=1}^n(\bu_i^{\top}\bz_1)^2(\bv_i^{\top}\bz_2)^2(\bw_i^{\top}\bz_3)^2(\bv_i^{\top}\bar{\bbeta}_2)^2(\bw_i^{\top}\bar{\bbeta}_3)^2\\
	&\leq& (1+\varepsilon_0)^4\varepsilon_0^4\Big(1+C\frac{(\log n)^5}{\sqrt{n}}\Big)\eta^{*\tfrac{8}{3}}\max_{j=1,2,3}\|\bz_j\|_2^2,
\end{eqnarray*}
with probability at least $1-1/n$. Similar bounds holds for other terms. As long as $n\geq C\log^{10} n$, we have with probability at least $1-7/n$, 
\begin{equation}
	\label{ineqn:bound_I1}
	I_1\leq \frac{7 \log p}{n}\max_{j=1,2,3}\Big\|\bar{\bbeta}_j-\bar{\bbeta}_j^*\Big\|_2^2.
\end{equation}


Now we turn to bound $I_2$. For fixed $\{\epsilon_i\}$, we have,
\begin{eqnarray*}
	&&\Big|\sum_{i=1}^n\epsilon_i^2(\bv_i^{\top}\bar{\bbeta}_2)^2(\bw_i^{\top}\bar{\bbeta}_3)^2- \sum_{i=1}^n\epsilon_i^2\|\bar{\bbeta}_2\|_2^2\|\bar{\bbeta}_3\|_2^2\Big|\\
	&\leq& C(\log n)^2\|\bepsilon^2\|_2\|\bar{\bbeta}_2\|_2^2\|\bar{\bbeta}_3\|_2^2,
\end{eqnarray*}
with probability at least $1-n^{-1}$. Combining with Lemma \ref{lemma:sub_exp},
\begin{equation}\label{ineqn:bound_I2}
	I_2\leq 4\sigma^2\eta^{*\tfrac{4}{3}}\frac{\log p}{n}.
\end{equation}
Putting \eqref{ineqn:bound_I1} and \eqref{ineqn:bound_I2} together, the thresholded effect can be bound by
\begin{equation}\label{bound:I3_nym}
	\frac{\sqrt[3]{\eta}}{\phi}|h(\bbeta_1)|\leq\sqrt{\frac{7 \log np}{n}}\max_{j=1,2,3}\Big\|\bar{\bbeta}_j-\bar{\bbeta}_j^*\Big\|_2+\frac{2\sigma}{(\sqrt[3]{\eta^*})^2}\sqrt{\frac{ \log np}{n}},
\end{equation}
with probability at least $1-8/n$, provided $n\gtrsim(\log n)^{10}$. \hfill $\blacksquare$\\



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Summary}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Putting the upper bounds \eqref{bound:I1_nym}, \eqref{bound:I2_nym} and \eqref{bound:I3_nym} together, we obtain that if step size $\mu$ satisfies $0<\mu<\mu_0$ for some small $\mu_0$,
\begin{eqnarray*}
	\Big\|\sqrt[3]{\eta}\tilde{\bbeta}_1^+-\sqrt[3]{\eta^*}\bbeta_1^*\Big\|_2\leq (1-\frac{\mu}{12})\max_{j=1,2,3}\Big\|\bar{\bbeta}_j-\bar{\bbeta}_j^*\Big\|_2+\mu\frac{3\sigma}{(\sqrt[3]{\eta^*})^2}\sqrt{\frac{3s \log p}{n}},
\end{eqnarray*}
with probability at least $1-12s/n$. This finishes our proof. \hfill $\blacksquare$\\





\begin{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{More Notations}\label{subsec:add_notation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textbf{Tensor multiplications:} For a third-order tensor $\cX\in\mathbb R^{p_1\times p_2\times p_3}$, the mode-one product with a matrix $\bU\in \mathbb R^{d\times p_1}$ is defined as $\cX\times_1 \bU\in \mathbb R^{d\times p_{2}\times p_3}$. More specifically, each entry is written as
\begin{eqnarray*}
	(\cX \times_1 \bU)_{j i_2i_3} = \sum_{i_1=1}^{p_1}x_{i_1i_2i_3}u_{ji_1}.
\end{eqnarray*}
The mode-two and mode-three product $\times_2,\times_3$ can be defined similarly. In particular, the successive tensor multiplication with vectors $\bu\in\mathbb R^{p_2}$, $\bv\in\mathbb R^{p_3}$ is denoted by
$$
\cX\times_2 \bu \times_3\bv = \sum_{j\in[p_2], l\in[p_3]}u_j v_l \cX_{[:,j,l]}\in \mathbb R^{p_1}.
$$
For two tensors $\cX\in \mR^{p_1\times p_2\times p_3}$ and $\cY\in \mR^{p_1\times p_2\times p_3}$ with the same size, we denote the \emph{tensor inner product} by
\begin{eqnarray}
\label{def:tensor_inner}
\langle\cX,\cY \rangle = \sum_{i,j,k} \cX_{ijk}\cY_{ijk},
\end{eqnarray}
which is the sum of the products of their entries. 

%\textbf{Derivate of tensor-valued function:}
\end{comment}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Matrix Form Gradient and Stochastic Gradient descent}\label{supp_sec:sgd}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Matrix Formulation of Gradient}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this section, we provide detail derivations for \eqref{eqn:symmetric_gradient} and \eqref{eqn:gradient_nonsym}.
\begin{lemma}
	\label{lemma:gradient_equivalence_sym}
	Let $\boldsymbol{\eta} = (\eta_1,\ldots,\eta_K)\in \mathbb R^{K\times 1}, \bX = (\bx_1,\ldots, \bx_n)\in \mathbb R^{p\times n}$ and $\bB = (\bbeta_1, \ldots, \bbeta_K)\in \mathbb R^{p\times K}$. The gradient of symmetric tensor estimation empirical risk function \eqref{eqn:risk_function_sym} can be written in a matrix form as follows 
	\begin{eqnarray*}
		\nabla_{\bB} \cL(\bB, \boldsymbol{\eta}) = \frac{6}{n}[((\bB^{\top}\bX)^{\top})^3\boldsymbol{\eta} - \by]^{\top}[(((\bB^{\top}\bX)^{\top})^2\odot\boldsymbol{\eta}^{\top})^{\top} \odot \bX]^{\top}.
	\end{eqnarray*}
\end{lemma}

\emph{Proof.} First let's have a look at the gradient for $k$-th component,
\begin{eqnarray*}
	\nabla \cL_k(\bbeta_k) = \frac{6}{n}(\sum_{k=1}^K\eta_k(\bx_i^{\top}\bbeta_k)^3-y_i)\eta_k(\bx_i^{\top}\bbeta_k)\bx_i\in \mathbb R^{p\times 1}, \ \ \text{for} \ k=1,\ldots, K.
\end{eqnarray*}
Correspondingly, each part can be written as a matrix form,
\begin{eqnarray*}
	&&((\underbrace{\bB^{\top}\bX}_{K\times n})^{\top})^3\boldsymbol{\eta} - \by\in\mathbb R^{n\times 1}\\
	&&(((\bB^{\top}\bX)^{\top})^2\odot\boldsymbol{\eta}^{\top})^{\top} \odot \bX \in \mathbb R^{pK\times n}.
\end{eqnarray*}
This implies that $[((\bB^{\top}\bX)^{\top})^3\eta - \by]^{\top}[(((\bB^{\top}\bX)^{\top})^2\odot\eta^{\top})^{\top} \odot \bX]^{\top}\in \mathbb R^{1\times pK}$. Note that $\nabla_{\bB} \cL(\bB, \boldsymbol{\eta}) = (\nabla \cL_1(\bbeta_1)^{\top}, \ldots, \nabla \cL_K(\bbeta_K)^{\top})\in \mathbb R^{1\times pK}$. The conclusion can be easily derived. \hfill $\blacksquare$\\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{Lemma}
	\label{lemma:gradient_equivalence_aym}
	Let $\boldsymbol{\eta} = (\eta_1,\ldots,\eta_K)\in \mathbb R^{K\times 1}, \bU = (\bu_1,\ldots, \bu_n)\in \mathbb R^{p_1\times n}, \bV = (\bv_1,\ldots, \bv_n)\in \mathbb R^{p_2\times n}, \bW = (\bw_1,\ldots, \bw_n)\in \mathbb R^{p_3\times n}$ and $\bB_1 = (\bbeta_{11}, \ldots, \bbeta_{1K})\in \mathbb R^{p_1\times K}, \bB_2 = (\bbeta_{21}, \ldots, \bbeta_{2K})\in \mathbb R^{p_2\times K}, \bB_3 = (\bbeta_{31}, \ldots, \bbeta_{3K})\in \mathbb R^{p_3\times K}$. The gradient of non-symmetric tensor estimation empirical risk function \eqref{def:risk_function_nym} can be written in a matrix form as follows 
	\begin{eqnarray*}
		\nabla_{\bB_1}\cL(\bB_1, \bB_2, \bB_3, \boldsymbol{\eta})  = \bD^{\top}(\bC_1^{\top}\odot\bU)^{\top},
	\end{eqnarray*}
	where $\bD = (\bB_1^{\top}\bU)^{\top}*(\bB_2^{\top}\bV)^{\top}*(\bB_3^{\top}\bW)^{\top}\boldsymbol{\eta} - \by$ and $\bC_1 = (\bB_2^{\top}\bV)^{\top}*(\bB_3^{\top}\bW)^{\top}\odot\boldsymbol{\eta}^{\top}$.
\end{Lemma}

\emph{Proof.} Recall that $\{*,\odot\}$ represent Hadamard product and Khatri-Rao product respectively. Then the dimensionality of $\bD, \bC_1, \bC_1\odot \bU$ can be calculated as follows
\begin{eqnarray*}
	&&\bD=\underbrace{(\bB_1^{\top}\bU)^{\top}}_{n\times K}*\underbrace{(\bB_2^{\top}\bV)^{\top}}_{n\times K}*\underbrace{(\bB_3^{\top}\bW)^{\top}}_{n\times K}\boldsymbol{\eta}-\by\in \mathbb R^{n\times 1},\\
	&&\bC_1 = (\bB_2^{\top}\bV)^{\top}*(\bB_3^{\top}\bW)^{\top}\odot\boldsymbol{\eta}^{\top}\in \mathbb R^{n\times K}, \bC_1^{\top}\odot \bU\in\mathbb R^{Kp_1\times n}.
\end{eqnarray*}
Therefore, $$\nabla_{\bB_1}\cL(\bB_1, \bB_2, \bB_3, \boldsymbol{\eta})  = \bD^{\top}(\bC_1^{\top}\odot\bU)^{\top} = (\nabla_1\cL(\bbeta_1)^{\top}, \ldots, \nabla_K\cL(\bbeta_K)^{\top}).$$\hfill $\blacksquare$\\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Stochastic Gradient descent}\label{subsec:stochas}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Stochastic thresholded gradient descent is a stochastic approximation of the gradient descent optimization method. Note that the empirical risk function (\ref{eqn:risk_function_sym}) that can be written as a sum of differentiable functions. Followed by \eqref{eqn:symmetric_gradient},  the gradient of (\ref{eqn:risk_function_sym}) evaluated at $i$-th sketching $\{y_i, \bx_i\}$ can be written as
\begin{eqnarray*}
	\nabla_{\bB}\cL_i(\bB, \boldsymbol{\eta})=[((\bB^{\top}\bx_i)^{\top})^3\boldsymbol{\eta} - y_i][(((\bB^{\top}\bx_i)^{\top})^2\odot \boldsymbol{\eta}^{\top})^{\top}\odot \bx_i]^{\top}\in \mathbb R^{1\times pK},
\end{eqnarray*}
Thus, the overall gradient $\nabla_{\bB}\cL_i(\bB, \boldsymbol{\eta})$ defined in \eqref{eqn:symmetric_gradient} can be expressed as a summand of $\nabla_{\bB}\cL_i(\bB, \boldsymbol{\eta})$,
\begin{eqnarray*}
	\nabla_{\bB}\cL_i(\bB, \boldsymbol{\eta})=\frac{1}{n}\sum_{i=1}^n \nabla_{\bB}\cL_i(\bB, \boldsymbol{\eta}).
\end{eqnarray*}
The thresholded step remains the same as Step 3 in Algorithm\ref{alg:overall_symmetric}. Then the symmetric update of stochastic thresholded gradient descent within one iteration is summarized by
\begin{eqnarray*}
	\tv(\bB^{(t+1)}) = \varphi_{\frac{\mu_{SGD}}{\phi}\bh(\bB^{(t)})}\Big(\tv(\bB^{(t)}) -\frac{\mu_{SGD}}{\phi}\nabla_{\bB}\cL_i(\bB^{(t)})\Big).
\end{eqnarray*}

















\begin{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Proof of Proposition \ref{thm:initial}} \label{proof:prop_initial}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Since $|\eta_k-\eta_k^*|\leq \varepsilon_0$, we have $\eta_k^*-\varepsilon_0\leq \eta_k\leq \eta_k^* +\varepsilon_0$. Divided by $\eta_k^*$, we have
\begin{eqnarray*}
1-\frac{\varepsilon_0}{\eta_k^*}\leq \frac{\eta_k}{\eta_k^*}\leq 1+\frac{\varepsilon_0}{\eta_k^*}
\end{eqnarray*}
with high probability. On the other hand, we have
\begin{eqnarray*}
\Big\|\sqrt[3]{\eta_k}\bbeta_k-\sqrt[3]{\eta_k^*}\bbeta_k^*\Big\|_2 &=& \Big\|\sqrt[3]{\eta_k}\bbeta_k-\sqrt[3]{\eta_k}\bbeta_k^*+\sqrt[3]{\eta_k}\bbeta_k^* - \sqrt[3]{\eta_k^*}\bbeta_k^*\Big\|_2\\
&\leq& \|\bbeta_k - \bbeta_k^*\|_2\sqrt[3]{\eta_k} + |\sqrt[3]{\eta_k}-\sqrt[3]{\eta_k^*}|\sqrt[3]{\eta_k^*}\\
&\leq& \varepsilon_0(1+\sqrt{1+\frac{\varepsilon_0}{\eta_k^*}})\sqrt[3]{\eta_k^*},
\end{eqnarray*}
with hihg probability. This ends the proof. \hfill $\blacksquare$\\

\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Technical Lemmas}\label{sec:tech_lemma}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{Lemma}
	\label{lemma:tensor_expectation}
	Suppose $\bx\in\mathbb R^p$ is a standard Gaussian random vector. For any non-random vector $\ba, \bb, \bc\in\mathbb R^p$, we have the following tensor expectation calculation,
	\begin{equation}
	\label{eqn:tensor_expectation}
	\begin{split}
	&\mathbb E\Big((\ba^{\top}\bx)(\bb^{\top}\bx)(\bc^{\top}\bx)\bx \circ\bx \circ \bx\Big)\\
	&= \Big(\ba\circ \bb \circ \bc + \ba\circ \bc \circ \bb + \bb \circ \ba\circ\bc+\bb\circ \bc \circ\ba+\bc\circ\bb\circ\ba+\bc\circ\ba\circ\bb\Big)\\
	&+3\sum_{m=1}^{p}\Big(\ba \circ \be_m\circ \be_m(\bb^{\top}\bc)+\be_m\circ\bb\circ\be_m(\ba^{\top}\bc)+\be_m\circ\be_m\circ \bc(\ba^{\top}\bb)\Big),
	\end{split}
	\end{equation}
	where $\be_m$ is a canonical vector in $\mathbb R^p$. 
\end{Lemma}
\emph{Proof.} Recall that for a standard Gaussian random variable $x$, its odd moments are zero and even moments are $\mathbb E(x^6) = 15, \mathbb E(x^4) = 4$. Expanding the LHS of \eqref{eqn:tensor_expectation} and comparing LHS and RHS, we will reach the conclusion. Details are omitted here. \hfill $\blacksquare$\\

\begin{Lemma}
	\label{lemma:tensor_expectation_asy}
	Suppose $\bu\in\mathbb R^{p_1}, \bv\in\mathbb R^{p_2}, \bw\in\mathbb R^{p_3} $ are independent standard Gaussian random vectors. For any non-random vector $\ba\in\mathbb R^{p_1}, \bb\in\mathbb R^{p_2}, \bc\in\mathbb R^{p_3}$, we have the following tensor expectation calculation
	\begin{equation}
		\label{eqn:tensor_expectation_asy}
		\begin{split}
			&\mathbb E\Big((\ba^{\top}\bu)(\bb^{\top}\bv)(\bc^{\top}\bw)\bu \circ\bv \circ \bw\Big)= \ba\circ \bb \circ \bc.
		\end{split}
	\end{equation}
\end{Lemma}
\emph{Proof.} Due to the independence among $\bu, \bv, \bw$, the conclusion is easy to obtain by using the moment of standard Gaussian random variable. \hfill $\blacksquare$\\


Note that in the left side of \eqref{eqn:tensor_expectation}, it involves an expectation of rank-one tensor. When multiplying any non-random rank-one tensor with same dimensionality, i.e. $\ba_1 \circ \bb_1 \circ \bc_1$, on both sides, it will facilitate us to calculate the expectation of product of Gaussian vectors, see next Lemma for details.


\begin{lemma}
	\label{cor:expectation_gaussian_vector}
	Suppose $\bx\in\mathbb R^p$ is a standard Gaussian random vector. For any non-random vector $\ba, \bb,\bc,\bd \in\mathbb R^p$, we have the following expectation calculation
	\begin{eqnarray*}
	&&\mathbb E(\bx^{\top}\ba)^6 = 15\|\ba\|_2^6,\\
	&&\mathbb E(\bx^{\top}\ba)^5(\bx^{\top}\bb) = 15\|\ba\|_2^4(\ba^{\top}\bb),\\
	&&\mathbb E(\bx^{\top}\ba)^4(\bx^{\top}\bb)^2 = 12\|\ba\|_2^2(\ba^{\top}\bb)^2+3\|\ba\|_2^4\|\bb\|_2^2,\\
	&&\mathbb E(\bx^{\top}\ba)^3(\bx^{\top}\bb)^3 = 6(\ba^{\top}\bb)^3+9(\ba^{\top}\bb)\|\ba\|_2^2\|\bb\|_2^2,\\
	&&\mathbb E(\bx^{\top}\ba)^3(\bx^{\top}\bb)^2(\bx^{\top}\bc) = 6(\ba^{\top}\bb)^2(\ba^{\top}\bc)+6(\ba^{\top}\bb)(\bb^{\top}\bc)(\ba^{\top}\ba)\\
	&&+3(\ba^{\top}\bc)(\bb^{\top}\bb)(\ba^{\top}\ba),\\
	&&\mathbb E(\bx^{\top}\ba)^2(\bx^{\top}\bb)(\bx^{\top}\bc)^2(\bx^{\top}\bd) = 2(\ba^{\top}\bc)^2(\bb^{\top}\bd) + 4(\ba^{\top}\bc)(\bb^{\top}\bc)(\ba^{\top}\bd)\\
	&&+6(\ba^{\top}\bc)(\ba^{\top}\bb)(\bc^{\top}\bd)+3(\bc^{\top}\bx)(\bb^{\top}\bd)(\ba^{\top}\ba).
	\end{eqnarray*}
\end{lemma}

\emph{Proof.} Note that $\mathbb E((\bx^{\top}\ba)^3(\bx^{\top}\bb)^3) = \mathbb E ((\bx^{\top}\ba)^3\langle\bx\circ \bx\circ \bx, \bb \circ \bb \circ \bb \rangle)$. Then we can apply the general result in Lemma \ref{lemma:tensor_expectation}. Comparing both sides, we will obtain the conclusion. Others part follows the similar strategy. \hfill $\blacksquare$\\







Next lemma provides a probabilistic concentration bound for non-symmetric rank-one tensor under tensor spectral norm.
\begin{Lemma} \label{lemma:tensor_concentration}
	Suppose $\bX =(\bx_1^{\top}, \cdots, \bx_n^{\top})^{\top}, \bY =(\by_1^{\top}, \cdots, \by_n^{\top})^{\top}, \bZ =(\bz_1^{\top}, \cdots, \bz_n^{\top})^{\top}$ are three $n\times p$ random matrices. The $\psi_2$-norm of each entry is bounded, s.t. $\|X_{ij}\|_{\psi_2}= K_x, \|Y_{ij}\|_{\psi_2}= K_y, \|Z_{ij}\|_{\psi_2}=K_z$. We assume the row of $\bX,\bY,\bZ$ are independent. There exists an absolute constant $C$ such that,
	\begin{equation*}
	\begin{split}
&\mathbb P\Big(\Big\|\frac{1}{n}\sum_{i=1}^n\Big[\bx_i\circ\by_i\circ\bz_i-\mathbb E(\bx_i\circ\by_i\circ\bz_i)\Big]\Big\|_{s}\geq C K_xK_yK_z\delta_{n,p,s}\Big)\leq p^{-1}.\\
&\mathbb P\Big(\Big\|\frac{1}{n}\sum_{i=1}^n\Big[\bx_i\circ\bx_i\circ\bx_i-\mathbb E(\bx_i\circ\bx_i\circ\bx_i)\Big]\Big\|_{s}\geq C K_x^3\delta_{n,p,s}\Big)\leq p^{-1}.
\end{split}
	\end{equation*}
Here, $\|\cdot\|_{s}$ is the sparse tensor spectral norm defined in \eqref{def:sparse_spectral} and $\delta_{n,p,s}= \sqrt{s\log (ep/s)/n}+\sqrt{s^3\log(ep/s)^3/n^2}$.
\end{Lemma}

\emph{Proof.}
Bounding spectral norm always relies on the construction of the $\epsilon$-net. Since we will bound a sparse tensor spectral norm, our strategy is to discrete the sparse set and construct the $\epsilon$-net on each one. Let us define a sparse set $\cB_0=\{\bx\in \mathbb R^p, \|\bx\|_2=1, \|\bx\|_0\leq s \}$. And let $\cB_{0,s}$ be the $s$-dimensional set defined by $\cB_{0,s}=\{\bx\in\mathbb R^s,\|\bx\|_2=1\}$. Note that $\cB_0$ is corresponding to $s$-sparse unit vector set which can be expressed as a union of subsets of dimension $s$ by expanding some zeros, namely $\cB_0=\cup \ \cB_{0,s}$. There should be at most ${p\choose s}\leq (\frac{ep}{s})^s$ such set $\cB_{0,s}$.

Recalling the definition of sparse tensor spectral norm in \eqref{def:sparse_spectral}, we have
\begin{eqnarray*}
	&&A=\Big\|\frac{1}{n}\sum_{i=1}^n\Big[\bx_i\circ\by_i\circ\bz_i-\mathbb E(\bx_i\circ\by_i\circ\bz_i)\Big]\Big\|_{s}\\
	&=& \sup_{\bchi_1,\bchi_2,\bchi_3\in \cB_0}\Big|\frac{1}{n}\sum_{i=1}^n \Big[\langle\bx_i,\bchi_1\rangle\langle\by_i,\bchi_2\rangle\langle\bz_i,\bchi_3\rangle-\mathbb E(\langle\bx_i,\bchi_1\rangle\langle\by_i,\bchi_2\rangle\langle\bz_i,\bchi_3\rangle)\Big]\Big|.
\end{eqnarray*}
Instead of constructing the $\epsilon$-net on $\cB_0$, we will construct an $\epsilon$-net for each of subsets $\cB_{0,s}$. Define $\cN_{\cB_{0,s}}$ as the $1/2$-set of $\cB_{0,s}$. From Lemma 3.18 in \cite{ledoux2005concentration}, the cardinality of $\cN_{0,s}$ is bounded by $5^s$. By Lemma \ref{lemma:varepsilon_net}, we obtain
\begin{equation}\label{ineqn:sup}
\begin{split}
&\sup_{\bchi_1,\bchi_2,\bchi_3\in \cB_{0,s}}\Big|\frac{1}{n}\sum_{i=1}^n \Big[\langle\bx_i,\bchi_1\rangle\langle\by_i,\bchi_2\rangle\langle\bz_i,\bchi_3\rangle-\mathbb E(\langle\bx_i,\bchi_1\rangle\langle\by_i,\bchi_2\rangle\langle\bz_i,\bchi_3\rangle)\Big]\Big|\\
\leq &2^3\sup_{\bchi_1,\bchi_2,\bchi_3\in \cN_{\cB_{0,s}}}\Big|\frac{1}{n}\sum_{i=1}^n \Big[\langle\bx_i,\bchi_1\rangle\langle\by_i,\bchi_2\rangle\langle\bz_i,\bchi_3\rangle-\mathbb E(\langle\bx_i,\bchi_1\rangle\langle\by_i,\bchi_2\rangle\langle\bz_i,\bchi_3\rangle)\Big]\Big|.
\end{split}
\end{equation}
By rotation invariance of sub-Gaussian random variable, $\langle\bx_i,\bchi_1\rangle$, $\langle\by_i,\bchi_2\rangle$, $\langle\bz_i,\bchi_3\rangle$ are still sub-Gaussian random variables with $\psi_2$-norm bounded by $K_x, K_y, K_z$, respectively.  Applying Lemma \ref{cor:concentr_high_order} and union bound over $\cN_{\cB_{0,s}}$, the right hand side of \eqref{ineqn:sup} can be bounded by
\begin{eqnarray*}
\mathbb P\Big(\text{RHS}\geq 8 K_xK_yK_zC\Big(\sqrt{\frac{\log\delta^{-1}}{n}}+\sqrt{\frac{(\log \delta^{-1})^{3}}{n^2}}\Big)\Big)\leq (5^s)^3\delta,
\end{eqnarray*}
for any $0<\delta<1$.

Lastly, taking the union bound over all possible subsets $\cB_{0,s}$ yields that
\begin{eqnarray*}
&&\mathbb P\Big(A\geq 8 K_xK_yK_zC\Big(\sqrt{\frac{\log\delta^{-1}}{n}}+\sqrt{\frac{(\log \delta^{-1})^{3}}{n^2}}\Big)\Big)\\
&\leq &(\frac{ep}{s})^s(5^s)^3\delta = (\frac{125ep}{s})^s\delta.
\end{eqnarray*}
Letting $p^{-1} = (\frac{125ep}{s})^s\delta$, we obtain with probability at least $1-1/p$
\begin{eqnarray*}
A
\leq C K_xK_yK_z\Big(\sqrt{\frac{s\log (p/s)}{n}}+\sqrt{\frac{s^3\log^3(p/s)}{n^2}}\Big),
\end{eqnarray*}
with some adjustments on constant C. The proof for symmetric case is similar to non-symmetric case so we omit here. 
\hfill $\blacksquare$\\


\begin{comment}
\emph{Proof.} The proof borrows the concentration result of sub-Gaussian vectors in \cite{YCS16}. Part three of Lemma 10 in \cite{YCS16} states that there exist constants $C_i$ such that for every $t\in(0, K^3\sqrt{p})$, when $n\geq C_1 (K^3/t)^2p^2$,
\begin{eqnarray*}
\mathbb P\Big(\Big\|\frac{1}{n}\sum_{i=1}^{n}\bX_i\circ \bX_i\circ \bX_i-\mathbb  E(\bX\circ\bX\circ\bX)\Big\|_{op}\geq t\Big)\leq e^{-C_2nt^2/(p^2K^6)}.
\end{eqnarray*}
Letting $\exp(-C_2nt^2) = \delta$, we have
\begin{equation*}
\Big\|\frac{1}{n}\sum_{i=1}^{n}\bX_i\circ \bX_i\circ \bX_i-\mathbb  E(\bX\circ\bX\circ\bX)\Big\|_{op}\leq CpK^3\sqrt{\frac{\log \delta^{-1}}{n}}
\end{equation*}
with probability at least $1-\delta$. By using similar idea in the proof of Lemma \ref{lemma:tensor_concentration}, we can transfer tensor spectral norm to sparse tensor spectral norm. The detail proof is omitted here. \hfill $\blacksquare$\\


Next lemma provides concentration results for non-identical cubes of sub-Gaussian random variable. 
\begin{lemma}
	\label{lemma: nonidential_cubes}
	Suppose $\{X_i\}_{i=1}^n, \{Y_i\}_{i=1}^n, \{Z_i\}_{i=1}^n$ are independent centered sub-Gaussian random variables with Orlicz norm $\|X_i\|_{\psi_2}\leq K_x$, $\|Y_i\|_{\psi_2}\leq K_y$, $\|Z_i\|_{\psi_2}\leq K_z$. For any non-random vector $\ba\in\mathbb R^n$, we conclude that,
\begin{eqnarray*}
	\mathbb P\Big(\Big|\frac{1}{n}\sum_{i=1}^na_iX_iY_iZ_i\Big|\geq \frac{K_xK_yK_z}{\sqrt{C_1C_2}}\|\ba\|_{2}\frac{\sqrt{\log(ne\delta^{-1})\log 2/\delta}}{n}\Big)\leq 2\delta,
\end{eqnarray*}
holds for $\delta\geq \exp(-C_1\|\ba\|_2^2/\|\ba\|_{\infty}^2)/2$, where $C_1, C_2$ are absolute constants.
	%\begin{eqnarray}
	%&&\mathbb P\Big(\Big|\frac{1}{n}\sum_{i=1}^na_iX_iY_iZ_i\Big| \geq CK_xK_yK_z\sqrt{\log n}\frac{\|\ba\|_2\sqrt{\log 2/\delta}+\|\ba\|_{\infty}\log 2/\delta}{n}\Big)\leq \delta+\frac{e}{n}\label{conclusion_1}\\
    %&&\mathbb P\Big(\Big|\frac{1}{n}\sum_{i=1}^na_iX_iY_iZ_i\Big|\geq CK_xK_yK_z\sqrt{\log(ne\delta^{-1})}\frac{\sqrt{\log (2/\delta)}\|\ba\|_2+\|\ba\|_{\infty}\log 2/\delta}{n}\Big)\leq 2\delta.\label{conclusion_2}
	%\end{eqnarray}
	%for some constant $C$.
\end{lemma}

\emph{Proof.} To overcome the obstacle from cube structure, we will lower the order of sub-Gaussian random variable by truncation. Denote the universal truncation level for $\{X_i| i\in[n]\}$ by $M$. It could possibly depend on $n$. And denote $X_i'=X_i\big||X_i|\leq M$ for any $i\in[n]$. According to the law of total probability, we have
\begin{eqnarray*}
&&\mathbb P\Big(\Big|\frac{1}{n}\sum_{i=1}^na_iX_iY_iZ_i\Big|\geq t\Big)\nonumber\\
&=& \mathbb P\Big(\Big|\frac{1}{n}\sum_{i=1}^na_iX_iY_iZ_i\Big|\geq t\Big|\bigcap_{i=1}^n\big\{|X_i|\leq M\big\}\Big)\mathbb P\Big(\bigcap_{i=1}^n\big\{|X_i|\leq M\big\}\Big)\nonumber\\
&&+\mathbb P\Big(\Big|\frac{1}{n}\sum_{i=1}^na_iX_iY_iZ_i\Big|\geq t\Big|\big(\bigcap_{i=1}^n\big\{|X_i|\leq M\big\}\big)^c\Big)\mathbb P\Big(\big(\bigcap_{i=1}^n\big\{|X_i|\leq M\big\}\big)^c\Big)\nonumber\\
&\leq& \mathbb P\Big(\Big|\frac{1}{n}\sum_{i=1}^na_iX_iY_iZ_i\Big|\geq t\Big|\bigcap_{i=1}^n\big\{|X_i|\leq M\big\}\Big)+\mathbb P\Big(\big(\bigcap_{i=1}^n\big\{|X_i|\leq M\big\}\big)^c\Big)\nonumber\\
&\leq& \underbrace{\mathbb P\Big(\Big|\frac{1}{n}\sum_{i=1}^na_iX_i'Y_iZ_i\Big|\geq t\Big)}_{I_1}+\underbrace{\sum_{i=1}^n\mathbb P\Big(\big|X_i\big|> M\Big)}_{I_2},
\end{eqnarray*}
where the last inequality is due to independence among $X_i, Y_i, Z_i$. 


We bound $I_1$ first. According to Lemma \ref{lemma:bounded_gaussian}, $X_i'Y_i$ is a sub-Gaussian variable with Orlicz norm $\|X_i'Y_i\|_{\psi_2} =MK_y$. This further implies that $X_i'Y_iZ_i$ is a centered sub-exponential random variable with Orlicz norm $\|X_i'Y_iZ_i\|_{\psi_1} = MK_yK_z$. Applying standard Bernstein-type inequality in \cite{RV12}, for every $\ba = (a_1, \ldots, a_n)\in \mathbb R^n$ and every $t\geq0$ we have
\begin{eqnarray}
\label{eqn:bernstein_type}
	\mathbb P\Big(\Big|\sum_{i=1}^na_i X_i'Y_iZ_i\Big|\geq t\Big)\leq 2\exp\Big(-C_1\min\Big\{\frac{t^2}{(MK_yK_z)^2\|\ba\|_2^2},\frac{t}{MK_yK_z\|\ba\|_{\infty}}\Big\}\Big).
\end{eqnarray}
When $t\leq MK_yK_z\|\ba\|_2^2/\|\ba\|_{\infty}$, the small deviation bound reduces to
\begin{equation*}
\mathbb P\Big(\Big|\sum_{i=1}^na_i X_i'Y_iZ_i\Big|\geq t\Big)\leq 2\exp\Big(-C_1\frac{t^2}{(MK_yK_z)^2\|\ba\|_2^2}\Big).
\end{equation*}
Letting $t=MK_yK_z\|\ba\|_2\sqrt{\log (\delta^{-1}/2)/C_1}$, we have
\begin{equation}\label{eq:sub_exp}
\mathbb P\Big(\Big|\sum_{i=1}^na_i X_i'Y_iZ_i\Big|\geq MK_yK_z\|\ba\|_2\sqrt{\log (\delta^{-1}/2)/C_1}\Big)\leq \delta,
\end{equation}
holds for $\delta\geq \exp(-C_1\|\ba\|_2^2/\|\ba\|_{\infty}^2)/2$.



Next we bound $I_2$. From the tail behavior of sub-Gaussian random variable $X_i$,
\begin{eqnarray*}
\mathbb P\Big(\big|X_i\big|> M\Big)\leq \exp\Big(1-C_2M^2/K_x^2\Big).
\end{eqnarray*}
By choosing $M=K_x\sqrt{\log (ne\delta^{-1})/C_2}$, it gives
\begin{eqnarray}
\label{case2_I_2}
\sum_{i=1}^n\mathbb P\Big(\big|X_i\big|> K_x\sqrt{\log (ne\delta^{-1})/C_2}\Big)\leq \delta.
\end{eqnarray}
Combining (\ref{eq:sub_exp}) and (\ref{case2_I_2}) together, we conclude that for $\delta\geq \exp(-C_1\|\ba\|_2^2/\|\ba\|_{\infty}^2)/2$,
\begin{eqnarray*}
	\mathbb P\Big(\Big|\frac{1}{n}\sum_{i=1}^na_iX_iY_iZ_i\Big|\geq \frac{K_xK_yK_z}{\sqrt{C_1C_2}}\|\ba\|_{2}\frac{\sqrt{\log(ne\delta^{-1})\log 2/\delta}}{n}\Big)\leq 2\delta,
\end{eqnarray*}
where $C_1, C_2$ are absolute constant. This ends the proof.
\hfill $\blacksquare$\\

Correspondingly, we have a concentration result for identical cubes of sub-Gaussian random variable. 
\begin{lemma}
	Suppose $\{X_i\}_{i=1}^n$ are independent sub-Gaussian random variables with Orlicz norm $\|X_i\|_{\psi_2}\leq K$. There exists an absolute constant $C$ such that for any $\delta\in(0,1)$,
	\begin{eqnarray}
	\mathbb P\Big(\Big|\frac{1}{n}\sum_{i=1}^nX_i^3-\mathbb E[X_i^3]\Big|>CK^3\frac{\sqrt{\log^3(1/\delta)+2\log^2(1/\delta)n}}{n}\Big)\leq \delta.
	\end{eqnarray}
\end{lemma}

\emph{Proof.} Detail proof can refer Lemma 11 in \citep{YCS16}. \hfill $\blacksquare$\\
\end{comment}



\begin{Lemma}[(Tensor Covering Number(Lemma 4 in  \cite{nguyen2015tensor} ))]\label{lemma:varepsilon_net}
	Let $\mathbb N$ be an $\epsilon$-net for a set $\bB$ associated with a norm $\|\cdot\|$. Then, the spectral norm of a $d$-mode tensor $\cA$ is bounded by 
	\begin{equation*}
		\begin{split}
	&\sup_{\bx_1,\ldots,\bx_{d-1}\in \bB}\|\cA \times_1\bx_1\ldots \times_{d-1}\bx_{d-1}\|_2\\
	&\leq \Big(\frac{1}{1-\varepsilon}\Big)^{d-1}\sup_{\bx_1\cdots\bx_{d-1}\in\mathbb N}\|\cA \times_1 \bx_1\cdots\times_{d-1}\bx_{d-1}\|_2.
	\end{split}
	\end{equation*}
	This immediately implies that the spectral norm of a $d$-mode tensor $\cA$ is bounded by
	\begin{eqnarray*}
	\|\cA\|_2 \leq (\frac{1}{1-\epsilon})^{d-1}\sup_{\bx_1\ldots\bx_{d-1}\in \cN}\|\cA\times_1\bx_1\cdots\times_{d-1}\bx_{d-1}\|_2,
	\end{eqnarray*}
	where $\mathbb N$ is the $\epsilon$-net for the unit sphere $\mathbb S^{n-1}$ in $\mathbb R^n$.
\end{Lemma}


\begin{Lemma}[(Sub-Gaussianess of the Product of Random Variables)]
	\label{lemma:bounded_gaussian}
	Suppose $X_1$ is a bounded random variable with $|X_1|\leq K_1$ almost surely for some $K_1$ and $X_2$ is a sub-Gaussian random variable with Orlicz norm $\|X_2\|_{\psi_2}K_2$. Then $X_1X_2$ is still a sub-Gaussian random variable with Orlicz norm $\|X_1X_2\|_{\psi_2} = K_1K_2$.
\end{Lemma}

\emph{Proof:} Following the definition of sub-Gaussian random variable, we have
\begin{eqnarray*}
  \mathbb P\Big(\big|X_1X_2\big|>t\Big)=\mathbb P\Big(\big|X_2\big|>\frac{t}{\big|X_1\big|}\Big)\leq \mathbb P\Big(\big|X_2\big|>\frac{t}{\big|K_1\big|}\Big)\leq \exp\Big(1-t^2/K_1^2K_2^2\Big),
\end{eqnarray*}
holds for all $t\geq 0$. This ends the proof.
\hfill $\blacksquare$\\

\begin{Lemma}[(Tail Probability for the Sum of Sub-exponential Random Variables (Lemma A.7 in \cite{CLM16}))]
	\label{lemma:sub_exp}
	Suppose $\epsilon_1,\ldots,\epsilon_n$ are independent centered sub-exponential random variables with
	\begin{eqnarray*}
	\sigma:=\max_{1\leq i \leq n}\|\epsilon_i\|_{\psi_1}.
	\end{eqnarray*}
	Then with probability at least $1-3/n$, we have
	\begin{equation*}
	\begin{split}
	&\Big|\frac{1}{n}\sum_{i=1}^n\epsilon_i\Big|\leq C_0\sigma\sqrt{\frac{\log n}{n}}, \   \big\|\bepsilon\big\|_{\infty}\leq C_0\sigma\log n,\\ &  \Big|\frac{1}{n}\sum_{i=1}^n\epsilon_i^2\Big|\leq C_0 \sigma^2, \Big|\frac{1}{n}\sum_{i=1}^n\epsilon_i^4\Big| \leq C_0 \sigma^4,
	\end{split}
		\end{equation*}
	for some constant $C_0$.
\end{Lemma}

\begin{Lemma}[(Tail Probability for the Sum of Weibull Distributions (Lemma 3.6 in \cite{ALPT2011}))]\label{lemma:alpha_1}
    Let $\alpha\in[1,2]$ and $Y_1,\ldots, Y_n$ be independent symmetric random variables satisfying $\mathbb P(|Y_i|\geq t)=\exp (-t^{\alpha})$. Then for every vector $\ba = (a_1,\ldots, a_n)\in \mathbb R^n$ and every $t\geq 0$,
    \begin{equation*}
        \mathbb P\Big(|\sum_{i=1}^n a_iY_i|\geq t\Big) \leq 2\exp\Big(-c\min\Big(\frac{t^2}{\|\ba\|_2^2}, \frac{t^{\alpha}}{\|\ba\|_{\alpha^*}^{\alpha}}\Big)\Big)
    \end{equation*}
\end{Lemma}
\emph{Proof.} It is a combination of Corollaries 2.9 and 2.10 in \cite{talagrand1994supremum}.

\begin{Lemma}[(Moments for the Sum of Weibull Distributions  (Corollary 1.2 in \cite{bogucki2015suprema}))]\label{lemma:alpha2}
    Let $X_1, X_2,\ldots, X_n$ be a sequence of independent symmetric random variables satisfying $\mathbb P(|Y_i|\geq t)=\exp (-t^{\alpha})$, where $0<\alpha<1$. Then, for $p\geq 2$ and some constant $C(\alpha)$ which depends only on $\alpha$,
    \begin{equation*}
        \left\|\sum_{i=1}^n a_iX_i\right\|_p\leq C(\alpha)(\sqrt{p} \|\ba\|_2+ p^{1/\alpha}\|\ba\|_{\infty}).
    \end{equation*}
\end{Lemma}

\begin{Lemma}[(Stein's Lemma \citep{stein2004use})]\label{lemma:stein_lemma}
    Let $\bx\in\mathbb R^{d}$ be a random vector with joint density function $p(\bx)$. Suppose the score function $\nabla_{\bx}\log p(\bx)$ exists. Consider any continuously differentiable function $G(\bx):\mathbb R^{d_x}\rightarrow \mathbb R$. Then, we have 
    \begin{equation*}
        \mathbb E\Big[G(\bx)\cdot \nabla_{\bx}\log p(\bx)\Big] = -\mathbb E\Big[\nabla_{\bx}G(\bx)\Big].
    \end{equation*}
\end{Lemma}

\begin{Lemma}[(Khinchin-Kahane Inequality (Theorem 1.3.1 in \cite{de2012decoupling}))]\label{lemma:Khi}
    Let $\{a_i\}_{i=1}^n$ a finite non-random sequence, $\{\varepsilon_i\}_{i=1}^n$ be a sequence of independent Rademacher variables and $1<p<q<\infty$. Then 
    \begin{equation*}
        \Big\|\sum_{i=1}^n \varepsilon_ia_i\Big\|_q \leq \Big(\frac{q-1}{p-1}\Big)^{1/2}\Big\|\sum_{i=1}^n\varepsilon_i a_i\Big\|_p.
    \end{equation*}
\end{Lemma}

\begin{Lemma}\label{lemma:proof_incoherence}
    Suppose each non-zero element of $\{\bx_k\}_{k=1}^K$ is drawn from standard Gaussian distribution and $\|\bx_k\|_0\leq s$ for $k\in[K]$. Then we have for any $0<\delta\leq 1$,
    \begin{equation*}
        \mathbb P\Big(\max_{1\leq k_1<k_2\leq K}|\langle \bx_{k_1}, \bx_{k_2} \rangle|\leq C\sqrt{s}\sqrt{\log K+\log 1/\delta}\Big)\geq 1-\delta,
    \end{equation*}
    where $C$ is some constant.
\end{Lemma}
\emph{Proof.} Let us denote $\cS_{k_1k_2}\subset [1,2,\ldots, p]$ as an index set such that for any $i, j\in \cS_{k_1k_2}$, we have $x_{k_1i}\neq 0$ and $x_{k_2j}\neq 0$. From the definition of $\cS_{k_1k_2}$, we know that $|\cS_{k_1k_2}|\leq s$ and $\bx_{k_1}^{\top}\bx_{k_2} = \sum_{j=1}^px_{k_1j}x_{k_2j} = \sum_{j\in\cS_{k_1k_2}}x_{k_1j}x_{k_2j}$. We apply standard Hoeffding's concentration inequality,
\begin{eqnarray*}
 \mathbb P\Big(|\langle \bx_{k_1}, \bx_{k_2} \rangle|\geq t\Big)=\mathbb P\Big(|\sum_{j\in\cS_{k_1k_2}}x_{k_1j}x_{k_2j}|\geq t\Big)\leq e\exp\Big(-\frac{ct^2}{s}\Big).
\end{eqnarray*}
Letting $ct^2/s = \log (1/\delta)$, we reach the conclusion.

